Semiparametric plug-in estimation, sup-norm risk bounds, marginal optimization, and inference in BTL model

The recent paper \cite{GSZ2023} on estimation and inference for top-ranking problem in Bradley-Terry-Lice (BTL) model presented a surprising result: component-wise estimation and inference can be done under much weaker conditions on the number of comparison then it is required for the full dimensional estimation. The present paper revisits this finding from completely different viewpoint. Namely, we show how a theoretical study of \emph{estimation in sup-norm} can be reduced to the analysis of \emph{plug-in semiparametric estimation}. For the latter, we adopt and extend the general approach from \cite{Sp2024} to high-dimensional estimation and inference. The main tool of the analysis is a theory of \emph{perturbed marginal optimization} when an objective function depends on a low-dimensional target parameter along with a high-dimensional nuisance parameter. A particular focus of the study is the critical dimension condition. Full-dimensional estimation requires in general the condition \( \mathbbmsl{N} \gg \mathbb{p} \) between the effective parameter dimension \( \mathbb{p} \) and the effective sample size \( \mathbbmsl{N} \) corresponding to the smallest eigenvalue of the Fisher information matrix \( \mathbbmsl{F} \). Inference on the estimated parameter is even more demanding: the condition \( \mathbbmsl{N} \gg \mathbb{p}^{2} \) cannot be generally avoided; see \cite{Sp2024}. However, for the sup-norm estimation, the critical dimension condition can be reduced to \( \mathbbmsl{N} \geq C \log p \).

==> localsmooth_short.tex <==
% !TEX root = ../semi/supnorm.tex

\Section{Perturbed optimization. A basic lemma}
Below we consider a function \( \fs(\upsv) \) which is assumed to be strongly concave.
This means that its negative Hessian 
\( \IFN(\upsv) \eqdef - \nabla^{2} \fs(\upsv) \in \Matr_{\dimp} \) is positive definite for all \( \upsv \). 
Also, assume \( \fs(\upsv) \) three or sometimes even four times Gateaux differentiable in \( \upsv \in \Ups \).
For any particular direction \( \uv \in \R^{\dimp} \), we consider the univariate function 
\( \fs(\upsv + t \uv) \) and measure its smoothness in \( t \).

\begin{description}
    \item[\label{LLsT3ref} \( \bb{(\mathcal{T}_{3}^{*})} \)]
    \emph{\( \fs(\upsv) \) is three times differentiable and 
%    is strongly concave, \( \DFN^{2}(\upsv) \leq - \nabla^{2} \fs(\upsv) \), and
	}
\begin{EQA}
    \sup_{\uv \colon \| \DFN(\upsv) \uv \| \leq \rr} \,\, \sup_{\zv \in \R^{\dimp}} \,\, 
    \frac{\bigl| \langle \nabla^{3} \fs(\upsv + \uv), \zv^{\otimes 3} \rangle \bigr|}
		 {\| \DFN(\upsv) \zv \|^{3}} 
	& \leq &
	\dltwu_{3} \, .
\label{jcxhydtferyu9j3d6vhew}
\end{EQA}

    \item[\label{LLsT4ref} \( \bb{(\mathcal{T}_{4}^{*})} \)]
    \emph{\( \fs(\upsv) \) is four times differentiable and 
%    strongly concave, \( \DFN^{2}(\upsv) \leq - \nabla^{2} \fs(\upsv) \), and
	}
\begin{EQA}
    \sup_{\uv \colon \| \DFN(\upsv) \uv \| \leq \rr} \,\, \sup_{\zv \in \R^{\dimp}} \,\, 
    \frac{\bigl| \langle \nabla^{4} \fs(\upsv + \uv), \zv^{\otimes 4} \rangle \bigr|}
		 {\| \DFN(\upsv) \zv \|^{4}} 
	& \leq &
	\dltwu_{4} \, .
\label{jcxhydtferyu9j3d6vhew4}
\end{EQA}

\end{description}

%The constants \( \dltwu_{3} \) and \( \hmax_{3} \) are related by 
%\( \dltwu_{3} = \hmax_{3}/\sqrt{n} \).
%
\noindent
By Banach's characterization \cite{Banach1938}, \nameref{LLsT3ref} implies
\begin{EQA}
	\bigl| \langle \nabla^{3} \fs(\upsv + \uv), \zv_{1} \otimes \zv_{2} \otimes \zv_{3} \rangle \bigr|
	& \leq &	 
	\dltwu_{3} \| \DFN(\upsv) \zv_{1} \| \, \| \DFN(\upsv) \zv_{2} \| \, \| \DFN(\upsv) \zv_{3} \| \, 
\label{jbuyfg773jgion94euyyfg}
\end{EQA}
for any \( \uv \) with \( \| \DFN(\upsv) \uv \| \leq \rr \) and all \( \zv_{1} , \zv_{2}, \zv_{3} \in \R^{\dimp} \).
Similarly under \nameref{LLsT4ref}
\begin{EQA}
	\bigl| \langle \nabla^{4} \fs(\upsv + \uv), \zv_{1} \otimes \zv_{2} \otimes \zv_{3} \otimes \zv_{4} \rangle \bigr|
	& \leq &	 
	\dltwu_{4} \prod_{k=1}^{4} \| \DFN(\upsv) \zv_{k} \| \, ,
	%\| \DFN(\upsv) \zv_{2} \| \, \| \DFN(\upsv) \zv_{3} \| \, \| \DFN(\upsv) \zv_{4} \| \, .
	\quad 
	\zv_{1} , \zv_{2}, \zv_{3}, \zv_{4} \in \R^{\dimp} \, .
	\qquad
\label{jbuyfg773jgion94euyyfg4}
\end{EQA}



The values \( \dltwu_{3} \) and \( \dltwu_{4} \) are usually very small.
Some quantitative bounds are given later in this section
under the assumption that the function \( \fs(\upsv) \) can be written in the form \( - \fs(\upsv) = n \hL(\upsv) \) 
for a fixed smooth function \( h(\upsv) \) with the Hessian \( \nabla^{2} \hL(\upsv) \). 
The factor \( n \) has meaning of the sample size%
\ifapp{; see \Chname \ref{ScritdimMLE} or \Chname \ref{SGBvM}.}{.}

\begin{description}
    \item[\label{LLtS3ref} \( \bb{(\mathcal{S}_{3}^{*})} \)]
      \emph{ \( - \fs(\upsv) = n \hL(\upsv) \) for \( \hL(\upsv) \) three times differentiable and
%      convex with \( \nabla^{2} \hL(\upsv) \geq \HL^{2}(\upsv) = \DFN^{2}(\upsv)/n \) and
\begin{EQA}
%	\sup_{\upsv \in \CA_{\GP}} \,\,
	\sup_{\uv \colon \| \HL(\upsv) \uv \| \leq \rr/\sqrt{n}} 
	\frac{\bigl| \langle \nabla^{3} \hL(\upsv + \uv), \uv^{\otimes 3} \rangle \bigr|}{\| \HL(\upsv) \uv \|^{3}}
	& \leq &
	\hmax_{3} \, .
\end{EQA}
}
    \item[\label{LLtS4ref} \( \bb{(\mathcal{S}_{4}^{*})} \)]
      \emph{ the function \( \hL(\cdot) \) satisfies \nameref{LLtS3ref} and  
\begin{EQA}
%	\sup_{\upsv \in \CA_{\GP}} \,\,
	\sup_{\uv \colon \| \HL(\upsv) \uv \| \leq \rr/\sqrt{n}}
	\frac{\bigl| \langle \nabla^{4} \hL(\upsv + \uv), \uv^{\otimes 4} \rangle \bigr|}{\| \HL(\upsv) \uv \|^{4}}
	& \leq &
	\hmax_{4} \, .
\end{EQA}
}
\end{description}

\noindent
\nameref{LLtS3ref} and \nameref{LLtS4ref}
are local versions of the so-called self-concordance condition; see \cite{Ne1988} and \cite{OsBa2021}.
%It is also referred to as \( L_{4}-L_{2} \) norm equivalence; see e.g. \cite{MeZi2020}.
In fact, they require that each univariate function \( \hL(\upsv + t \uv) \) of \( t \in \R \)
is self-concordant with some universal constants \( \hmax_{3} \) and \( \hmax_{4} \).



==> marginal_opt.tex <==
% !TEX root = ../perturb/marginal.tex
%% !TEX root = ../generic.tex

\def\AUv{\Delta}
\def\cmax{\CONST}
\def\upsn{\ups^{\circ}}
\def\pert{t}

\Section{Conditional and marginal optimization}
\label{Ssemiopt}
This section describes the problem of conditional/partial and marginal optimization. 
Consider a function \( \fs(\prmtv) \) of a parameter \( \prmtv \in \R^{\dimttl} \)
which can be represented as \( \prmtv = (\targv,\nuiv) \), where \( \targv \in \R^{\dimp} \)
is the target subvector while \( \nuiv \in \R^{\dimq} \) is a nuisance variable.
Our goal is to study the solution to the optimization problem 
\( \prmtvs = (\targvs,\nuivs) = \argmin_{\prmtv} \fs(\prmtv) \) and, in particular, 
its target component \( \targvs \).
%Later we consider a localized setup with a set \( \Ups \) of pairs \( \prmtv = (\targv,\nuiv) \) 
%to be fixed around \( \prmtvs \).


\Subsection{Partial optimization}
For any fixed value of the nuisance variable \( \nuiv \in \Nui \), consider 
\( \fs_{\nuiv}(\targv) = \fs(\targv,\nuiv) \) as a function of \( \targv \) only.
Below we assume that \( \fs_{\nuiv}(\targv) \) is convex in \( \targv \) for any \( \nuiv \in \Nui \).
Define 
\begin{EQA}[rcl]
	\targv_{\nuiv}
	& \eqdef &
	\argmin_{\targv \colon (\targv,\nuiv) \in \Ups} \fs_{\nuiv}(\targv) \, .
\label{jfoiuy2wedfv7tr2qsdzxdfso}
%	\\
%	\feta_{\nuiv}
%	& \eqdef &
%	\max_{\targv \colon (\targv,\nuiv) \in \Ups} \fs_{\nuiv}(\targv) - \fs(\prmtvs)
%	=
%	\fs_{\nuiv}(\targv_{\nuiv}) - \fs(\prmtvs) .
%\label{kfdy8d3fgfnm0lkgrr3so}
\end{EQA}
%The value \( - \feta_{\nuiv} \) measuring the difference between the global maximum of 
%\( \fs(\prmtv) \) and the partial maximum of \( \fs(\targv,\nuiv) \) w.r.t. \( \targv \) 
%for \( \nuiv \) fixed can be called the \( \nuiv \)-\emph{deficiency}. 
Our goal is to describe variability of the partial solution \( \targv_{\nuiv} \) in \( \nuiv \) in terms of \( \targv_{\nuiv} - \targvs \)
and \( \fs_{\nuiv}(\targv_{\nuiv}) - \fs(\prmtvs) \).
Introduce 
\begin{EQ}[rcccc]
	\Av_{\nuiv}
	& \eqdef &
	\nabla \fs_{\nuiv}(\targvs)
	&=&
	\nabla_{\targv} \fs(\targvs,\nuiv) 
	\, ,
	\\
	\IFN_{\nuiv}
	& \eqdef &
	\nabla^{2} \fs_{\nuiv}(\targvs) 
	&=&
	\nabla_{\targv\targv}^{2} \fs(\targvs,\nuiv) 
	\, .
\label{ge8qwefygw3qytfyju8qfhbdso}
\end{EQ}
Local smoothness of each function \( \fs_{\nuiv}(\cdot) \) around \( \targv_{\nuiv} \) 
can be well described under the self-concordance property.
Let for any \( \nuiv \in \Nui \), some radius \( \rrn_{\nuiv} \) be fixed.
%For ease of notation, we omit the subindex \( \nuiv \) here.
%in a way that \( \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \| \leq \amax \, \rrn \). 
We also assume that a local metric on \( \R^{\dimp} \)
for the target variable \( \targv \) is defined by a matrix \( \DFN_{\nuiv} \in \Matr_{\dimp} \)
that may depend on \( \nuiv \in \Nui \).
Later we assume \nameref{LLsT3ref} %or \nameref{LLsT4ref} 
to be fulfilled for all \( \fs_{\nuiv} \), \( \nuiv \in \Nui \).

\begin{description}

    \item[\label{LLsoT3ref} \( \bb{(\mathcal{T}_{3|\nuiv}^{*})} \)]
      \emph{For \( \nuiv \in \Nui \), 
      % the function \( \fs_{\nuiv}(\targv) \) is strongly convex. 
      % for all \( \targv \in \CA \) 
      %With \( \DFN_{\nuiv}^{2} \leq \dmax^{2} \, \IFN_{\nuiv} \), 
      it holds
\begin{EQA}
%	\sup_{\targv \in \CA_{\GP}} \,\,
	\sup_{\uv \in \R^{\dimp} \colon \| \DFN_{\nuiv} \uv \| \leq \rrn_{\nuiv}}  \,\, \sup_{\zv \in \R^{\dimp}} \,\,
	\frac{\bigl| \langle \nabla^{3} \fs_{\nuiv}(\targv_{\nuiv} + \uv), \zv^{\otimes 3} \rangle \bigr|}
		 {\| \DFN_{\nuiv} \zv \|^{3}}
	& \leq &
	\dltwu_{3} \, .
\label{d6f53ye5vry4fddfgeyd}
\end{EQA}
}

%    \item[\label{LLsoT4ref} \( \bb{(\mathcal{T}_{4|\nuiv}^{*})} \)]
%      \emph{\( \fs_{\nuiv}(\targv) \) follows \nameref{LLsoT3ref} 
%      and }
%\begin{EQA}
%%	\sup_{\targv \in \CA_{\GP}} \,\,
%	\sup_{\uv \in \R^{\dimp} \colon \| \DFN_{\nuiv} \uv \| \leq \rrn}  \,\, \sup_{\zv \in \R^{\dimp}} \,\,
%	\frac{\bigl| \langle \nabla^{4} \fs_{\nuiv}(\targv_{\nuiv} + \uv), \zv^{\otimes 4} \rangle \bigr|}
%		 {\| \DFN_{\nuiv} \zv \|^{4}}
%	& \leq &
%	\dltwu_{4} \, .
%\label{d6f53ye5vry4fddfgeyd4}
%\end{EQA}
\end{description}


Our first result describes the \emph{semiparametric bias} \( \targvs - \targv_{\nuiv} \) caused by using
the value \( \nuiv \) of the nuisance variable in place of \( \nuivs \).

\begin{proposition}
\label{PbiassemiN}
Let \( \fs_{\nuiv}(\targv) \) be a strongly convex function with 
\( \fs_{\nuiv}(\targv_{\nuiv}) = \max_{\targv} \fs_{\nuiv}(\targv) \)  
and \( \IFN_{\nuiv} = \nabla^{2} \fs_{\nuiv}(\targv_{\nuiv}) \).
Let \( \Av_{\nuiv} \) and \( \IFN_{\nuiv} \) be given by \eqref{ge8qwefygw3qytfyju8qfhbdso}.
Assume \nameref{LLsoT3ref} at \( \targv_{\nuiv} \) with \( \DFN_{\nuiv}^{2} \), \( \rrn_{\nuiv} \), and \( \dltwu_{3} \) such that 
\begin{EQA}[c]
	\DFN_{\nuiv}^{2} \leq \dmax^{2} \, \IFN_{\nuiv} ,
	\quad
	\rrn_{\nuiv} \geq \frac{3}{2} \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \| \, ,
	\quad
	\dmax^{2} \dltwu_{3} \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \| < \frac{4}{9} \, .
\label{8difiyfc54wrboer7bjfr}
\end{EQA}
%Assume \nameref{LLsoT3ref} with \( \rrn \geq \amax^{-1} \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \| \) for \( \amax \leq 2/3 \).
%Let also \( \dltwu_{3} \, \rrn/2 < 1 - \amax \).
Then \( \| \DFN_{\nuiv} (\targv_{\nuiv} - \targvs) \| \leq (3/2) \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \| \) and moreover,
\begin{EQ}[rcccl]
    \| \DFN_{\nuiv}^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs + \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
    & \leq &
    \frac{3\dltwu_{3}}{4} \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{2} 
    & \leq &
    \frac{\dltwu_{3} \, \rrn_{\nuiv}}{2} \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|
%	\, ,
%	\qquad
%	\\
%    \| \IFN_{\nuiv}^{1/2} (\targv_{\nuiv} - \targvs - \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
%    & \leq &
%    \frac{3 \dmax^{3} \dltwu_{3} }{4} \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} 
%    & \leq &
%    \frac{\dmax^{2} \dltwu_{3} \, \rr}{2} \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|
	\, .
	\qquad
\label{jhcvu7ejdytur39e9frtfw}
\end{EQ}
Moreover,
\begin{EQA}
	\bigl| 
		2 \fs_{\nuiv}(\targv_{\nuiv}) - 2 \fs_{\nuiv}(\targvs) + \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} 
	\bigr|
	& \leq &
	\frac{5\dltwu_{3}}{2} \, \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{3} \, .
	\qquad
\label{gtxddfujhyfdytet6ywerfd}
\end{EQA}

\end{proposition}

\begin{proof}
Define \( \fn_{\nuiv}(\targv) = \fs_{\nuiv}(\targv) - \langle \targv,\Av_{\nuiv} \rangle \).
Then \( \fn_{\nuiv} \) is convex and \( \nabla \fn_{\nuiv}(\targvs) = 0 \) yielding 
\( \targvs = \argmin_{\targv} \fn_{\nuiv}(\targv) \).
Now Theorem~\ref{PFiWigeneric2} yields \eqref{jhcvu7ejdytur39e9frtfw}.
Also by \eqref{3d3Af12DGttGa2}
\begin{EQA}
	\Bigl| 2 \fn_{\nuiv}(\targvs) - 2 \fn_{\nuiv}(\targv_{\nuiv}) + \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} \Bigr|
	& \leq &
	\frac{\dltwu_{3}}{2} \, \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{3} 
\label{ytduw237832jfg656335hdi}
\end{EQA}
yielding
\begin{EQA}
	\bigl| 
		2 \fs_{\nuiv}(\targvs) - 2 \fs_{\nuiv}(\targv_{\nuiv}) - 2 \langle \targvs - \targv_{\nuiv} , \Av_{\nuiv} \rangle 
		- \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} 
	\bigr|
	& \leq &
	\frac{\dltwu_{3}}{2} \, \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{3} \, .
	\qquad
\label{gtxdbcbcgdfswerfdsdew}
\end{EQA}
By \eqref{jhcvu7ejdytur39e9frtfw}
\begin{EQA}
	&& \nquad
	\bigl| \langle \targvs - \targv_{\nuiv} , \Av_{\nuiv} \rangle + \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} \bigr|
	=
	\bigl| \langle \IFN_{\nuiv}^{1/2} (\targvs - \targv_{\nuiv}) , \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \rangle 
	+ \langle \IFN_{\nuiv}^{-1/2} \Av_{\nuiv},\IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \rangle \bigr|
	\\
	&=&
	\bigl| \langle \IFN_{\nuiv}^{1/2} (\targvs - \targv_{\nuiv} + \IFN_{\nuiv}^{-1} \Av_{\nuiv}) , 
		\IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \rangle 
	\bigr|
	\\
	& \leq &
	\| \DFN_{\nuiv}^{-1} \, \IFN_{\nuiv} (\targvs - \targv_{\nuiv} + \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \| \, \,
		\| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|
	\leq 
	\frac{3\dltwu_{3}}{4} \, \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{3}
\label{duy7cyf6re6eytedhge2}
\end{EQA}
This and \eqref{gtxdbcbcgdfswerfdsdew} imply \eqref{gtxddfujhyfdytet6ywerfd}.
\end{proof}

%Two values \( \nuiv \) and \( \nuivs \) of the nuisance variable in the result 
%of Proposition~\ref{PbiassemiN} can be exchanged. 
%This leads to the following bounds.
%
%
%\begin{proposition}
%\label{PbiassemiNs}
%Define \( \Avs_{\nuiv} \eqdef \nabla \fs_{\nuivs}(\targv_{\nuiv}) \).
%Assume \nameref{LLsoT3ref} with \( \rrn \geq \amax^{-1} \| \IFN^{-1/2} \Avs_{\nuiv} \| \) for 
%\( \amax \leq 2/3 \).
%Let also \( \dltwu_{3} \, \rrn/2 < 1 - \amax \).
%Then
%\begin{EQ}[rcl]
%	\| \IFN^{1/2} (\targvs - \targv_{\nuiv}) \|
%	& \leq &
%	\amax^{-1} \| \IFN^{-1/2} \Avs_{\nuiv} \| \, ,
%\label{duejei9viewe76fyjrtgbhgs}
%	\\
%	\| \IFN^{1/2} (\targv_{\nuiv} - \targvs) - \IFN^{-1/2} \Avs_{\nuiv} \|^{2}
%	& \leq &
%	\dltwu_{3} \, \| \IFN^{-1/2} \Avs_{\nuiv} \|^{3} \, .
%%\label{jhcvu7ejdytur39e9frtfws}
%\end{EQ}
%Moreover,
%\begin{EQA}
%	\bigl| 
%		2 \fs_{\nuivs}(\targvs) - 2 \fs_{\nuivs}(\targv_{\nuiv}) - \| \IFN^{-1/2} \Avs_{\nuiv} \|^{2} 
%	\bigr|
%	& \leq &
%	\dltwu_{3} \, \| \IFN^{-1/2} \Avs_{\nuiv} \|^{3} 
%	+ 2 \sqrt{\dltwu_{3}} \, \| \IFN^{-1/2} \Avs_{\nuiv} \|^{5/2} \, .
%	\qquad
%\label{gtxddfujhyfdytet6ywerfds}
%\end{EQA}
%\end{proposition}

%The approximation bounds can be improved under higher order smoothness of each \( \fs_{\nuiv} \).
%Namely, Proposition~\ref{Pconcgeneric4} implies the following advanced approximation.
%
%\begin{proposition}
%\label{PbiassemiNs4}
%Assume the conditions of Proposition~\ref{PbiassemiN} and \nameref{LLsoT4ref}.
%Define
%\begin{EQA}
%	\avn_{\nuiv} 
%	&=&
%	\IFN_{\nuiv}^{-1} \{ \Av_{\nuiv} + \nabla \Tens_{\nuiv}(\IFN_{\nuiv}^{-1} \Av_{\nuiv}) \} ,
%\label{8vfjvr43223efryfuweefse}
%\end{EQA}
%where \( \Tens_{\nuiv}(\uv) = \frac{1}{6} \langle \nabla_{\targv\targv\targv}^{3} \fs(\targvs,\nuiv), \uv^{\otimes 3} \rangle \)
%and \( \nabla \Tens_{\nuiv}(\uv) = \frac{1}{2} \langle \nabla_{\targv\targv\targv}^{3} \fs(\targvs,\nuiv), \uv^{\otimes 2} \rangle \).
%Then
%\begin{EQ}[rcl]
%	\| \IFN_{\nuiv}^{1/2} \avn_{\nuiv} - \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|
%	& \leq &
%	\frac{\dltwu_{3}}{2} \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} 
%	\leq 
%	\frac{\dltwu_{3} \, \amax \, \rr}{2} \, \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|,
%	\\
%	\| \IFN_{\nuiv}^{1/2} \avn_{\nuiv} \|
%	& \leq &
%	\Bigl( 1 + \frac{\dltwu_{3} \, \amax \, \rr}{2} \Bigr) \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \| \, ,
%	\qquad
%\label{iuvchycvf6e64rygh322se}
%\end{EQ}
%and
%\begin{EQ}[rcccl]
%    \| \IFN_{\nuiv}^{1/2} (\targv_{\nuiv} - \targvs + \avn_{\nuiv}) \|
%    & \leq &
%    \frac{\dltwu_{4} + 3 \dltwu_{3}^{2}}{6(1 - \dltwu_{3} \, \rr)} \, \| \IFN_{\nuiv}^{1/2} \avn_{\nuiv} \|^{3} 
%    & \leq &
%    \frac{\dltwu_{4} + 3 \dltwu_{3}^{2}}{3} \, \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{3} \, .
%%    \| \IFN^{-1/2} \Avs_{\nuiv} \|^{3} \, ,
%\label{DGttGtsGDGm13rGa4se}
%\end{EQ}
%\end{proposition}
%

\Subsection{Conditional optimization under (semi)orthogonality}
\label{SortLaplsemi}
Here we study variability of the value \( \targv_{\nuiv} = \argmin_{\targv} \fs(\targv,\nuiv) \)
w.r.t. the nuisance para\-meter \( \nuiv \).
It appears that local quadratic approximation of the function \( \fs \) in a vicinity of the extreme point
\( \prmtvs \) yields a nearly linear dependence of \( \targv_{\nuiv} \) on \( \nuiv \).
We illustrate this fact on the case of a quadratic function \( \fs(\cdot) \).
Consider the Hessian \( \IFT = \nabla^{2} \fs(\prmtvs) \) in the block form:
\begin{EQA}
	\IFT
	& \eqdef &
	\nabla^{2} \fs(\prmtvs)
	=
	\begin{pmatrix}
	\IFT_{\targv\targv} & \IFT_{\targv\nuiv}
	\\
	\IFT_{\nuiv\targv} & \IFT_{\nuiv\nuiv}
	\end{pmatrix} 
\label{hwe78yf2diwe76tfw67etfwtbso}
\end{EQA}
with \( \IFT_{\nuiv\targv} = \IFT_{\targv\nuiv}^{\T} \).
If \( \fs(\prmtv) \) is quadratic then \( \IFT \) and its blocks do not depend on \( \prmtv \).

\begin{lemma}
\label{Lpartmaxq}
%To see this, suppose for a moment that 
Let \( \fs(\prmtv) \) be {quadratic}, {strongly convex}, and \( \nabla \fs(\prmtvs) = 0 \).
Then
\begin{EQA}
	\targv_{\nuiv} - \targvs 
	&=& 
	- \IFT_{\targv\targv}^{-1} \, \IFT_{\targv\nuiv} \, (\nuiv - \nuivs) .
\label{0fje7fhihy84efiewkw}
\end{EQA}
\end{lemma}

\begin{proof}
The condition \( \nabla \fs(\prmtvs) = 0 \) implies 
\( \fs(\prmtv) = \fs(\prmtvs) + (\prmtv - \prmtvs)^{\T} \IFT \, (\prmtv - \prmtvs)/2 \) 
with \( \IFT = \nabla^{2} \fs(\prmtvs) \).
For \( \nuiv \) fixed, the point \( \targv_{\nuiv} \) minimizes 
\( (\targv - \targvs)^{\T} \IFT_{\targv\targv} \, (\targv - \targvs) /2 + (\targv - \targvs)^{\T} \IFT_{\targv\nuiv} \, (\nuiv - \nuivs) \)
and thus, \( \targv_{\nuiv} - \targvs = - \IFT_{\targv\targv}^{-1} \, \IFT_{\targv\nuiv} \, (\nuiv - \nuivs) \).
\end{proof} 

This observation \eqref{0fje7fhihy84efiewkw} is in fact discouraging 
because the bias \( \targv_{\nuiv} - \targvs \) has the same magnitude as the nuisance parameter \( \nuiv - \nuivs \).
However, the condition \( \IFT_{\targv\nuiv} = 0 \) yields \( \targv_{\nuiv} \equiv \targvs \) 
and the bias vanishes.
If \( \fs(\prmtv) \) is not quadratic, the \emph{orthogonality} condition \( \nabla_{\nuiv} \nabla_{\targv} \, \fs(\targv,\nuiv) \equiv 0 \)
for all \( (\targv,\nuiv) \in \WV \) still ensures a vanishing bias.


\begin{lemma}
\label{Lpartmax}
Let \( \fs(\targv,\nuiv) \) be continuously differentiable and 
\( \nabla_{\nuiv} \nabla_{\targv} \, \fs(\targv,\nuiv) \equiv 0 \).
Then the point 
\( \targv_{\nuiv} = \argmin_{\targv} f(\targv,\nuiv) \) does not depend on \( \nuiv \).
\end{lemma}

\begin{proof}
The condition \( \nabla_{\nuiv} \nabla_{\targv} \, \fs(\targv,\nuiv) \equiv 0 \) implies the decomposition 
\( \fs(\targv,\nuiv) = \fs_{1}(\targv) + \fs_{2}(\nuiv) \) for some functions 
\( \fs_{1} \) and \( \fs_{2} \).
This in turn yields \( \targv_{\nuiv} \equiv \targvs \).
%Moreover, without loss of generality, one may assume \( \fs_{1}(\targvs) = \max_{\targv} \fs_{1}(\targv) = 0 \) and 
%\( \fs_{2}(\nuivs) = \max_{\nuiv} \fs_{2}(\nuiv) = 0 \).  
\end{proof}

In some cases, one can check \emph{semi-orthogonality} condition 
\begin{EQA}
	\nabla_{\nuiv} \nabla_{\targv} \, \fs(\targvs,\nuiv)  
	&=&
	0,
	\qquad
	\forall \nuiv \in \Nui \, .
\label{jdgyefe74erjscgygfydhwse}
\end{EQA}
\ifapp{A typical example is given by nonlinear regression; see Section~\ref{SnonlinLA}.}{}

\begin{lemma}
\label{Lsemiorto}
Assume \eqref{jdgyefe74erjscgygfydhwse}.
Then 
\begin{EQA}[rcccl]
	\nabla_{\targv} \, \fs(\targvs,\nuiv)
	& \equiv &
	0,
	\qquad
%	\IFN_{\nuiv}
%	& \equiv &
%	\IFN_{\nuivs}
%	= 
	\nabla_{\targv\targv}^{2} \fs(\targvs,\nuiv) 
	& \equiv &
	\nabla_{\targv\targv}^{2} \fs(\targvs,\nuivs),
	\qquad
	\nuiv \in \Nui .
\label{0xyc5ftr4j43vefvuruendt}
\end{EQA}
Moreover, if \( \fs(\targv,\nuiv) \) is convex in \( \targv \) given \( \nuiv \) then
\begin{EQA}
	\targv_{\nuiv} 
	& \eqdef & 
	\argmin_{\targv} \fs(\targv,\nuiv) \equiv \targvs ,
	\qquad
	\forall \nuiv \in \Nui \,.
\label{irdtyrnjjutu45r7gjhr}
\end{EQA}
%\( \IFN_{\nuiv} \eqdef - \nabla_{\targv\targv}^{2} \fs(\targvs,\nuiv) \) satisfies
\end{lemma}

\begin{proof}
Consider the vector \( \Av_{\nuiv} = \nabla_{\targv} \, \fs(\targvs,\nuiv) \).
%\begin{EQA}
%	\Av_{\nuiv} 
%	& \eqdef & 
%	\nabla_{\targv} \, \fs(\targvs,\nuiv) \, .
%\label{02h874shki7rwhuyfv}
%\end{EQA}
Obviously \( \Av_{\nuivs} = 0 \).
Moreover, \eqref{jdgyefe74erjscgygfydhwse} implies that \( \Av_{\nuiv} \) 
does not depend on \( \nuiv \) and thus, vanishes everywhere.
As \( \fs \) is convex in \( \targv \), 
this implies \( \fs(\targvs,\nuiv) = \max_{\targv} \fs(\targv,\nuiv) \)
and \( \targv_{\nuiv} = \argmin_{\targv} \fs(\targv,\nuiv) \equiv \targvs \).
Similarly, by \eqref{jdgyefe74erjscgygfydhwse}, it holds
\( \nabla_{\nuiv} \nabla_{\targv\targv} \, \fs(\targvs,\nuiv) \equiv 0 \) 
and \eqref{0xyc5ftr4j43vefvuruendt} follows.
Convexity of \( \fs(\targv,\nuiv) \) in \( \targv \) for \( \nuiv \) fixed and \eqref{0xyc5ftr4j43vefvuruendt} 
imply \eqref{irdtyrnjjutu45r7gjhr}.
\end{proof}

Orthogonality or semi-orthogonality \eqref{jdgyefe74erjscgygfydhwse} conditions are rather 
restrictive and fulfilled only in special situations.
% like nonlinear regression in Section~\ref{SnonlinLA}.
A weaker condition of 
%
\emph{one-point orthogonality} means \( \nabla_{\nuiv} \nabla_{\targv} \, \fs(\targvs,\nuivs) = 0 \).
This condition is not restrictive and can always be enforced by a linear transform of the nuisance variable \( \nuiv \).
%see Section~\ref{Sonepointtrans}.


\Subsection{Semiparametric bias}
\label{Sonepoint}


%\Subsection{A bound on \( \targv_{\nuiv} \)}

This section explains how one can bound variability of 
\( \IFN_{\nuiv} = \nabla_{\targv\targv}^{2} \fs(\targvs,\nuiv) \)
and of the norm of \( \targv_{\nuiv} - \targvs \) under  
conditions on the cross-derivatives of \( \fs(\targv,\nuiv) \) for \( \nuiv = \nuivs \)
or \( \targv = \targvs \).
Suppose that the nuisance variable \( \nuiv \) is already localized to a small vicinity \( \Nui \) of \( \nuivs \).
A typical example is given by the level set \( \Nui \) of the form
\begin{EQA}
	\Nui
	&=&
	\bigl\{ \nuiv \colon \| \HFN (\nuiv - \nuivs) \|_{\nano} \leq \rru \bigr\} ,
\label{6chbdtw2hydfuguye4223w23}
\end{EQA}
where \( \HFN \) is a metric tensor in \( \R^{\dimq} \), 
\( \| \cdot \|_{\nano} \) is a norm in \( \R^{\dimq} \), and \( \rru > 0 \).
Often \( \| \cdot \|_{\nano} \) is the usual \( \ell_{2} \)-norm.
However, in some situations, it is beneficial to use different topology for the target parameter \( \targv \)
and the nuisance parameter \( \nuiv \).
One example is given by estimation in \( \sup \)-norm with \( \| \cdot \|_{\nano} = \| \cdot \|_{\infty} \).

Assume the following condition.

\begin{description}

%    \item[\label{LLpT2ref} \( \bb{(\mathcal{T}_{2,\Nui}^{*})} \)]
%      \emph{
%      It holds with some \( \dltwbns \)
%}
%\begin{EQA}
%	\sup_{\nuiv \in \Nui} \,\, 
%	\sup_{\zv \in \R^{\dimp}, \wv \in \R^{\dimq}} \,
%	\frac{| \langle \nabla_{\targv\nuiv}^{2} \fs(\targvs,\nuiv), \zv \otimes \wv \rangle |}
%		 {\| \DFN \zv \| \, \| \HFN \wv \|_{\nano}}
%	& \leq &
%	\dltwbns \, ;
%	\qquad
%\label{c6ceyecc5e5etcT1}
%\end{EQA}

    \item[\label{LLpT3ref} \( \bb{(\mathcal{T}_{3,\Nui}^{*})} \)]
      \emph{%The function \( \fs(\targvs,\nuiv) \) is strongly convex in \( \nuiv \).
%      With \( \DFN^{2} \leq - \nabla_{\targv\targv}^{2} \fs(\prmtvs) \) and
%      \( \HFN^{2} \leq - \nabla_{\nuiv\nuiv}^{2} \fs(\prmtvs) \), 
      It holds with some \( \dltwun, \dltwunn \)
}
\begin{EQA}[rccl]
	\sup_{\nuiv \in \Nui} \,\, 
	\sup_{\zv \in \R^{\dimp}, \wv \in \R^{\dimq}} \,
	&
	\frac{| \langle \nabla_{\targv\nuiv\nuiv}^{3} \fs(\targvs,\nuiv), \zv \otimes \wv^{\otimes 2} \rangle |}
		 {\| \DFN \zv \| \, \| \HFN \wv \|_{\nano}^{2}}
	& \leq &
	\dltwun \, ,
	\qquad
\label{c6ceyecc5e5etcT2}
	\\
	\sup_{\nuiv \in \Nui} \,\, 
	\sup_{\zv \in \R^{\dimp}, \wv \in \R^{\dimq}} \,
	&
	\frac{| \langle \nabla_{\targv\targv\nuiv}^{3} \fs(\targvs,\nuiv), \zv^{\otimes 2} \otimes \wv \rangle |}
		 {\| \DFN \zv \|^{2} \, \| \HFN \wv \|_{\nano}}
	& \leq &
	\dltwunn \, .
\label{c6ceyecc5e5etctwhcyegwc}
\end{EQA}
\end{description}



\begin{remark}
Later we establish some bounds on the semiparametric bias assuming %\( \dltwu_{3} \, \rr \ll 1 \) from \nameref{LLsoT3ref} and 
\( (\dltwun + \dltwunn) \, \rru \ll 1 \). % from \nameref{LLpT3ref}. 
\end{remark}

\begin{remark}
Condition \nameref{LLpT3ref} only involves mixed derivatives 
%\( \nabla_{\targv\nuiv}^{2} \fs(\targvs,\nuiv) \), 
\( \nabla_{\targv\nuiv\nuiv}^{3} \fs(\targvs,\nuiv) \) and \( \nabla_{\targv\targv\nuiv}^{3} \fs(\targvs,\nuiv) \) 
of \( \fs(\targvs,\nuiv) \) for the fixed value \( \targv = \targvs \),
while condition \nameref{LLsoT3ref} only concerns smoothness of \( \fs(\targv,\nuiv) \) w.r.t. \( \targv \) for \( \nuiv \) fixed.
Therefore, the combination of \nameref{LLsoT3ref} and \nameref{LLpT3ref} is much weaker than the full dimensional 
condition \nameref{LLsT3ref}.
\end{remark}


The next result provides an expansion of the semiparametric bias \( \targv_{\nuiv} - \targvs \). 
For the norm \( \| \cdot \|_{\nano} \), 
let \( \| \BBH \|_{\dual} \) be the corresponding dual norm of an operator
\( \BBH \colon \R^{\dimq} \to \R^{\dimp} \):
\begin{EQA}
	\| \BBH \|_{\dual}
	&=&
	\sup_{\zv \colon \| \zv \|_{\nano} \leq 1} \| \BBH \zv \| .
\label{ygtuesdfhiwdsoif9ruta}
\end{EQA}
If \( p=1 \) and \( \| \cdot \|_{\nano} \) is the sup-norm \( \| \cdot \|_{\infty} \) then 
\( \| \BBH \|_{\dual} = \| \BBH \|_{1} \).
Define
\begin{EQA}
\label{f8vuehery6gv65ftehwee}
	\crossnorm
	& \eqdef &
	\| \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1} \|_{\dual} \, ,
	\\
	\crossgrad
	& \eqdef &
	\| \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1} \|_{\dual} + \dltwun \, \rru /2 \, .
\label{f8vuehery6gv65ftehwee1}
\end{EQA}
%
Proposition~\ref{PbiassemiN} evaluates the semiparametric bias \( \targvs - \targv_{\nuiv} \) in terms of 
the matrix 
%Later we need an upper bound on variability of the matrix 
\( \IFN_{\nuiv} = \nabla_{\targv\targv}^{2} \fs(\targvs,\nuiv) \) and the vector 
\( \Av_{\nuiv} = \nabla \fs_{\nuiv}(\targvs) \).
The next result explains how these quantities can be controlled under \nameref{LLpT3ref}.
To simplify the formulation, we assume that \( \DFN^{2} \leq \IFN \); see Remark~\ref{Rdmax2} for an extension.

\begin{proposition}
\label{PsemiAvex}
Assume \nameref{LLpT3ref} with \( \DFN^{2} \leq \IFN \).
%\( \Nui \) from \eqref{6chbdtw2hydfuguye4223w23}, and
%\( \DFN, \dltwun, \dltwunn , \rru \) satisfying 
Fix \( \nuiv \in \Nui \), set \( \dltwbun \eqdef \dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} \), 
and assume \nameref{LLsoT3ref} with \( \DFN_{\nuiv} \equiv \DFN \), \( \rrn_{\nuiv} \equiv \rrn \), 
and \( \dltwu_{3} \),
such that %with \( \dltwbun \eqdef \dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} \), it holds
\begin{EQA}[c]
	\dltwbun < 1 \, ,
	\quad
	\rr 
	\geq 
	\frac{3 \crossgrad}{2(1 - \dltwbun)} \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, ,
	\quad
	\frac{\crossgrad \, \dltwu_{3}}{1 - \dltwbun} \, \| \HFN (\nuiv - \nuivs) \|_{\nano}
	\leq 
	\frac{4}{9} \, ,
	\qquad
\label{6cuydjd5eg3jfggu8eyt4h}
\end{EQA}
for \( \crossgrad \) from \eqref{f8vuehery6gv65ftehwee1}.
Then the partial solution \( \targv_{\nuiv} \) obeys 
\begin{EQA}
	\| \DFN (\targv_{\nuiv} - \targvs) \|
	& \leq &
	\frac{3 \crossgrad}{2(1 - \dltwbun)} \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \,. 
\label{rhDGtuGmusGU0a2spt}
\end{EQA}
%If \( \IFT_{\targv\nuiv} = \nabla_{\targv} \nabla_{\nuiv} \, \fs(\targvs,\nuivs) = 0 \), then
%for any linear mapping \( \QP \colon \R^{\dimp} \to \R^{\dimq} \)
%\begin{EQA}
%\label{36gfijh94ejdvtwekoi}
%	\| \QP (\targv_{\nuiv} - \targvs) \|
%	& \leq &
%	\| \QP \, \IFN^{-1} \DFN \| \, \frac{1}{1 - \dltwbun}
%	\Bigl( \frac{\dltwun}{2} 
%		+ \frac{3\dltwu_{3} \, \dltwun^{2} \, \rru^{2}}{4(1-\dltwbund)^{2}} 
%	\Bigr) 
%	\| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
%%	(1 + \dltwbun) \, \frac{\dltwun}{2} \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} 
% 	\, .
%\end{EQA}
Moreover, with \( \crossnorm \) from \eqref{f8vuehery6gv65ftehwee}, it holds
\begin{EQA}[c]
\label{36gfijh94ejdvtwekoise}
	\| \QP \{ \targv_{\nuiv} - \targvs + \IFN^{-1} \IFT_{\targv\nuiv} (\nuiv - \nuivs) \} \|
	\leq 
	\| \QP \, \IFN^{-1} \DFN \| \, \dltwuns
	\, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
	\, ,
	\qquad
	\\
	\dltwuns
	\eqdef 
	\frac{1}{1 - \dltwbun} \, 
	\biggl( \crossnorm \, \dltwunn + \frac{\dltwun}{2}
		+ \frac{3\crossgrad^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} 
%		+ \frac{3\dltwu_{3}\, \dltwun^{2} \, \rru^{2}}{4(1 - \dltwbund)^{2}} 
	\biggr) \, .
\label{36gfijh94ejdvtwekoised}
\end{EQA}
\end{proposition}

\begin{proof}
First we bound the variability of \( \IFN_{\nuiv} \) over \( \Nui \). 
%For \( \Nui \) of the form \eqref{6chbdtw2hydfuguye4223w23}, such a bound can be obtained from \nameref{LLpT3ref}.
Let \( \IFN = \IFN_{\nuivs} \).

\begin{lemma}
\label{L3IFNNui}
Assume \nameref{LLpT3ref}.
% and let \( \dltwunn \, \rru < 1 \).
Then for any \( \nuiv \in \Nui \)
\begin{EQA}
	\| \DFN^{-1} \, (\IFN_{\nuiv} - \IFN) \, \DFN^{-1} \|
	& \leq &
	\dltwunn \, \| \HFN (\nuiv - \nuivs) \|_{\nano} 
	\, .
\label{8c7c67cc6c63kdldlvvudw}
\end{EQA}
\end{lemma}

\begin{proof}
Let \( \nuiv \in \Nui \).
By \eqref{c6ceyecc5e5etctwhcyegwc}, for any \( \zv \in \R^{\dimp} \), it holds
\begin{EQA}
	&& \!\!\!\!
	\bigl| \bigl\langle \DFN^{-1} \, (\IFN_{\nuiv} - \IFN) \, \DFN^{-1}, \zv^{\otimes 2} \bigr\rangle \bigr|
	=
	\bigl| \bigl\langle \IFN_{\nuiv} - \IFN, (\DFN^{-1} \zv)^{\otimes 2} \bigr\rangle \bigr|
	\\
	& \leq &
	\sup_{t \in [0,1]}
	\bigl| \langle \nabla_{\targv\targv\nuiv}^{3} \fs(\targvs,\nuivs + t (\nuiv - \nuivs)), (\DFN^{-1} \zv)^{\otimes 2} \otimes (\nuiv - \nuivs) \rangle \bigr|
	\leq 
	\dltwunn \, \| \zv \|^{2}  \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, .
\label{9487654r5tghasdfgsup}
\end{EQA}
This yields \eqref{8c7c67cc6c63kdldlvvudw}.
\end{proof}


The next result describes some corollaries of \eqref{8c7c67cc6c63kdldlvvudw}. 

\begin{lemma}
\label{LIFvari}
Assume \( \DFN^{2} \leq \dmax^{2} \IFN \) and let some other matrix \( \IFN_{1} \in \Matr_{\dimp} \) satisfy
\begin{EQA}
	\| \DFN^{-1} \, (\IFN_{1} - \IFN) \, \DFN^{-1} \|
	& \leq &
	\dmax^{-2} \dltwbun 
\label{icfuifcu7dy7e3gw3ft6e}
\end{EQA}
with \( \dltwbun < 1 \).
Then
%Moreover, if \( \dltwbun \eqdef \dmax^{2} \, \dltwuud \| \HFN (\nuiv - \nuivs) \|_{\nano} < 1 \), then
\begin{EQA}[ccc]
\label{8c7c67cc6c63kdldlvvudw2}
	\| \IFN^{-1/2} \, (\IFN_{1} - \IFN) \, \IFN^{-1/2} \|
	& \leq &
	\dltwbun 
%	=
%	\dmax^{2} \, \dltwuud \| \HFN (\nuiv - \nuivs) \|_{\nano} 
	\, ,
	\\
	\| \IFN^{1/2} \, (\IFN_{1}^{-1} - \IFN^{-1}) \, \IFN^{1/2} \|
	& \leq &
	\frac{\dltwbun}{1 - \dltwbun} 
	\, ,
\label{g98g75re3gf76r4egu4e}
\end{EQA}
and
\begin{EQA}
	\frac{1}{1 + \dltwbun} \, \| \DFN \, \IFN^{-1} \, \DFN \|
	\leq 
	\| \DFN \, \IFN_{1}^{-1} \DFN \|
	& \leq &
	\frac{1}{1 - \dltwbun} \, \| \DFN \, \IFN^{-1} \, \DFN \|
	\, .
\label{g98g75re3gf76r4egu4ee}
\end{EQA}
Furthermore, for any vector \( \uv \)
\begin{EQA}[rcccl]
\label{uciuvcdiu3eoooodffcy}
	(1 - \dltwbun) \| \DFN^{-1} \IFN \uv \|
	& \leq &
	\| \DFN^{-1} \IFN_{1} \uv \|
	& \leq &
	(1 + \dltwbun) \| \DFN^{-1} \IFN \uv \| \, ,
	\qquad
	\\
	\frac{1 - 2 \dltwbun}{1 - \dltwbun} \| \DFN \, \IFN^{-1} \uv \|
	& \leq &
	\| \DFN \, \IFN_{1}^{-1} \uv \|
	& \leq &
	\frac{1}{1 - \dltwbun} \| \DFN \, \IFN^{-1} \uv \| \, .
	\qquad
\label{uciuvcdiu3eoooodffcym}
\end{EQA}
\end{lemma}

\begin{proof}
Statement \eqref{8c7c67cc6c63kdldlvvudw2} follows from \eqref{icfuifcu7dy7e3gw3ft6e}
because of \( \IFN^{-1} \leq \dmax^{2} \, \DFN^{-2} \).
Define now \( \Uv \eqdef \IFN^{-1/2} \, (\IFN_{1} - \IFN) \, \IFN^{-1/2} \). 
Then \( \| \Uv \| \leq \dltwbun \) and
\begin{EQA}
	\| \IFN^{1/2} \, (\IFN_{1}^{-1} - \IFN^{-1}) \, \IFN^{1/2} \|
	&=&
	\| (\Id + \Uv)^{-1} - \Id \|
	\leq 
	\frac{1}{1 - \dltwbun} \| \Uv \|
\label{uefu83yr83y38frkfbg7e}
\end{EQA}
yielding \eqref{g98g75re3gf76r4egu4e}.
Further,
\begin{EQA}
	\| \DFN \, (\IFN_{1}^{-1} - \IFN^{-1}) \, \DFN \|
	&=&
	\| \DFN \, \IFN_{1}^{-1} \IFN_{1} (\IFN_{1}^{-1} - \IFN^{-1}) \, \IFN \, \IFN^{-1} \DFN \|
	\\
	&=&
	\| \DFN \, \IFN_{1}^{-1} \DFN \, \DFN^{-1} (\IFN_{1} - \IFN) \DFN^{-1} \, \DFN \, \IFN^{-1} \DFN \|
	\\
	& \leq &
	\| \DFN \, \IFN_{1}^{-1} \DFN \| \, \| \DFN \, \IFN^{-1} \DFN \| \, \| \DFN^{-1} (\IFN_{1} - \IFN) \DFN^{-1} \| 
	\leq 
	\dltwbun \| \DFN \, \IFN_{1}^{-1} \DFN \| \, .
\label{odfu7eujgvy55r44rf}
\end{EQA}
This implies \eqref{g98g75re3gf76r4egu4ee}.
Also, by \( \DFN^{2} \leq \dmax^{2} \IFN \)
\begin{EQA}
	\| \DFN^{-1} \IFN_{1} \uv \|
	& \leq &
	\| \DFN^{-1} \IFN \uv \| + \| \DFN^{-1} (\IFN_{1} - \IFN) \DFN^{-1} \DFN \uv \|
	\leq 
	\| \DFN^{-1} \IFN \uv \| + \dltwbun \, \| \DFN \uv \|
	\\
	& \leq & 
	\| \DFN^{-1} \IFN \uv \| + \dltwbun \| \DFN^{-1} \IFN \uv \| 
	\leq 
	(1 + \dltwbun) \| \DFN^{-1} \IFN \uv \| \, ,
	\qquad
\label{uciuvcdiu3ery7httrwbgfcy}
\end{EQA}
and \eqref{uciuvcdiu3eoooodffcy} follows.
Similarly
\begin{EQA}
	\| \DFN \, (\IFN_{1}^{-1} - \IFN^{-1}) \uv \| 
	& = &
	\| \DFN \, \IFN_{1}^{-1} (\IFN_{1} - \IFN) \IFN^{-1} \uv \|
	=
	\| \DFN \, \IFN_{1}^{-1} \DFN \,\, \DFN^{-1} (\IFN_{1} - \IFN) \DFN^{-1} \, \DFN \, \IFN^{-1} \uv \|
	\\
	& \leq &
	\| \DFN^{-1} \, (\IFN_{1} - \IFN) \, \DFN^{-1} \| \,\,
	\| \DFN \, \IFN_{1}^{-1} \, \DFN \| \,\, \| \DFN \, \IFN^{-1} \uv \|
	\leq 
	\frac{\dltwbun}{1 - \dltwbun} \| \DFN \, \IFN^{-1} \uv \|
\label{rtiuru8bttg3hfy7vrgf}
\end{EQA}
and \eqref{uciuvcdiu3eoooodffcym} follows as well.
\end{proof}



Definition \eqref{ygtuesdfhiwdsoif9ruta} implies the following bound.
\begin{lemma}
\label{Lsemidual}
For any \( \nuiv \in \Nui \) and any linear mapping \( \QP \), it holds
\begin{EQA}
	\| \QP \IFT_{\targv\nuiv} (\nuiv - \nuivs) \|
	& \leq &
	\| \QP \IFT_{\targv\nuiv} \, \HFN^{-1} \|_{\dual} \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, .
\label{difkjv78frhjrjhfh6wekd}
\end{EQA}
\end{lemma}

The next lemma shows that \( \Av_{\nuiv} = \nabla \fs_{\nuiv}(\targvs) \) is nearly linear in \( \nuiv \).

\begin{lemma}
\label{LvarDVa}
Assume \eqref{c6ceyecc5e5etcT2}.
Then
\begin{EQA}
	\| \DFN^{-1} \{ \Av_{\nuiv} - \IFT_{\targv\nuiv} (\nuiv - \nuivs) \} \|
	& \leq &
	\frac{\dltwun}{2} \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} \, ,
\label{4cbijjm09j9hhrjfifkrs3}
\end{EQA}
and with \( \crossgrad \) from \eqref{f8vuehery6gv65ftehwee1}, it holds
\begin{EQA}
	\| \DFN^{-1} \Av_{\nuiv} \|
	& \leq &
	\Bigl( \| \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1} \|_{\dual} 
	+ \frac{\dltwun}{2} \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \Bigr) \, \| \HFN (\nuiv - \nuivs) \|_{\nano}
	\\
	& \leq &
	\crossgrad \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, .
\label{4cbijjm09j9hhrjfifkrs}
\end{EQA}
\end{lemma}

\begin{proof}
Fix \( \nuiv \in \Nui \) and define \( \av_{\nuiv}(t) \eqdef \Av_{\nuivs + t (\nuiv - \nuivs)} \).
Then \( \av_{\nuiv}(0) = \Av_{\nuivs} = 0 \), \( \av_{\nuiv}(1) = \Av_{\nuiv} \), 
and
\begin{EQA}
	\av_{\nuiv}(1) - \av_{\nuiv}(0) 
	&=&
	\int_{0}^{1} \av'_{\nuiv}(t) \, dt \, ,
\label{dsf7hgduw3heiuwed53ww3}
\end{EQA}
where \( \av'_{\nuiv}(t) = \frac{d}{dt} \av_{\nuiv}(t) \) for \( t \in [0,1] \).
%Condition \eqref{c6ceyecc5e5etcT1} ensures
%\begin{EQA}
%	\bigl| \langle \av'_{\nuiv}(t), \zv \rangle \bigr|
%	&=&
%	\bigl| \bigl\langle \nabla_{\targv\nuiv}^{2} \fs(\targvs,\nuivs + t (\nuiv - \nuivs)), \zv \otimes (\nuiv - \nuivs) \bigr\rangle \bigr|
%	\leq 
%	\crossgrad \, \| \DFN \zv \| \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, .
%\label{5cbgcfyt6webhwefuy62}
%\end{EQA}
%This implies 
%%by \( \DFN^{2} \leq \, \IFN \) 
%\begin{EQA}
%	\| \DFN^{-1} \av'_{\nuiv}(t) \|
%	&=&
%	\sup_{\zv \colon \| \zv \| \leq 1} \bigl| \langle \DFN^{-1} \av'_{\nuiv}(t), \zv \rangle \bigr|
%	=
%	\sup_{\zv \colon \| \zv \| \leq 1}  
%		\bigl| \langle \av'_{\nuiv}(t), \DFN^{-1} \zv \rangle \bigr|
%	\\
%	& \leq &
%	\crossgrad \sup_{\zv \colon \| \zv \| \leq 1}
%	\| \zv \| \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, 
%	=
%	\crossgrad \| \HFN (\nuiv - \nuivs) \|_{\nano} \,
%\label{bje4f7hj4g8mnw3furtf}
%\end{EQA}
%yielding \eqref{4cbijjm09j9hhrjfifkrs}.
Similarly, by \( \av'_{\nuiv}(0) = \IFT_{\targv\nuiv} (\nuiv - \nuivs) \), we derive 
\begin{EQA}
	\av_{\nuiv}(1) - \av_{\nuiv}(0) - \av'_{\nuiv}(0)
	&=&
	\int_{0}^{1} (\av'_{\nuiv}(t) - \av'_{\nuiv}(0)) \, dt
	=
	\int_{0}^{1} (1 - t) \, \av''_{\nuiv}(t) \, dt \, ,
\label{g8eh35fgtg7t76868jdy}
\end{EQA}
where 
\( \av''_{\nuiv}(t) = \frac{d^{2}}{dt^{2}} \av_{\nuiv}(t) \).
By condition \nameref{LLpT3ref} 
\begin{EQA}
	\bigl| \langle \av''_{\nuiv}(t), \zv \rangle \bigr|
	&=&
	\bigl| \bigl\langle \nabla_{\targv\nuiv\nuiv}^{3} \fs(\targvs,\nuivs + t (\nuiv - \nuivs)), \zv \otimes (\nuiv - \nuivs)^{\otimes 2} \bigr\rangle \bigr|
	\leq 
	\dltwun \, \| \DFN \zv \| \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} \, 
\label{5cbgcfyt6webhwefuy6}
\end{EQA}
and hence,
%by \( \DFN^{2} \leq \, \IFN \) 
\begin{EQA}
	\| \DFN^{-1} \av''_{\nuiv}(t) \|
	&=&
	\sup_{\zv \colon \| \zv \| \leq 1} \bigl| \langle \DFN^{-1} \av''_{\nuiv}(t), \zv \rangle \bigr|
	=
	\sup_{\zv \colon \| \zv \| \leq 1}  
		\bigl| \langle \av''_{\nuiv}(t), \DFN^{-1} \zv \rangle \bigr|
	\\
	& \leq &
	\dltwun \sup_{\zv \colon \| \zv \| \leq 1}
	\| \zv \| \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} \, 
	=
	\dltwun  \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} \, .
\label{hgvytew3hw36fdfnhrg}
\end{EQA}
This yields
\begin{EQA}
	\| \DFN^{-1} \{ \Av_{\nuiv} - \IFT_{\targv\nuiv} (\nuiv - \nuivs) \} \|
	& \leq &
	\dltwun \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} \, \int_{0}^{1} (1 - t) \, dt
	\leq 
	\frac{\dltwun \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}}{2} \, 
\label{4cbijjm09j9hhrjfifkr}
\end{EQA}
as claimed in \eqref{4cbijjm09j9hhrjfifkrs3}. 
Lemma~\ref{Lsemidual} implies \eqref{4cbijjm09j9hhrjfifkrs}.
\end{proof}

\noindent
Now Proposition~\ref{PbiassemiN} helps to show \eqref{rhDGtuGmusGU0a2spt} and to bound
\( \targv_{\nuiv} - \targvs - \IFN_{\nuiv}^{-1} \Av_{\nuiv} \).

\begin{lemma}
If \( \dltwbun = \dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} < 1 \) then
\begin{EQA}
	\| \DFN (\targv_{\nuiv} - \targvs) \|
	& \leq &
	\frac{3}{2} \| \DFN \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \| 
	\leq 
	\frac{3 \crossgrad}{2(1 - \dltwbun)} \, \| \HFN (\nuiv - \nuivs) \|_{\nano}\,. 
\label{rhDGtuGmusGU0a2sp}
\end{EQA}
Moreover, 
\begin{EQA}
	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs + \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
	& \leq &
	\frac{3 \crossgrad^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} \, 
	\| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
	\, .
	\qquad
\label{d73jejg7tre3fdy3fujell}
\end{EQA}
\end{lemma}

\begin{proof}
%First rescale \( \DFN \) to reduce the proof to the case \( \dmax = 1 \).
By \( \DFN^{2} \leq \IFN \), \eqref{8c7c67cc6c63kdldlvvudw},
\eqref{uciuvcdiu3eoooodffcym} of Lemma~\ref{LIFvari}, and \eqref{4cbijjm09j9hhrjfifkrs} 
\begin{EQA}
	\| \DFN \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|
	& \leq &
	\| \DFN \, \IFN_{\nuiv}^{-1} \DFN \| \,\, \| \DFN^{-1} \Av_{\nuiv} \|
	\leq 
	\frac{1}{1 - \dltwbun} \, \| \DFN^{-1} \Av_{\nuiv} \|
	\leq 
	\frac{\crossgrad}{1 - \dltwbun} \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, .
\label{6dvgycuw76yeficf7wnfo}
\end{EQA}
This and the conditions of the proposition enable us to apply Proposition~\ref{PbiassemiN} which implies \eqref{rhDGtuGmusGU0a2sp} and
\begin{EQA}
	&& \nquad
	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs + \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
	\leq 
	\frac{3 \dltwu_{3}}{4} \, \| \DFN \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{2}
	\leq 
	\frac{3 \crossgrad^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} \, \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
	\, .
\label{suhyd78wyedw378yedh2}
\end{EQA}
This completes the proof.
\end{proof}


%
%
%\begin{lemma}
%It holds with \( \varrho = \| \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1} \|_{\dual} \)
%and \( \dltwbun = \, \dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} < 1 \)
%\begin{EQA}
%	&& \nquad
%	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs - \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
%	\leq
%	\frac{\dltwu_{3}}{(1 - \dltwbun)^{2}} \, 
%	\Bigl( \varrho^{2} \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} 
%		+ \frac{3 \dltwun^{2}}{4} \| \HFN (\nuiv - \nuivs) \|_{\nano}^{4} 
%	\Bigr)
%	\\
%	& \leq &
%	\frac{\dltwu_{3}}{(1 - \dltwbun)^{2}} \, 
%	\Bigl( \varrho^{2} + \frac{3 \dltwun^{2} \, \rru^{2}}{4} \Bigr) \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
%	\, .
%	\qquad
%\label{d73jejg7tre3fdy3fujelld}
%\end{EQA}
%\end{lemma}
%
%\begin{proof}
%First rescale \( \DFN \) to reduce the proof to the case \( \dmax = 1 \).
%Then \( \DFN^{2} \leq \IFN \) and by \eqref{8c7c67cc6c63kdldlvvudw}, \eqref{uciuvcdiu3eoooodffcym},
%and \eqref{usucxy88u7vjwdodx} 
%\begin{EQA}
%	\| \DFN \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|
%	& \leq &
%	\frac{1}{1 - \dltwbun} \, \| \DFN \, \IFN^{-1} \Av_{\nuiv} \|
%	\leq 
%	\frac{1}{1 - \dltwbun} \, \| \DFN^{-1} \Av_{\nuiv} \|
%	\leq 
%	\frac{1}{1 - \dltwbun} \, \Bigl( \varrho \, \rru + \frac{\dltwun}{2} \rru^{2} \Bigr) \, .
%\label{6dvgycuw76yeficf7wnfo}
%\end{EQA}
%This and the conditions of the proposition enable us to apply Proposition~\ref{PbiassemiN}.
%The use of \( \frac{3}{4} (a+b)^{2} \leq a^{2} + 3 b^{2} \) for any \( a,b \), 
%and of the bound \eqref{jhcvu7ejdytur39e9frtfw} yields with \( \AUv_{\nuiv} \eqdef \IFT_{\targv\nuiv} (\nuiv - \nuivs) \)
%\begin{EQA}
%	&& \nquad
%	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs - \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
%	\leq 
%	\frac{3 \dltwu_{3}}{4} \, \| \DFN \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{2}
%	\leq 
%	\frac{3 \dltwu_{3}}{4} \, \| \DFN \, \IFN_{\nuiv}^{-1} \DFN \|^{2} \, \| \DFN^{-1} \Av_{\nuiv} \|^{2}
%	\\
%	& \leq &
%	\dltwu_{3} \, \| \DFN \, \IFN_{\nuiv}^{-1} \DFN \|^{2} \, 
%	\Bigl( \| \DFN^{-1} \AUv_{\nuiv} \|^{2} + 3 \| \DFN^{-1} (\Av_{\nuiv} - \AUv_{\nuiv}) \|^{2} \Bigr)
%	\, ,
%\label{suhyd78wyedw378yedh}
%\end{EQA}
%where by \eqref{s8dfy8weiu3re5gdh36b} 
%\( \| \DFN^{-1} \AUv_{\nuiv} \| \leq \varrho \| \HFN (\nuiv - \nuivs) \|_{\nano} \).
%The obtained bounds together with \eqref{4cbijjm09j9hhrjfifkrs} and \eqref{g98g75re3gf76r4egu4ee} imply 
%\begin{EQA}[c]
%	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs - \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
%	\leq 
%	\frac{\dltwu_{3}}{(1 - \dltwbun)^{2}} \, 
%	\Bigl( \varrho^{2} \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} 
%		+ \frac{3 \, \dltwun^{2}}{4} \| \HFN (\nuiv - \nuivs) \|_{\nano}^{4} 
%	\Bigr)
%	\, ,
%\label{suhyd78wyedw378yedhh}
%\end{EQA}
%and \eqref{d73jejg7tre3fdy3fujell} follows.
%\end{proof}


Now we can finalize the proof of the proposition.
With \( \AUv_{\nuiv} \eqdef \IFT_{\targv\nuiv} (\nuiv - \nuivs) \), it holds
\begin{EQA}
	&& \nquad
	\targv_{\nuiv} - \targvs + \IFN^{-1} \AUv_{\nuiv}
	=
	\targv_{\nuiv} - \targvs + \IFN_{\nuiv}^{-1} \Av_{\nuiv}
	- \IFN_{\nuiv}^{-1} \Av_{\nuiv}
	+ \IFN^{-1} \AUv_{\nuiv} 
	\\
	& = &
	\targv_{\nuiv} - \targvs + \IFN_{\nuiv}^{-1} \Av_{\nuiv}
	- \IFN_{\nuiv}^{-1} (\Av_{\nuiv} - \AUv_{\nuiv}) 
	- (\IFN_{\nuiv}^{-1} - \IFN^{-1}) \AUv_{\nuiv}
	\, .
\label{36gfijh94ejdvtwekoDg}
\end{EQA}
The use of \eqref{8c7c67cc6c63kdldlvvudw} and \eqref{f8vuehery6gv65ftehwee} yields
\begin{EQA}
	&& \! \! \! \! \! \! \! \! 
	\| \DFN^{-1} \IFN_{\nuiv} (\IFN^{-1} - \IFN_{\nuiv}^{-1}) \AUv_{\nuiv} \|
	= 
	\| \DFN^{-1} (\IFN - \IFN_{\nuiv}) \IFN^{-1} \AUv_{\nuiv} \|
	\\
	& \leq &
	\| \DFN^{-1} (\IFN - \IFN_{\nuiv}) \DFN^{-1} \| \,\, 
	\| \DFN \, \IFN^{-1} \DFN \| \,\, \| \DFN^{-1} \IFT_{\targv\nuiv} \HFN^{-1} \|_{\dual} \,\, \| \HFN (\nuiv - \nuivs) \|_{\nano}
	\\
	& \leq &
	\dltwunn \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, \,
	\crossnorm \, \| \HFN (\nuiv - \nuivs) \|_{\nano}.
	\qquad
\label{jufuf7yfy7tg643yrh}
\end{EQA}
This together with \eqref{4cbijjm09j9hhrjfifkrs} and \eqref{d73jejg7tre3fdy3fujell} implies
\begin{EQA}[c]
	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs + \IFN^{-1} \AUv_{\nuiv}) \|
	\leq 
	\Bigl\{ \frac{3 \crossgrad^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} \, 
	+ \crossnorm \, \dltwunn + \frac{\dltwun}{2}
	\Bigr\} \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
	\, .
\label{7tfce7sdfy7w7y73wrytk3f7}
\end{EQA}
The use of \eqref{uciuvcdiu3eoooodffcy} allows to bound
\begin{EQA}[c]
	\| \DFN^{-1} \IFN (\targv_{\nuiv} - \targvs + \IFN^{-1} \AUv_{\nuiv}) \|
	\leq
	\frac{1}{1 - \dltwbun} \, 
	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs + \IFN^{-1} \AUv_{\nuiv}) \| 
	\, ,
\label{9jjjjh3d4dd32x32sg3thj}
\end{EQA}
and \eqref{36gfijh94ejdvtwekoise} follows.
% by \( \dltwbun \leq \dltwbund \).
\end{proof}


\begin{remark}
\label{Rdmax2}
An extension to the case \( \DFN^{2} \leq \dmax^{2} \IFN \) can be done by replacing everywhere
\( \dltwu_{3} \),
\( \dltwun \),
\( \dltwunn \),
\( \dltwuns \),
\( \crossnorm \),
\( \crossgrad \) with \( \dmax^{3} \dltwu_{3} \), \( \dmax \, \dltwun \), 
\( \dmax^{2} \dltwunn \), 
\( \dmax \, \dltwuns \), 
\( \dmax^{-1} \crossnorm \), 
\( \dmax^{-1} \crossgrad \)
respectively.
\end{remark}

\Subsection{A linear perturbation}
Let \( \fn(\targv,\nuiv) \) be a linear perturbation of \( \fs(\targv,\nuiv) \):
\begin{EQA}
	\fn(\targv,\nuiv) - \fn(\targvs,\nuivs)
	&=&
	\fs(\targv,\nuiv) - \fn(\targvs,\nuivs) + \langle \AAv,\targv - \targvs \rangle + \langle \CCv,\nuiv - \nuivs \rangle ;
\label{s6cdt76ws6656ysjwsdftc6}
\end{EQA}
cf. \eqref{4hbh8njoelvt6jwgf09}.
Let also \( \Nui \) be given by \eqref{6chbdtw2hydfuguye4223w23} and \( \nuiv \in \Nui \).
We are interested in quantifying the distance between \( \targvs \) and \( \targvn_{\nuiv} \), where 
\begin{EQA}
	\targvn_{\nuiv}
	& \eqdef &
	\argmin_{\targv} \fn(\targv,\nuiv) .
\label{8dcudxjd5t6t5mkwsyddf}
\end{EQA}
The linear perturbation \( \langle \CCv,\nuiv - \nuivs \rangle \) does not depend on \( \targv \) and it can be ignored.



\begin{proposition}
\label{Pconcsupp}
For \( \nuiv \in \Nui \),
assume the conditions of Proposition~\ref{PsemiAvex} and let 
\begin{EQA}[c]
	\dltwbun \eqdef \dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} \leq 1/4 \, .
\end{EQA}
Then 
\begin{EQA}
	\| \DFN (\targvn_{\nuiv} - \targvs) \|
	& \leq &
	\frac{3 }{2(1 - \dltwbun)} \, 
	\bigl( \crossgrad \, \| \HFN (\nuiv - \nuivs) \|_{\nano} + \| \DFN^{-1} \AAv \| \bigr) 
\label{ysd7euwejfg653wthf873k}
\end{EQA}
and for any linear mapping \( \QP \), it holds with 
\( \dltwuns \) from \eqref{36gfijh94ejdvtwekoised} 
%and \( \| \HFN (\nuiv - \nuivs) \|_{\nano} = \| \HFN (\nuiv - \nuivs) \|_{\nano} \)
\begin{EQA}[l]
	\!\!\!
	\| \QP \{ \targvn_{\nuiv} - \targvs + \IFN^{-1} \IFT_{\targv\nuiv} (\nuiv - \nuivs) - \IFN^{-1} \AAv \} \|
	\\
	\leq 
	\| \QP \, \IFN^{-1} \DFN \| \, \Bigl( \dltwuns \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
		+ 2 \dltwu_{3} \, \| \DFN \, \IFN^{-1} \AAv \|^{2}
		+ \frac{4\dltwunn}{3} \, \| \DFN \, \IFN^{-1} \AAv \| \, \| \HFN (\nuiv - \nuivs) \|_{\nano}
	\Bigr)	
	\\
	\leq 
	\| \QP \, \IFN^{-1} \DFN \| \, \Bigl\{ (\dltwuns + \dltwunn) \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
		+ (2 \dltwu_{3} + \dltwunn/2) \, \| \DFN \, \IFN^{-1} \AAv \|^{2}
	\Bigr\}	
	\, .
	\qquad 
\label{usdhyw6hikhurnetr256}
\end{EQA}
\end{proposition}

\begin{proof}
%Let us fix any \( \nuiv \in \Nui \).
Proposition~\ref{PbiassemiN} applied to \( \fs_{\nuiv}(\targv) \) and 
\( \fn_{\nuiv}(\targv) = \fs_{\nuiv}(\targv) - \langle \AAv, \targv \rangle \) implies  by \eqref{uciuvcdiu3eoooodffcym}
\begin{EQA}
	\| \DFN (\targvn_{\nuiv} - \targv_{\nuiv}) \|
	& \leq &
	\frac{3}{2} \| \DFN \, \IFN_{\nuiv}^{-1} \AAv \|
	\leq 
	\frac{3}{2(1 - \dltwbun)} \| \DFN^{-1} \AAv \| 
	\, .
\label{djvhehfief6yh3jfgiu2}
\end{EQA}
This and \eqref{rhDGtuGmusGU0a2spt} imply \eqref{ysd7euwejfg653wthf873k}.
Next we check \eqref{usdhyw6hikhurnetr256} using the decomposition
\begin{EQA}
	&& \nquad
	\targvn_{\nuiv} - \targvs + \IFN^{-1} \IFT_{\targv\nuiv} (\nuiv - \nuivs) - \IFN^{-1} \AAv
	\\
	&=&
	(\targvn_{\nuiv} - \targv_{\nuiv} - \IFN_{\nuiv}^{-1} \AAv) 
	+ (\IFN_{\nuiv}^{-1} \AAv - \IFN^{-1} \AAv)
	+ \{ \targv_{\nuiv} - \targvs + \IFN^{-1} \IFT_{\targv\nuiv} (\nuiv - \nuivs) \} 
	\, .
\label{yhdt56swhew454erjhfgi}
\end{EQA}
Proposition~\ref{PsemiAvex} evaluates the last term.
Lemma~\ref{L3IFNNui} helps to bound
\begin{EQA}
	\| \DFN^{-1} \IFN (\IFN_{\nuiv}^{-1} - \IFN^{-1}) \IFN_{\nuiv} \, \DFN^{-1} \|
	& = &
	\| \DFN^{-1} (\IFN_{\nuiv} - \IFN) \DFN^{-1} \|
	\leq 
	\dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} 
	\, .
\label{cuyedgfcuedgtfbvj}
\end{EQA}
This yields 
\begin{EQA}
	\| \QP (\IFN_{\nuiv}^{-1} - \IFN^{-1}) \AAv \|
	& \leq &
	\| \QP \, \IFN^{-1} \DFN \| 
	\, \| \DFN^{-1} \IFN_{\nuiv} (\IFN_{\nuiv}^{-1} - \IFN^{-1}) \IFN \, \DFN^{-1} \|
	\, \| \DFN \, \IFN_{\nuiv}^{-1} \AAv \|
	\\
	& \leq &
	\| \QP \, \IFN^{-1} \DFN \| 
	\, \dltwunn \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \,
	\, \frac{1}{1 - \dltwbun} \| \DFN \, \IFN^{-1} \AAv \|
	\, .
\label{7duewjf87he4fyjwucyfne}
\end{EQA}
Moreover, 
for \( \epsv_{\nuiv} \eqdef \targvn_{\nuiv} - \targv_{\nuiv} - \IFN_{\nuiv}^{-1} \AAv \), it holds
\begin{EQA}
	\| \DFN^{-1} \IFN_{\nuiv} \, \epsv_{\nuiv} \|
	& \leq &
	\frac{3 \dltwu_{3}}{4} \| \DFN \, \IFN_{\nuiv}^{-1} \AAv \|^{2}  
	\leq 
	\frac{3 \dltwu_{3}}{4(1 - \dltwbun)^{2}} \| \DFN \, \IFN^{-1} \AAv \|^{2}
	\, ,
\label{ud82uegkftryyde6ewhde}
\end{EQA} 
and by \eqref{uciuvcdiu3eoooodffcym} and \( \dltwbun \leq 1/4 \)
\begin{EQA}
	\| \QP \, \epsv_{\nuiv} \|
	& \leq &
	\| \QP \, \IFN^{-1} \DFN \| \,\, \| \DFN^{-1} \IFN \, \epsv_{\nuiv} \|
	\leq 
	\| \QP \, \IFN^{-1} \DFN \| \, \frac{1 - \dltwbun}{1 - 2 \dltwbun} \, \| \DFN^{-1} \IFN_{\nuiv} \, \epsv_{\nuiv} \|
	\\
	& \leq &
	\| \QP \, \IFN^{-1} \DFN \| \,\, 
	\frac{3 \dltwu_{3}}{4(1 - \dltwbun) (1 - 2 \dltwbun)} \| \DFN \, \IFN^{-1} \AAv \|^{2} 
	\leq 
	\| \QP \, \IFN^{-1} \DFN \| \, 2 \dltwu_{3} \, \| \DFN \, \IFN^{-1} \AAv \|^{2}
	\, .
\label{ysdudhwuw8ey87wejue4bf}
\end{EQA}
The obtained bounds imply \eqref{usdhyw6hikhurnetr256} in view of
\( (4/3)ab \leq a^{2} + b^{2}/2 \) for any \( a,b \).
\end{proof}

\begin{comment}
\Subsection{One-point orthogonality by a linear transform}
\label{Sonepointtrans}
\emph{One-point orthogonality} condition means \( \nabla_{\nuiv} \nabla_{\targv} \, \fs(\prmtvs) = 0 \).
This section explains how
this condition can be enforced for a general function \( \fs \) by 
a linear transform of the nuisance parameter.
We only need a mild \emph{separability condition} which 
assumes that the full-dimensional information matrix
\( \IFT(\prmtv) = \nabla^{2} \fs(\prmtv) \) is well posed
%can be bounded from below by the block-diagonal matrix 
%\( \blk\{ - \nabla_{\targv\targv}^{2} \fs(\prmtv), - \nabla_{\nuiv\nuiv}^{2} \fs(\prmtv) \} \)
for \( \prmtv = \prmtvs \).

\begin{description}
	\item[\label{IFLref} \( \bb{(\IFT)} \)]
	\emph{%The function \( \fs(\prmtv) \) is strongly convex. 
	The matrix \( \IFT = \IFT(\prmtvs) \) is positive definite 
	and for some constant \( \rhoIF = \rhoIF(\IFT) < 1 \)} % and \( \prmtv = \prmtvs \), it holds}
\begin{EQA}
	\| 
	\IFT_{\targv\targv}^{-1/2} \IFT_{\targv\nuiv} \, \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} \, \IFT_{\targv\targv}^{-1/2} 
	\|
	& \leq &
	\rhoIF^{2}
	< 
	1 .
\label{vcjcfvedt7wdwhesqgghwqLco}
\end{EQA}
\end{description}


\begin{lemma}
\label{Lidentsemi}
Suppose \nameref{IFLref}. 
Then with \( \IFTN \eqdef \blk\{ \IFT_{\targv\targv},\IFT_{\nuiv\nuiv} \} \)
\begin{EQA}
	(1 - \rhoIF) \IFTN
	\leq 
	\IFT
	& \leq &
	(1 + \rhoIF) \IFTN
\label{f6eh3ewfd6ehev65r43tre}
\end{EQA}
and the matrices
\begin{EQA}
	\IFTb_{\targv\targv} 
	& \eqdef &
	\IFT_{\targv\targv} - \IFT_{\targv\nuiv} \, \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} \, ,
	\qquad
	\IFTb_{\nuiv\nuiv}
	\eqdef 
	\IFT_{\nuiv\nuiv} - \IFT_{\nuiv\targv} \, \IFT_{\targv\targv}^{-1} \, \IFT_{\targv\nuiv} \, ,
	\qquad
\label{ljhy6furf4rfeder8jfu8rd}
\end{EQA}
satisfy
\begin{EQA}
	(1 - \rhoIF^{2}) \, \IFT_{\targv\targv}
	\leq 
	\IFTb_{\targv\targv}
	& \leq &
	\IFT_{\targv\targv} \, ,
	\qquad
	(1 - \rhoIF^{2}) \, \IFT_{\nuiv\nuiv}
	\leq 
	\IFTb_{\nuiv\nuiv}
	\leq 
	\IFT_{\nuiv\nuiv} \, .
\label{yg3w5dffctvyry4r7er7dgfe}
\end{EQA}
\end{lemma}

\begin{proof}
Define \( \DFN^{2} = \IFT_{\targv\targv} \), \( \HFN^{2} = \IFT_{\nuiv\nuiv} \),
\( \IFTN = \blk\{ \DFN^{2},\HFN^{2} \} \), \( \AFN = \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1} \), and consider the matrix 
\begin{EQA}
	\IFTN^{-1/2} \IFT \, \IFTN^{-1/2} - \Id_{\dimttl}
	&=&
	\begin{pmatrix}
		0 & \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1}
		\\
		\HFN^{-1} \IFT_{\nuiv\targv} \, \DFN^{-1} & 0
	\end{pmatrix}
	=
	\begin{pmatrix}
		0 & \AFN
		\\
		\AFN^{\T} & 0
	\end{pmatrix} .
\label{gswrew35e35e35e5txzgtqw}
\end{EQA}
Condition \eqref{vcjcfvedt7wdwhesqgghwqLco} implies \( \| \AFN \AFN^{\T} \| \leq \rhoIF^{2} \) and hence,
\begin{EQA}
	- \rhoIF \, \Id_{\dimttl} 
	& \leq &
	\IFTN^{-1/2} \IFT \, \IFTN^{-1/2} - \Id_{\dimttl} 
	\leq 
	\rhoIF \, \Id_{\dimttl} \, .
\label{ye376evhgder52wedsytg}
\end{EQA}
Moreover,
\begin{EQA}
	\IFTb_{\targv\targv} 
	& = &
	\IFT_{\targv\targv} - \IFT_{\targv\nuiv} \, \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} 
	=
	\DFN (\Id_{\dimp} - \AFN \AFN^{\T}) \DFN 
	\geq 
	(1 - \rhoIF^{2}) \DFN^{2} \, ,
\label{ljhy6furf4jfu8rdfcweerdd}
\end{EQA}
and similarly for \( \IFTb_{\nuiv\nuiv} \).
\end{proof}

\noindent
Note that \( \DFN^{2} = \IFT_{\targv\targv} \) is the \( \targv\targv \)-block of \( \IFT = \nabla^{2} \fs(\prmtvs) \), while 
\( \DFNb^{-2} \eqdef \IFTb_{\targv\targv}^{-1} \) from \eqref{ljhy6furf4rfeder8jfu8rd} 
is the \( \targv\targv \)-block of \( \IFT^{-1} \)
by the formula of block-inversion.
The matrices \( \DFN^{2} \) and \( \DFNb^{2} \) only coincide if the matrix \( \IFT \) is of block-diagonal structure.

\begin{lemma}
\label{Onepointorto}
%
With block representation \eqref{hwe78yf2diwe76tfw67etfwtbso},
define \( \CFT = \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} \) and
\begin{EQ}[rcl]
	\nuov 
	&=& 
	\nuiv + \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} \, (\targv - \targvs) 
	=
	\nuiv + \CFT \, (\targv - \targvs) ,
	\\
	\fsb(\targv,\nuov)
	&=&
	\fs(\targv,\nuiv) 
	=
	\fs(\targv,\nuov - \CFT \, (\targv - \targvs)) .
\label{0vcucvf653nhftdreyenwe}
\end{EQ}
Then 
\begin{EQA}
	\nabla_{\nuov} \nabla_{\targv} \, \fsb(\targv,\nuov) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}}
	&=&
	0 \, ,
	\quad
%\label{jdgyefe74erjscgygfydhw}
	\nabla_{\targv\targv}^{2} \, \fsb(\targv,\nuov) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}} 
	=
	\DFNb^{2} \, ,
	\quad
	\nabla_{\nuov\nuov}^{2} \, \fsb(\targv,\nuov) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}} 
	=
	\HFN^{2} 
	 \, .
	 \qquad
\label{n6d2fgujrt6fgfrjrd}
\end{EQA}
\end{lemma}

\begin{proof}
By definition \( \fs(\targv,\nuiv) = \fs(\targv,\nuov - \CFT \, \targv) \), and it is straightforward to check that
\begin{EQA}
	\nabla_{\nuov} \nabla_{\targv} \, \fsb(\targv,\nuov) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}}
%	_{\targv=\targvs,\nuov=\nuivs}
	=
	\nabla_{\nuov} \nabla_{\targv} \, \fs(\targv,\nuov 
	- \CFT \, (\targv - \targvs)) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}} 
	&=&
	0 .
	\qquad
\label{jdgyefe74erjscgygfydhwp}
\end{EQA}
Similarly
\begin{EQA}
	\nabla_{\targv\targv}^{2} \, \fsb(\prmtvs) 
	=
	\nabla_{\targv\targv}^{2} \, \fs(\targv,\nuov - \CFT \, (\targv - \targvs)) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}}
	&=&
	\IFT_{\targv\targv} - \IFT_{\targv\nuiv} \, \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} 
	=
	\DFNb^{2} \, 
\label{d3gr7hyrfygieshfdhfjk}
\end{EQA}
and \( \nabla_{\nuov\nuov}^{2} \, \fsb(\prmtvs) = \nabla_{\nuiv\nuiv}^{2} \, \fs(\prmtvs) = \HFN^{2} \)
as required.
\end{proof}


%Note that \( \DFNb^{-2} \) is the \( \targv\targv \)-block of \( \IFT^{-1} \) by the formula of block-inversion.
We can summarize that the linear transform \eqref{0vcucvf653nhftdreyenwe} ensures the one-point orthogonality
condition \( \nabla_{\nuov} \nabla_{\targv} \, \fsb(\prmtvs) = 0 \) for the function 
\( \fsb(\targv,\nuov) = \fs(\targv,\nuov - \cc{C} \, (\targv - \targvs)) \) with 
\( - \nabla_{\targv\targv}^{2} \fsb(\prmtvs) = \DFNb^{2} \).
For this function, one can redefine all the characteristics including
\begin{EQA}
	\breve{\feta}_{\nuov}
	& \eqdef &
	\max_{\targv} \fsb(\targv,\nuov),
	\\
	\targvb_{\nuov}
	& \eqdef &
	\argmin_{\targv} \fsb(\targv,\nuov),
	\\
	\DFNb_{\nuov}^{2}
	& \eqdef &
	- \nabla_{\targv\targv}^{2} \fsb(\targvb_{\nuov},\nuov). 
\label{nfyehendcghegwdgqgqngd}
\end{EQA}
If \( \fs(\targv,\nuiv) \) is quadratic, then orthogonality can be achieved by a linear transform of the nuisance parameter \( \nuiv \).
In particular, for \( \fs(\prmtv) = \fs(\prmtvs) - (\prmtv - \prmtvs)^{\T} \IFT \, (\prmtv - \prmtvs)/2 \) quadratic, it holds with 
\( \HFN^{2} = \IFT_{\nuiv\nuiv} \)
\begin{EQA}
	\fsb(\targv,\nuov)
	&=&
	\fs(\prmtvs) - \frac{\| \DFNb (\targv - \targvs) \|^{2}}{2}  - \frac{\| \HFN (\nuov - \nuivs) \|^{2}}{2}  \, ,
\label{ovjv8734mfdgdytwndbgg}
\end{EQA}
and hence
\begin{EQA}
	\targvb_{\nuov}
	& \equiv &
	\targvs,
	\qquad
	\DFNb_{\nuov}^{2}
	\equiv 
	\DFNb^{2} ,
	\qquad
	\breve{\feta}_{\nuov}
	=
	- \frac{\| \HFN (\nuov - \nuivs) \|^{2}}{2} \, .
\label{lfibubgue5t335r6tt7ehw}
\end{EQA}

%\Subsection{Semiorthogonality}

For a general smooth function \( \fs(\prmtv) = \fs(\targv,\nuiv) \) satisfying \nameref{LLsT3ref}, 
we expect that these identities are fulfilled
in a local vicinity of \( \prmtvs \) up to the error of quadratic approximation.
The next result quantifies this guess.

\begin{proposition}
\label{PonepptLL}
Let \( \fs(\prmtv) \) satisfy \nameref{IFLref}, \nameref{LLsT3ref}, and
\begin{EQA}[c]
	(1 - \rhoIF)^{-1} \, \dltwu_{3} \, \rr
	\leq 
	1/3 .
\label{8uiiihkkcrdrdteggcjcjdan}
\end{EQA} 
Then for any \( \nuov \) with \( \| \HFN (\nuov - \nuovs) \| \leq \rr \) and any linear mapping 
\( \QP \colon \R^{\dimp} \to \R^{\dimq} \), the bias \( \targvb_{\nuov} - \targvs \) satisfies
with \( \DFNb^{2} = \IFTb_{\targv\targv} \) from \eqref{ljhy6furf4rfeder8jfu8rd} 
\begin{EQA}
	\| \QP (\targvb_{\nuov} - \targvs) \|
	& \leq &
	\| \QP \, \DFNb^{-1} \| \, \frac{(1 + \dltwu_{3} \, \rr/2)}{2(1 - \dltwu_{3} \, \rr)} \, \dltwu_{3} \, \| \HFN (\nuov - \nuovs) \|^{2} \, .
\label{36gfijh94ejdvtwekoib}
\end{EQA}
In particular, with \( \QP = \DFNb \)
\begin{EQA}
	\| \DFNb (\targvb_{\nuov} - \targvs) \|
	& \leq &
	\frac{(1 + \dltwu_{3} \, \rr/2)}{2(1 - \dltwu_{3} \, \rr)} \, \dltwu_{3} \, \| \HFN (\nuov - \nuovs) \|^{2} \, .
\label{36gfijh94ejdvtwekoDL}
\end{EQA}
\end{proposition}

\begin{proof}
Linear transform \eqref{0vcucvf653nhftdreyenwe} reduces the proof 
to the case with one-point orthogonality. 
Condition \nameref{LLsT3ref} still applies with the same constant \( \dltwu_{3} \).
Condition \eqref{8uiiihkkcrdrdteggcjcjdan} ensures \nameref{LLsoT3ref}, \nameref{LLpT3ref} after
this transform, and the result follows from Proposition~\ref{PsemiAv}.
\end{proof}
\end{comment}


%\Subsection{Semiorthogonality}
%
%This section discusses a special case when the mixed derivative of 
%\( \fs(\targv,\nuiv) \) only depends on \( \targv \):
%\begin{EQA}
%	\nabla_{\nuiv} \nabla_{\targv} \fs(\targv,\nuiv)
%	& \equiv &
%	- \dCross(\targv) ,
%	\qquad
%	\nabla_{\nuiv\nuiv}^{2} \fs(\targv,\nuiv)
%	\equiv 
%	- \dPartial^{2}(\targv),
%\label{0hy533rycirudle}
%\end{EQA}
%for a \( \dimq \times \dimp \)-matrix function \( \dCross(\targv) \) and a positive \( \dimq \times \dimq \)-matrix function 
%\( \dPartial^{2}(\targv) \).
%We also write \( \dCross \) and \( \dPartial^{2} \) in place of \( \dCross(\targvs) \) and \( \dPartial^{2}(\targvs) \).
%Due to the next result, this condition yields a semi-orthogonality of the transformed function \( \fsb(\cdot) \).
%
%\begin{lemma}
%\label{LCrossdervs}
%Assume \eqref{0hy533rycirudle}.
%Then the function \( \fsb(\targv,\nuov) \) from \eqref{0vcucvf653nhftdreyenwe} satisfies the semi-orthogonality condition 
%\begin{EQA}
%	\nabla_{\nuov} \nabla_{\targv} \fsb(\targvs,\nuov)
%	& \equiv &
%	0.
%\label{juifue36fhg65e3yeh}
%\end{EQA}
%Moreover, %with \( \DFNb^{2} = - \nabla_{\targv\targv}^{2} \fsb(\targvs,\nuivs) =  \)
%for any \( \nuov \) with \( (\targvs,\nuov) \in \Upsb \), it holds
%\begin{EQA}[rcccl]
%	\nabla_{\targv} \fsb(\targvs,\nuov)
%	& \equiv &
%	0,
%	\qquad
%	\nabla_{\targv\targv}^{2} \fsb(\targvs,\nuov)
%	& \equiv &
%	\nabla_{\targv\targv}^{2} \fsb(\targvs,\nuivs) .
%\label{klfu87fjhr57765645r}
%\end{EQA}
%If \( \fs(\prmtv) \) is convex in \( \prmtv \) then 
%\begin{EQA}
%	\targvb_{\nuov}
%	& \eqdef &
%	\argmin_{\targv} \fsb(\targv,\nuov)
%	\equiv 
%	\targvs \, .	
%\label{juifue36fhg65e3yehop}
%\end{EQA}
%%and
%%\begin{EQA}
%%	\targv_{\nuiv}
%%	\eqdef
%%	\argmin_{\targv} \fs(\targv,\nuiv)
%%	& \equiv &
%%	\targvs \, .
%%\label{juifue36fhg65e3yehopb}
%%\end{EQA}
%\end{lemma}
%
%\begin{proof}
%Let \( \fsb(\targv,\nuov) \) be defined by \eqref{0vcucvf653nhftdreyenwe}.
%Lemma~\ref{Onepointorto} ensures one-point orthogonality 
%\( \nabla_{\nuov} \nabla_{\targv} \fsb(\prmtvs) = \nabla_{\nuov} \nabla_{\targv} \fsb(\targvs,\nuivs) = 0 \).
%Moreover, \eqref{0hy533rycirudle} yields \( \CFT = \dPartial^{-2} \, \dCross \).
%Now consider \( \nabla_{\nuov} \nabla_{\targv} \fsb(\targvs,\nuov) \).
%It holds by \eqref{0hy533rycirudle} and definition \eqref{0vcucvf653nhftdreyenwe}
%\begin{EQA}
%	\nabla_{\nuov} \nabla_{\targv} \fsb(\targvs,\nuov) 
%	&=&
%	\nabla_{\nuov} \nabla_{\targv} \fs(\targv,\nuov - \CFT \, (\targv - \targvs)) \bigg|_{\targv = \targvs}
%	\\
%	&=&
%	\nabla_{\nuov} \nabla_{\targv} \fs(\targvs,\nuov) - \nabla_{\nuov}^{2} \fs(\targvs,\nuov) \CFT
%	=
%	- \dCross + \dPartial^{2} \CFT
%	=
%	0
%\label{ucieruier3dchedndm}
%\end{EQA}
%yielding semi-orthogonality of \( \fsb \).
%Lemma~\ref{Lsemiorto} implies \eqref{klfu87fjhr57765645r} and \eqref{juifue36fhg65e3yehop}.
%\end{proof}
%
%


\Section{Sup-norm expansions for linearly perturbed optimization}
\label{Ssupnormco}
Let \( \fs(\upsv) \) be a convex function and \( \upsvs = \argmin_{\upsv} \fs(\upsv) \).
Define \( \IFT = \nabla^{2} \fs(\upsvs) = (\IFT_{jm}) \).
Let also \( \fn(\upsv) \) be obtained by a linear perturbation of \( \fs(\upsv) \) as in \eqref{4hbh8njoelvt6jwgf09}
and let \( \upsvn = \argmin_{\upsv} \fn(\upsv) \).
We intend to bound the corresponding change \( \upsvn - \upsvs \) in a sup-norm.
The strategy of the study is to fix one component \( \ups_{j} \) of \( \upsv \) and treat the remaining entries as the nuisance 
parameter.
Fix a metric tensor \( \DFN \) in diagonal form:
\begin{EQA}[c]
	\DFN \eqdef \diag(\DFN_{1}, \ldots, \DFN_{\dimp}).
\label{7dycf8mwdy6ey43hf98yh}
\end{EQA}
Later we assume \( \DFN_{j}^{2} = \IFT_{jj} \).
For each \( j \leq \dimp \), we will use the representation \( \upsv = (\ups_{j},\nuiv_{j}) \), where 
\( \nuiv_{j} \in \R^{\dimp-1} \) collects all the remaining entries of \( \upsv \).
Similarly, define \( \DFN = (\DFN_{j},\HFN_{j}) \) with \( \HFN_{j} = \diag(\DFN_{m}) \) for \( m \neq j \).
%
Define also for some radius \( \rrinf \)
\begin{EQA}[c]
	\Upsd = \{ \upsv \colon \| \DFN (\upsv - \upsvs) \|_{\infty} \leq \rrinf \} 
	=
	\Bigl\{ \upsv \colon \max_{j \leq \dimp} \bigl| \DFN_{j} (\ups_{j} - \upss_{j}) \bigr| 
	\leq \rrinf \Bigr\}.
\label{du7duydy7cy6fc6df3}
\end{EQA}
%Also, for each \( j \leq \dimp \), define
%\begin{EQA}
%	\Nuid_{j}
%	& \eqdef &
%	\bigl\{ \nuiv_{j} \colon \| \HFN_{j}(\nuiv_{j} - \nuivs_{j}) \|_{\infty} \leq \rrinf \bigr\} \, .
%\label{6xdycyvtv544e4seg3df}
%\end{EQA}
Assume the following condition.

\begin{description}
    \item[\label{LLpsupref} \( \bb{(\mathcal{T}_{\infty}^{*})} \)]
      \emph{For each \( j \leq \dimp \), 
     the function \( \fs(\ups_{j},\nuiv_{j}) \) fulfills}
%   \item[\label{LLpsup3ref} \( \bb{(\mathcal{T}_{3,\infty}^{*})} \)]
%      \emph{For each \( j \leq \dimp \), 
%      }
\begin{EQA}[rcl]
	\sup_{\nuiv_{j} \colon \| \HFN_{j} (\nuiv_{j} - \nuivs_{j}) \|_{\infty} \leq \rrinfi} \,\, 
	\sup_{\ups \colon \DFN_{j} |\ups - \upss_{j}| \leq 2\rrinfi} \,
	\frac{\bigl| \nabla_{\ups_{j}\ups_{j} \ups_{j}}^{(3)} \fs(\ups_{j},\nuiv_{j}) \bigr|}
		 {\DFN_{j}^{3}}
	& \leq &
	\dltwu_{3} \, ,
\label{d6f53ye5vry4fddfgsup}
\end{EQA}
\emph{and}
\begin{EQA}[lccl]
	\sup_{\upsv = (\upss_{j},\nuiv_{j}) \in \Upsd} \,
	\sup_{\zv_{j} \in \R^{\dimp-1}} \,
	&
	\frac{| \langle \nabla_{\ups_{j}\ups_{j}\nuiv_{j}}^{(3)} \fs(\upss_{j},\nuiv_{j}), \zv_{j} \rangle |}
		 {\DFN_{j}^{2} \, \| \HFN_{j} \zv_{j} \|_{\infty}}
	& \leq &
	\dltwunn 
	\, ,
\label{c6hyi8ietctwhcsup}
	\\
	\sup_{\upsv = (\upss_{j},\nuiv_{j}) \in \Upsd}  \,
	\sup_{\zv_{j} \in \R_{j}^{\dimp}} \,
	&
	\frac{| \langle \nabla_{\ups_{j}\nuiv_{j}\nuiv_{j}}^{3} \fs(\upss_{j},\nuiv_{j}), \zv_{j}^{\otimes 2} \rangle |}
		 {\DFN_{j} \, \| \HFN_{j} \zv_{j} \|_{\infty}^{2}}
	& \leq &
	\dltwun 
	\, .
	\qquad
\label{c6ceyecc5e5etcT2sup}
\end{EQA}
\end{description}

For the dual norm \( \| \cdot \|_{\dual} \) from \eqref{ygtuesdfhiwdsoif9ruta}, define
\begin{EQA}
	\crosssup
	& \eqdef &
	\max_{j = 1,\ldots,\dimp} \| \DFN_{j}^{-1} \IFT_{\ups_{j},\nuiv_{j}} \, \HFN_{j}^{-1} \|_{\dual} 
	=
	\max_{j = 1,\ldots,\dimp} \,\, \sup_{\| \zv \|_{\infty} \leq 1}
	\| \DFN_{j}^{-1} \IFT_{\ups_{j},\nuiv_{j}} \, \HFN_{j}^{-1} \zv \|
	\, .
	\qquad
\label{7tdsyf8iuwopkrtg4576}
\end{EQA}

\begin{lemma}
\label{Lcrosssup}
It holds
\begin{EQA}[c]
	\crosssup^{2}
	\leq 
	\max_{j = 1,\ldots,\dimp} \frac{1}{\DFN_{j}^{2}}
	\sum_{m \neq j} \frac{\IFT_{jm}^{2}}{\DFN_{m}^{2}} \, .
\end{EQA}
\end{lemma}

\begin{proof}
By definition,
\begin{EQA}[rcl]
	\crosssup^{2}
	& \leq &
	\max_{j = 1,\ldots,\dimp} \,\, \sup_{\| \zv \|_{\infty} \leq 1}
	\sum_{m \neq j} \frac{1}{\DFN_{j}^{2} \, \DFN_{m}^{2}} \, \IFT_{jm}^{2} z_{m}^{2} 
	\leq 
	\max_{j = 1,\ldots,\dimp} \frac{1}{\DFN_{j}^{2}}
	\sum_{m \neq j} \frac{\IFT_{jm}^{2}}{\DFN_{m}^{2}} \,  
\end{EQA}
as claimed.
\end{proof}
%
It is mandatory for the proposed approach that \( \crosssup < 1 \).
% and \( \dltwbun = \dltwunn \, \rrinf < 1 \).
%Moreover, some of results including the final expansion \eqref{usdhyw6hikhurnetrspp2} assume that \( \crosssup \) is small.
%The value \( \dltwuns \) from \eqref{36gfijh94ejdvtwekoised} can be specified as
The next result provides an upper bound on \( \| \upsvd - \upsvs \|_{\infty} \).


\begin{proposition}
\label{Psemibiassup}
Let \( \fs(\upsv) \) be convex function and 
\( \fn(\upsv) \) be a linear perturbation of \( \fs(\upsv) \) with a vector \( \AAv \). 
For a diagonal metric tensor \( \DFN \), assume \( \crosssup < 1 \); see \eqref{7tdsyf8iuwopkrtg4576}. 
Fix 
\begin{EQA}
	\rrinf 
	&=& 
	\frac{\sqrt{2}}{1 - \crosssup} \| \DFN^{-1} \AAv \|_{\infty} 
	\, .
\label{8drywjwuycrt5sdeteyhfuwk}
\end{EQA}
Let \nameref{LLpsupref} hold with this \( \rrinf \) and
\( \dltwun, \dltwunn, \dltwu_{3} \) satisfying  
\begin{EQA}[c]
	\dltwbun = \dltwunn \, \rrinf \leq 1/4 ,
	\qquad
	\dltwun \, \rrinf \leq 1/4 \, ,
	\qquad	
	\dltwunss \| \DFN^{-1} \AAv \|_{\infty} 
	\leq 
	\sqrt{2} - 1
	\, ,
\label{dhfiejfowelocuyehbrf}
\end{EQA}
where
\begin{EQA}[rcl]
	\dltwuns
	& \eqdef &
	\frac{1}{1 - \dltwbun} \, 
	\biggl( \crosssup \, \dltwunn + \frac{\dltwun}{2}
		+ \frac{3(\crosssup + \dltwbun/2)^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} 
%		+ \frac{3\dltwu_{3}\, \dltwun^{2} \, \rru^{2}}{4(1 - \dltwbund)^{2}} 
	\biggr) 
	\, ,
\label{36gfijh94ejdvtwekoisedi}
	\\
	\dltwunss
	& \eqdef &
	2 \dltwu_{3} + \frac{\dltwunn}{2}  + \frac{2(\dltwuns + \dltwunn)}{(1 - \crosssup)^{2}} 
	\, .
\end{EQA}
Then \( \upsvd = \argmin_{\upsv} \fn(\upsv) \) satisfies
\begin{EQA}
	\| \DFN (\upsvd - \upsvs) \|_{\infty}
	\eqdef
	\max_{j \leq \dimp} | \DFN_{j} (\upsd_{j} - \upss_{j}) |
	& \leq &
	\rrinf \, .
\label{7ytdufchskmls7rghnk}
\end{EQA} 
Furthermore, 
\begin{EQA}
\label{usdhyw6hikhurnetrspp}
	\bigl\| \DFN^{-1} \bigl\{ \IFT (\upsvd - \upsvs) - \AAv \bigr\} \bigr\|_{\infty}
	& \leq &
	\dltwunss \, \| \DFN^{-1} \AAv \|_{\infty}^{2} 
	\, ,
	\\
	\bigl\| \DFN (\upsvd - \upsvs - \IFT^{-1} \AAv) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}^{2} 
	\, ,
	\qquad
\label{usdhyw6hikhurnetrspp1}
\end{EQA}
and with \( \Delta \eqdef \Id_{\dimp} - \DFN^{-1} \IFT \, \DFN^{-1} \)
\begin{EQ}[rcl]
	\bigl\| \DFN (\upsvd - \upsvs) - \DFN^{-1} \AAv) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}^{2} + \frac{\crosssup}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}
	\, ,
	\\
	\bigl\| \DFN (\upsvd - \upsvs) - (\Id_{\dimp} + \Delta) \DFN^{-1} \AAv) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}^{2} + \frac{\crosssup^{2}}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}
	\, .
	\qquad
\label{usdhyw6hikhurnetrspp2}
\end{EQ}
\end{proposition}


\begin{remark}
To gain an intuition about the result of the proposition, consider a typical situation with 
\( \dltwun \leq \dltwu_{3} \),
\( \dltwunn \leq \dltwu_{3} \),
\( \dltwbun \leq 1/4 \),
\( 1 - \crosssup \leq 1/\sqrt{2} \).
Then \( \dltwuns \) from \eqref{36gfijh94ejdvtwekoisedi} fulfills \( \dltwuns \leq 1.37 \), and it holds
\( \dltwunss \leq 12 \dltwu_{3} \).
\end{remark}



\begin{proof}
Let us fix any \( j \leq \dimp \), e.g. \( j=1 \).
Represent any \( \upsv \in \Upsd \) as \( \upsv = (\ups_{1},\nuiv_{1}) \), where \( \nuiv_{1} = (\ups_{2},\ldots,\ups_{\dimp})^{\T} \). 
%Define \( \Nuid_{1} = \{ \nuiv_{1} \colon  \max_{j\geq 2} \| \DFN_{j} \ups_{j} \| \leq \rrinf \} \).
By \eqref{7tdsyf8iuwopkrtg4576}
\begin{EQA}
	&& \nquad
	\bigl| \DFN_{1} \IFT_{11}^{-1} \IFT_{\ups_{1}\nuiv_{1}}(\nuiv_{1} - \nuivs_{1}) \bigr|
	\leq 
	\bigl| \DFN_{1}^{-1} \IFT_{\ups_{1}\nuiv_{1}}(\nuiv_{1} - \nuivs_{1}) \bigr|
	\leq 
	\crosssup \, \| \HFN_{1} (\nuiv_{1} - \nuivs_{1}) \|_{\infty}
%	\\
%	& \leq &
%	\sum_{m=2}^{\dimp} \frac{|\IFT_{1m}|}{\DFN_{1} \DFN_{m}} \bigl| \DFN_{m} (\ups_{m} - \upss_{m}) \bigr|
%	\leq 
%	\crosssup \, \max_{m=2,\ldots,\dimp} \bigl| \DFN_{m} (\ups_{m} - \upss_{m}) \bigr|
	\, .
\label{dekweivytre34wfgbc}
\end{EQA}
For any \( \nupv_{1} \), define
\begin{EQA}
	\upsd_{1}(\nupv_{1})
	& \eqdef &
	\argmin_{\ups_{1}} \fn(\ups_{1},\nupv_{1}) .
\label{fifwi9jhrio3jiofcwgyt7we}
\end{EQA}
Now we apply Proposition~\ref{Pconcsupp} 
with \( \QP = \DFN_{1} \), \( \IFN = \IFT_{11} \), \( \HFN = \HFN_{1} = \diag(\DFN_{2},\ldots,\DFN_{\dimp}) \),
and \( \| \HFN_{1} (\nuiv_{1} - \nuivs_{1}) \|_{\infty} \leq \rrinf \).
%using 
%\( \IFT_{\targv\nuiv} (\nuiv - \nuivs) = \Delta_{1} \) and 
%\( \| \HFN (\nuiv - \nuivs) \|_{\nano} \leq \| \DFN (\upsv - \upsvs) \|_{\infty} \leq \rrinf \).
As \( \DFN_{1} \IFT_{11}^{-1} \leq \DFN_{1}^{-1} \), bound \eqref{usdhyw6hikhurnetr256} yields
\begin{EQA}
	&& \nquad
	\bigl| \DFN_{1} \{ \upsd_{1}(\nuiv_{1}) - \upss_{1} - \IFT_{11}^{-1} \AAv_{1} + \IFT_{11}^{-1} \IFT_{\ups_{1}\nuiv_{1}}(\nuiv_{1} - \nuivs_{1}) \} \bigr|
	\\
	& \leq &
	(\dltwuns + \dltwunn) \, \| \HFN_{1} (\nuiv_{1} - \nuivs_{1}) \|_{\nano}^{2}
		+ \bigl(2 \dltwu_{3} + \frac{\dltwunn}{2} \bigr) \, \DFN_{1}^{-2} \AAv_{1}^{2}
	\\
	& \leq &
	(\dltwuns + \dltwunn) \rrinf^{2} + \bigl(2 \dltwu_{3} + \frac{\dltwunn}{2} \bigr) \, \| \DFN^{-1} \AAv \|_{\infty}^{2} 
	=
	\dltwunss \, \| \DFN^{-1} \AAv \|_{\infty}^{2} 
	\, .
	\qquad
\label{usdhyw6hikhurnetr256sup}
\end{EQA}
This, \eqref{dekweivytre34wfgbc}, and \eqref{dhfiejfowelocuyehbrf} imply by \( \rrinf = \cmax \| \DFN^{-1} \AAv \|_{\infty} \)
and \( \cmax = \sqrt{2}/(1 - \crosssup) \)
\begin{EQA}
	\bigl| \DFN_{1} \{ \upsd_{1}(\nupv) - \upss_{1} \} \bigr|
	& \leq &
	\| \DFN^{-1} \AAv \|_{\infty} + \crosssup \, \rrinf
	+ \dltwunss \, \| \DFN^{-1} \AAv \|_{\infty}^{2}
	\\
	& \leq &
	\bigl( 1 + \cmax \, \crosssup + \sqrt{2} - 1 \bigr) \| \DFN^{-1} \AAv \|_{\infty}
	=
	\cmax \| \DFN^{-1} \AAv \|_{\infty}
	= 
	\rrinf \, .
\label{7deje8vg7g76gvgv5f43w}
\end{EQA}
The same bounds apply to each \( j \leq \dimp \).
Therefore, when started from any point \( \upsv \in \Upsd \), the sequential optimization procedure 
which maximizes the objective function w.r.t. one coordinate while keeping all the remaining coordinates
has its solution within \( \Upsd \).
As the function \( \fs \) is strongly convex, and its value improves at every step, the procedure converges to a unique solution \( \upsvd \in \Upsd \).
This implies \eqref{7ytdufchskmls7rghnk}.
Further, with \( \upsv = \upsvd \), 
\begin{EQA}
	\IFT_{11} \{ \ups_{1}(\nuiv_{1}) - \upss_{1} \} + \IFT_{\ups_{1}\nuiv_{1}}(\nuiv_{1} - \nuivs_{1})
	&=&
	\IFT (\upsvd - \upsvs) 
	\, .
\label{tdtdtd6tf78gf98ggt}
\end{EQA}
This yields \eqref{usdhyw6hikhurnetrspp}.
Moreover, with \( \uv \eqdef \DFN (\upsvd - \upsvs) \) and \( B \eqdef \DFN^{-1} \IFT \, \DFN^{-1} \), it holds
\begin{EQA}
	\DFN^{-1} \bigl\{ \IFT (\upsvd - \upsvs) - \AAv \bigr\} 
	&=&
	B (\uv - \DFN \, \IFT^{-1} \AAv) \, ,
\label{fi8fu7v7y6vyv44v3eged}
\end{EQA}
and by \eqref{usdhyw6hikhurnetrspp} and Lemma~\ref{LinvGersh} 
\begin{EQA}
	&& \nquad
	\bigl\| \DFN (\upsvd - \upsvs - \IFT^{-1} \AAv) \bigr\|_{\infty}
	=
	\bigl\| \uv - \DFN \, \IFT^{-1} \AAv \bigr\|_{\infty}
	\\
	&=&
	\bigl\| B^{-1} \DFN^{-1} \{ \IFT (\upsvd - \upsvs) - \AAv \} \bigr\|_{\infty}
	\leq 
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}^{2} 
	\, .
\label{6f6f67vfg3we5dgwytquw}
\end{EQA}
Finally, by \eqref{Thd7w3jhdujrrfrrfgdyw3} of Lemma~\ref{LinvGersh} and by \( \DFN \, \IFT^{-1} \AAv = \BBN^{-1} \DFN^{-1} \AAv  \)
\begin{EQA}[rcccl]
	\| \DFN \, \IFT^{-1} \AAv - \DFN^{-1} \AAv \|_{\infty}
	& = &
	\bigl\| (\BBN^{-1} - \Id_{\dimp}) \DFN^{-1} \AAv \bigr\|_{\infty}
	& \leq &
	\frac{\crosssup}{1 - \crosssup} \| \DFN^{-1} \AAv \bigr\|_{\infty} \, ,
	\\
	\| \DFN \, \IFT^{-1} \AAv - (\Id_{\dimp} + \Delta) \DFN^{-1} \AAv \|_{\infty}
	& = &
	\bigl\| (\BBN^{-1} - \Id_{\dimp} - \Delta) \DFN^{-1} \AAv \bigr\|_{\infty}
	& \leq &
	\frac{\crosssup^{2}}{1 - \crosssup} \| \DFN^{-1} \AAv \bigr\|_{\infty} \, .
\label{6c6tyc6c6cf6de5tw5}
\end{EQA}
This and \eqref{6f6f67vfg3we5dgwytquw} imply the final inequalities of the proposition.
\end{proof}

\begin{lemma}
\label{LinvGersh}
Let \( \BBN = (\BBN_{ij}) \in \Matr_{\dimp} \) with \( \BBN_{ii} = 1 \) and 
\begin{EQA}[c]
	\sup_{\uv \colon \| \uv \|_{\infty} \leq 1} \, \| (\BBN - \Id_{\dimp}) \uv \|_{\infty} \leq \crosssup < 1 .
\label{8f98dej237yt656543n}
\end{EQA}
Then \( \| \BBN \uv \|_{\infty} \leq (1 - \crosssup)^{-1} \| \uv \|_{\infty} \) for any \( \uv \in \R^{\dimp} \).
Similarly,
\begin{EQA}[c]
	\| (\BBN^{-1} - \Id_{\dimp}) \uv \|_{\infty} \leq \frac{\crosssup}{1 - \crosssup} \, \| \uv \|_{\infty}
	\, ,
	\quad
	\| (\BBN^{-1} - 2 \Id_{\dimp} + \BBN) \uv \|_{\infty} \leq \frac{\crosssup^{2}}{1 - \crosssup} \, \| \uv \|_{\infty}
	\, .
	\qquad
\label{Thd7w3jhdujrrfrrfgdyw3}
\end{EQA}
\end{lemma}

\begin{proof}
Represent \( \BBN = \Id_{\dimp} - \Delta \).
Then \eqref{8f98dej237yt656543n} implies \( \| \Delta \uv \|_{\infty} \leq \crosssup \| \uv \|_{\infty} \).
The use of \( \BBN^{-1} = \Id_{\dimp} + \Delta + \Delta^{2} + \ldots \) yields for any \( \uv \in \R^{\dimp} \)
\begin{EQA}[c]
	\| \BBN^{-1} \uv \|_{\infty}
	\leq 
	\sum_{m=0}^{\infty} \| \Delta^{m} \uv \|_{\infty} \, .
\end{EQA}
Further, with \( \uv_{m} \eqdef \Delta^{m} \uv \), it holds
\begin{EQA}
	\| \Delta^{m+1} \uv \|_{\infty}
	&=&
	\| \Delta \uv_{m} \|_{\infty}
	\leq 
	\crosssup \| \uv_{m} \|_{\infty} \, .
\label{cd7dysrtd4ftgewhged4r}
\end{EQA}
By induction, this yields \( \| \Delta^{m} \uv \|_{\infty} \leq \crosssup^{m} \| \uv \|_{\infty} \) and thus,
\begin{EQA}[c]
	\| \BBN^{-1} \uv \|_{\infty}
	\leq 
	\sum_{m=0}^{\infty} \crosssup^{m} \| \uv \|_{\infty}
	= 
	\frac{1}{1 - \crosssup} \, \| \uv \|_{\infty}
\end{EQA}
as claimed. 
The proof of \eqref{Thd7w3jhdujrrfrrfgdyw3} is similar in view of \( \Id_{\dimp} + \Delta = 2 \Id_{\dimp} - \BBN \).
\end{proof}

\Section{Sup-norm expansions for a separable perturbation}
A linear perturbation is a special case of a separable perturbation of the form 
\( \pert(\upsv) = \sum_{j} \pert_{j}(\ups_{j}) \).
Another popular example is a Tikhonov regularization with \( \pert_{j}(\ups_{j}) = \lambda \ups_{j}^{2} \) or, 
more generally, a Sobolev-type penalty \( \pert_{j}(\ups_{j}) = \gp_{j}^{2} \ups_{j}^{2} \) for a given sequence 
\( \gp_{j}^{2} \).
Later we assume each component \( \pert_{j}(\ups_{j}) \) to be sufficiently smooth.
This does not allow to incorporate a sparse penalty \( \pert_{j}(\ups_{j}) = \lambda |\ups_{j}| \) or
complexity penalty \( \pert_{j}(\ups_{j}) = \lambda \Ind(\ups_{j} \neq 0) \).

Let \( \fs(\upsv) \) be convex, \( \upsvs = \argmin_{\upsv} \fs(\upsv) \), and
\( \IFT = \nabla^{2} \fs(\upsvs) = (\IFT_{jm}) \).
Define a separable perturbation \( \fn(\upsv) = \fs(\upsv) - \pert(\upsv) \) of \( \fs(\upsv) \) by smooth functions \( \pert_{j}(\ups_{j}) \):
\begin{EQA}
	\fn(\upsv)
	&=&
	\fs(\upsv) - \pert(\upsv)
	=
	\fs(\upsv) - \sum_{j} \pert_{j}(\ups_{j}), 
\label{c7c7ctefwct5enfvyewsd}
\end{EQA} 
and let \( \upsvn = \argmin_{\upsv} \fn(\upsv) \).
We intend to bound the corresponding change \( \upsvn - \upsvs \) in a sup-norm.
Separability of the penalty is very useful, the cross derivatives of \( \fn \) are the same as for \( \fs \).
We only update the tensor \( \DFN(\upsv) \) assuming concavity of each \( \pert_{j}(\cdot) \):
\begin{EQA}
	\DFN(\upsv)
	& \eqdef &
	\diag\{ \DFN_{1}(\upsv),\ldots,\DFN_{\dimp}(\upsv) \},
	\qquad
	\DFN_{j}^{2}(\upsv)
	\eqdef
	\IF_{jj}(\upsv) - \pert''_{j}(\ups_{j}) \, .
\label{7fyc5wgdf7vrewgdhfywh}
\end{EQA}

\begin{proposition}
\label{Psemibiassupp}
Let \( \fs(\upsv) \) be convex function and 
\( \fn(\upsv) \) be a separable perturbation of \( \fs(\upsv) \); see \eqref{c7c7ctefwct5enfvyewsd}. 
For \( \upsvn = \argmin_{\upsv} \fn(\upsv) \), define the diagonal metric tensor \( \DFN = \DFN(\upsvn) \); 
see \eqref{7fyc5wgdf7vrewgdhfywh}.
Let \( \crosssup \) from \eqref{7tdsyf8iuwopkrtg4576} fulfill \( \crosssup < 1 \). 
Fix \( \Avm \eqdef \nabla \pert(\upsvs) = (\pert'_{j}(\upss_{j})) \) and 
\begin{EQA}
	\rrinf 
	&=& 
	\frac{\sqrt{2}}{1 - \crosssup} \| \DFN^{-1} \Avm \|_{\infty} 
	\, .
\label{8drywjwuycrt5sdeteyhfuwkp}
\end{EQA}
Let \nameref{LLpsupref} hold for \( \fn \) with this \( \rrinf \) and
\( \dltwun, \dltwunn, \dltwu_{3} \) satisfying  
\begin{EQA}[c]
	\dltwbun = \dltwunn \, \rrinf \leq 1/4 ,
	\qquad
	\dltwun \, \rrinf \leq 1/4 \, ,
	\qquad	
	\dltwunss \| \DFN^{-1} \Avm \|_{\infty} 
	\leq 
	\sqrt{2} - 1
	\, ,
\label{dhfiejfowelocuyehbrfp}
\end{EQA}
where
\begin{EQA}[rcl]
	\dltwuns
	& \eqdef &
	\frac{1}{1 - \dltwbun} \, 
	\biggl( \crosssup \, \dltwunn + \frac{\dltwun}{2}
		+ \frac{3(\crosssup + \dltwbun/2)^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} 
%		+ \frac{3\dltwu_{3}\, \dltwun^{2} \, \rru^{2}}{4(1 - \dltwbund)^{2}} 
	\biggr) 
	\, ,
\label{36gfijh94ejdvtwekoisedip}
	\\
	\dltwunss
	& \eqdef &
	2 \dltwu_{3} + \frac{\dltwunn}{2}  + \frac{2(\dltwuns + \dltwunn)}{(1 - \crosssup)^{2}} 
	\, .
\end{EQA}
Then \( \upsvd = \argmin_{\upsv} \fn(\upsv) \) satisfies
\begin{EQA}
	\| \DFN (\upsvd - \upsvs) \|_{\infty}
	\eqdef
	\max_{j \leq \dimp} | \DFN_{j} (\upsd_{j} - \upss_{j}) |
	& \leq &
	\rrinf \, .
\label{7ytdufchskmls7rghnkp}
\end{EQA} 
Furthermore, 
\begin{EQA}
\label{usdhyw6hikhurnetrsppp}
	\bigl\| \DFN^{-1} \bigl\{ \IFT (\upsvd - \upsvs) - \Avm \bigr\} \bigr\|_{\infty}
	& \leq &
	\dltwunss \, \| \DFN^{-1} \Avm \|_{\infty}^{2} 
	\, ,
	\\
	\bigl\| \DFN (\upsvd - \upsvs - \IFT^{-1} \Avm) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \Avm \|_{\infty}^{2} 
	\, ,
	\qquad
\label{usdhyw6hikhurnetrspp1p}
\end{EQA}
and with \( \Delta \eqdef \Id_{\dimp} - \DFN^{-1} \IFT \, \DFN^{-1} \)
\begin{EQ}[rcl]
	\bigl\| \DFN (\upsvd - \upsvs) - \DFN^{-1} \Avm) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \Avm \|_{\infty}^{2} + \frac{\crosssup}{1 - \crosssup} \, \| \DFN^{-1} \Avm \|_{\infty}
	\, ,
	\\
	\bigl\| \DFN (\upsvd - \upsvs) - (\Id_{\dimp} + \Delta) \DFN^{-1} \Avm) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \Avm \|_{\infty}^{2} + \frac{\crosssup^{2}}{1 - \crosssup} \, \| \DFN^{-1} \Avm \|_{\infty}
	\, .
	\qquad
\label{usdhyw6hikhurnetrspp2p}
\end{EQ}
\end{proposition}

\begin{remark}
\label{RLLsup}
If each \( \pert_{j}(\ups_{j}) \) is quadratic, then condition \nameref{LLpsupref} for \( \fn(\upsv) \) follows from 
the same condition for \( \fs(\upsv) \) as the third derivatives of these two functions coincide.
For general smooth perturbations \( \pert_{j} \), \eqref{d6f53ye5vry4fddfgsup} should be checked
for \( \nabla^{3}_{\ups_{j}\ups_{j} \ups_{j}} \fn(\upsv) = \nabla^{3}_{\ups_{j}\ups_{j} \ups_{j}} \fs(\upsv) + \pert'''_{j}(\ups_{j}) \).
The other conditions in \nameref{LLpsupref} can be checked for \( \fs \).
\end{remark}




==> semi_opt.tex <==
% !TEX root = ../semi/semiplugin.tex
%% !TEX root = ../generic.tex

\def\AUv{\Delta}
\def\cmax{\CONST}
\def\upsn{\ups^{\circ}}
\def\pert{t}

\Section{Conditional and marginal optimization}
\label{Ssemiopt}
This section describes the problem of conditional/partial and marginal optimization. 
Consider a function \( \fs(\prmtv) \) of a parameter \( \prmtv \in \R^{\dimttl} \)
which can be represented as \( \prmtv = (\targv,\nuiv) \), where \( \targv \in \R^{\dimp} \)
is the target subvector while \( \nuiv \in \R^{\dimq} \) is a nuisance variable.
Our goal is to study the solution to the optimization problem 
\( \prmtvs = (\targvs,\nuivs) = \argmax_{\prmtv} \fs(\prmtv) \) and, in particular, 
its target component \( \targvs \).
Later we consider a localized setup with a set \( \Ups \) of pairs \( \prmtv = (\targv,\nuiv) \) 
to be fixed around \( \prmtvs \).


\Subsection{Partial optimization}
For any fixed value of the nuisance variable \( \nuiv \in \Nui \), consider 
\( \fs_{\nuiv}(\targv) = \fs(\targv,\nuiv) \) as a function of \( \targv \) only.
Below we assume that \( \fs_{\nuiv}(\targv) \) is concave in \( \targv \) for any \( \nuiv \in \Nui \).
Define 
\begin{EQA}[rcl]
	\targv_{\nuiv}
	& \eqdef &
	\argmax_{\targv \colon (\targv,\nuiv) \in \Ups} \fs_{\nuiv}(\targv) \, .
\label{jfoiuy2wedfv7tr2qsdzxdfso}
%	\\
%	\feta_{\nuiv}
%	& \eqdef &
%	\max_{\targv \colon (\targv,\nuiv) \in \Ups} \fs_{\nuiv}(\targv) - \fs(\prmtvs)
%	=
%	\fs_{\nuiv}(\targv_{\nuiv}) - \fs(\prmtvs) .
%\label{kfdy8d3fgfnm0lkgrr3so}
\end{EQA}
%The value \( - \feta_{\nuiv} \) measuring the difference between the global maximum of 
%\( \fs(\prmtv) \) and the partial maximum of \( \fs(\targv,\nuiv) \) w.r.t. \( \targv \) 
%for \( \nuiv \) fixed can be called the \( \nuiv \)-\emph{deficiency}. 
Our goal is to describe variability of the partial solution \( \targv_{\nuiv} \) in \( \nuiv \) in terms of \( \targv_{\nuiv} - \targvs \)
and \( \fs(\prmtvs) - \fs_{\nuiv}(\targv_{\nuiv}) \).
Introduce 
\begin{EQ}[rcccc]
	\Av_{\nuiv}
	& \eqdef &
	\nabla \fs_{\nuiv}(\targvs)
	&=&
	\nabla_{\targv} \fs(\targvs,\nuiv) 
	\, ,
	\\
	\IFN_{\nuiv}
	& \eqdef &
	- \nabla^{2} \fs_{\nuiv}(\targvs) 
	&=&
	- \nabla_{\targv\targv}^{2} \fs(\targvs,\nuiv) 
	\, .
\label{ge8qwefygw3qytfyju8qfhbdso}
\end{EQ}
Local smoothness of each function \( \fs_{\nuiv}(\cdot) \) around \( \targv_{\nuiv} \) 
can be well described under the self-concordance property.
Let for any \( \nuiv \in \Nui \), some radius \( \rrn_{\nuiv} \) be fixed.
%For ease of notation, we omit the subindex \( \nuiv \) here.
%in a way that \( \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \| \leq \amax \, \rrn \). 
We also assume that a local metric on \( \R^{\dimp} \)
for the target variable \( \targv \) is defined by a matrix \( \DFN_{\nuiv} \in \Matr_{\dimp} \)
that may depend on \( \nuiv \in \Nui \).
Later we assume \nameref{LLsT3ref} %or \nameref{LLsT4ref} 
to be fulfilled for all \( \fs_{\nuiv} \), \( \nuiv \in \Nui \).

\begin{description}

    \item[\label{LLsoT3ref} \( \bb{(\mathcal{T}_{3|\nuiv}^{*})} \)]
      \emph{For \( \nuiv \in \Nui \), 
      % the function \( \fs_{\nuiv}(\targv) \) is strongly concave. 
      % for all \( \targv \in \CA \) 
      %With \( \DFN_{\nuiv}^{2} \leq \dmax^{2} \, \IFN_{\nuiv} \), 
      it holds
\begin{EQA}
%	\sup_{\targv \in \CA_{\GP}} \,\,
	\sup_{\uv \in \R^{\dimp} \colon \| \DFN_{\nuiv} \uv \| \leq \rrn_{\nuiv}}  \,\, \sup_{\zv \in \R^{\dimp}} \,\,
	\frac{\bigl| \langle \nabla^{3} \fs_{\nuiv}(\targv_{\nuiv} + \uv), \zv^{\otimes 3} \rangle \bigr|}
		 {\| \DFN_{\nuiv} \zv \|^{3}}
	& \leq &
	\dltwu_{3} \, .
\label{d6f53ye5vry4fddfgeyd}
\end{EQA}
}

%    \item[\label{LLsoT4ref} \( \bb{(\mathcal{T}_{4|\nuiv}^{*})} \)]
%      \emph{\( \fs_{\nuiv}(\targv) \) follows \nameref{LLsoT3ref} 
%      and }
%\begin{EQA}
%%	\sup_{\targv \in \CA_{\GP}} \,\,
%	\sup_{\uv \in \R^{\dimp} \colon \| \DFN_{\nuiv} \uv \| \leq \rrn}  \,\, \sup_{\zv \in \R^{\dimp}} \,\,
%	\frac{\bigl| \langle \nabla^{4} \fs_{\nuiv}(\targv_{\nuiv} + \uv), \zv^{\otimes 4} \rangle \bigr|}
%		 {\| \DFN_{\nuiv} \zv \|^{4}}
%	& \leq &
%	\dltwu_{4} \, .
%\label{d6f53ye5vry4fddfgeyd4}
%\end{EQA}
\end{description}


Our first result describes the \emph{semiparametric bias} \( \targvs - \targv_{\nuiv} \) caused by using
the value \( \nuiv \) of the nuisance variable in place of \( \nuivs \).

\begin{proposition}
\label{PbiassemiN}
Let \( \fs_{\nuiv}(\targv) \) be a strongly concave function with 
\( \fs_{\nuiv}(\targv_{\nuiv}) = \max_{\targv} \fs_{\nuiv}(\targv) \)  
and \( \IFN_{\nuiv} = - \nabla^{2} \fs_{\nuiv}(\targv_{\nuiv}) \).
Let \( \Av_{\nuiv} \) and \( \IFN_{\nuiv} \) be given by \eqref{ge8qwefygw3qytfyju8qfhbdso}.
Assume \nameref{LLsoT3ref} at \( \targv_{\nuiv} \) with \( \DFN_{\nuiv}^{2} \), \( \rrn_{\nuiv} \), and \( \dltwu_{3} \) such that 
\begin{EQA}[c]
	\DFN_{\nuiv}^{2} \leq \dmax^{2} \, \IFN_{\nuiv} ,
	\quad
	\rrn_{\nuiv} \geq \frac{3}{2} \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \| \, ,
	\quad
	\dmax^{2} \dltwu_{3} \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \| < \frac{4}{9} \, .
\label{8difiyfc54wrboer7bjfr}
\end{EQA}
%Assume \nameref{LLsoT3ref} with \( \rrn \geq \amax^{-1} \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \| \) for \( \amax \leq 2/3 \).
%Let also \( \dltwu_{3} \, \rrn/2 < 1 - \amax \).
Then \( \| \DFN_{\nuiv} (\targv_{\nuiv} - \targvs) \| \leq (3/2) \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \| \) and moreover,
\begin{EQ}[rcccl]
    \| \DFN_{\nuiv}^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs - \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
    & \leq &
    \frac{3\dltwu_{3}}{4} \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{2} 
    & \leq &
    \frac{\dltwu_{3} \, \rrn_{\nuiv}}{2} \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|
%	\, ,
%	\qquad
%	\\
%    \| \IFN_{\nuiv}^{1/2} (\targv_{\nuiv} - \targvs - \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
%    & \leq &
%    \frac{3 \dmax^{3} \dltwu_{3} }{4} \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} 
%    & \leq &
%    \frac{\dmax^{2} \dltwu_{3} \, \rr}{2} \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|
	\, .
	\qquad
\label{jhcvu7ejdytur39e9frtfw}
\end{EQ}
Moreover,
\begin{EQA}
	\bigl| 
		2 \fs_{\nuiv}(\targv_{\nuiv}) - 2 \fs_{\nuiv}(\targvs) - \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} 
	\bigr|
	& \leq &
	\frac{5\dltwu_{3}}{2} \, \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{3} \, .
	\qquad
\label{gtxddfujhyfdytet6ywerfd}
\end{EQA}

\end{proposition}

\begin{proof}
Define \( \fn_{\nuiv}(\targv) = \fs_{\nuiv}(\targv) - \langle \targv,\Av_{\nuiv} \rangle \).
Then \( \fn_{\nuiv} \) is concave and \( \nabla \fn_{\nuiv}(\targvs) = 0 \) yielding 
\( \targvs = \argmax_{\targv} \fn_{\nuiv}(\targv) \).
Now Proposition~\ref{PFiWigeneric2} yields \eqref{jhcvu7ejdytur39e9frtfw}.
Also by \eqref{3d3Af12DGttGa2}
\begin{EQA}
	\Bigl| 2 \fn_{\nuiv}(\targvs) - 2 \fn_{\nuiv}(\targv_{\nuiv}) - \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} \Bigr|
	& \leq &
	\frac{\dltwu_{3}}{2} \, \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{3} 
\label{ytduw237832jfg656335hdi}
\end{EQA}
yielding
\begin{EQA}
	\bigl| 
		2 \fs_{\nuiv}(\targvs) - 2 \fs_{\nuiv}(\targv_{\nuiv}) - 2 \langle \targvs - \targv_{\nuiv} , \Av_{\nuiv} \rangle 
		- \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} 
	\bigr|
	& \leq &
	\frac{\dltwu_{3}}{2} \, \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{3} \, .
	\qquad
\label{gtxdbcbcgdfswerfdsdew}
\end{EQA}
By \eqref{jhcvu7ejdytur39e9frtfw}
\begin{EQA}
	&& \nquad
	\bigl| \langle \targvs - \targv_{\nuiv} , \Av_{\nuiv} \rangle + \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} \bigr|
	=
	\bigl| \langle \IFN_{\nuiv}^{1/2} (\targvs - \targv_{\nuiv}) , \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \rangle 
	+ \langle \IFN_{\nuiv}^{-1/2} \Av_{\nuiv},\IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \rangle \bigr|
	\\
	&=&
	\bigl| \langle \IFN_{\nuiv}^{1/2} (\targvs - \targv_{\nuiv} + \IFN_{\nuiv}^{-1} \Av_{\nuiv}) , 
		\IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \rangle 
	\bigr|
	\\
	& \leq &
	\| \DFN_{\nuiv}^{-1} \, \IFN_{\nuiv} (\targvs - \targv_{\nuiv} + \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \| \, \,
		\| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|
	\leq 
	\frac{3\dltwu_{3}}{4} \, \| \DFN_{\nuiv} \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{3}
\label{duy7cyf6re6eytedhge2}
\end{EQA}
This and \eqref{gtxdbcbcgdfswerfdsdew} imply \eqref{gtxddfujhyfdytet6ywerfd}.
\end{proof}

%Two values \( \nuiv \) and \( \nuivs \) of the nuisance variable in the result 
%of Proposition~\ref{PbiassemiN} can be exchanged. 
%This leads to the following bounds.
%
%
%\begin{proposition}
%\label{PbiassemiNs}
%Define \( \Avs_{\nuiv} \eqdef \nabla \fs_{\nuivs}(\targv_{\nuiv}) \).
%Assume \nameref{LLsoT3ref} with \( \rrn \geq \amax^{-1} \| \IFN^{-1/2} \Avs_{\nuiv} \| \) for 
%\( \amax \leq 2/3 \).
%Let also \( \dltwu_{3} \, \rrn/2 < 1 - \amax \).
%Then
%\begin{EQ}[rcl]
%	\| \IFN^{1/2} (\targvs - \targv_{\nuiv}) \|
%	& \leq &
%	\amax^{-1} \| \IFN^{-1/2} \Avs_{\nuiv} \| \, ,
%\label{duejei9viewe76fyjrtgbhgs}
%	\\
%	\| \IFN^{1/2} (\targv_{\nuiv} - \targvs) - \IFN^{-1/2} \Avs_{\nuiv} \|^{2}
%	& \leq &
%	\dltwu_{3} \, \| \IFN^{-1/2} \Avs_{\nuiv} \|^{3} \, .
%%\label{jhcvu7ejdytur39e9frtfws}
%\end{EQ}
%Moreover,
%\begin{EQA}
%	\bigl| 
%		2 \fs_{\nuivs}(\targvs) - 2 \fs_{\nuivs}(\targv_{\nuiv}) - \| \IFN^{-1/2} \Avs_{\nuiv} \|^{2} 
%	\bigr|
%	& \leq &
%	\dltwu_{3} \, \| \IFN^{-1/2} \Avs_{\nuiv} \|^{3} 
%	+ 2 \sqrt{\dltwu_{3}} \, \| \IFN^{-1/2} \Avs_{\nuiv} \|^{5/2} \, .
%	\qquad
%\label{gtxddfujhyfdytet6ywerfds}
%\end{EQA}
%\end{proposition}

%The approximation bounds can be improved under higher order smoothness of each \( \fs_{\nuiv} \).
%Namely, Proposition~\ref{Pconcgeneric4} implies the following advanced approximation.
%
%\begin{proposition}
%\label{PbiassemiNs4}
%Assume the conditions of Proposition~\ref{PbiassemiN} and \nameref{LLsoT4ref}.
%Define
%\begin{EQA}
%	\avn_{\nuiv} 
%	&=&
%	\IFN_{\nuiv}^{-1} \{ \Av_{\nuiv} + \nabla \Tens_{\nuiv}(\IFN_{\nuiv}^{-1} \Av_{\nuiv}) \} ,
%\label{8vfjvr43223efryfuweefse}
%\end{EQA}
%where \( \Tens_{\nuiv}(\uv) = \frac{1}{6} \langle \nabla_{\targv\targv\targv}^{3} \fs(\targvs,\nuiv), \uv^{\otimes 3} \rangle \)
%and \( \nabla \Tens_{\nuiv}(\uv) = \frac{1}{2} \langle \nabla_{\targv\targv\targv}^{3} \fs(\targvs,\nuiv), \uv^{\otimes 2} \rangle \).
%Then
%\begin{EQ}[rcl]
%	\| \IFN_{\nuiv}^{1/2} \avn_{\nuiv} - \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|
%	& \leq &
%	\frac{\dltwu_{3}}{2} \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{2} 
%	\leq 
%	\frac{\dltwu_{3} \, \amax \, \rr}{2} \, \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|,
%	\\
%	\| \IFN_{\nuiv}^{1/2} \avn_{\nuiv} \|
%	& \leq &
%	\Bigl( 1 + \frac{\dltwu_{3} \, \amax \, \rr}{2} \Bigr) \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \| \, ,
%	\qquad
%\label{iuvchycvf6e64rygh322se}
%\end{EQ}
%and
%\begin{EQ}[rcccl]
%    \| \IFN_{\nuiv}^{1/2} (\targv_{\nuiv} - \targvs + \avn_{\nuiv}) \|
%    & \leq &
%    \frac{\dltwu_{4} + 3 \dltwu_{3}^{2}}{6(1 - \dltwu_{3} \, \rr)} \, \| \IFN_{\nuiv}^{1/2} \avn_{\nuiv} \|^{3} 
%    & \leq &
%    \frac{\dltwu_{4} + 3 \dltwu_{3}^{2}}{3} \, \| \IFN_{\nuiv}^{-1/2} \Av_{\nuiv} \|^{3} \, .
%%    \| \IFN^{-1/2} \Avs_{\nuiv} \|^{3} \, ,
%\label{DGttGtsGDGm13rGa4se}
%\end{EQ}
%\end{proposition}
%

\Subsection{Conditional optimization under (semi)orthogonality}
\label{SortLaplsemi}
Here we study variability of the value \( \targv_{\nuiv} = \argmax_{\targv} \fs(\targv,\nuiv) \)
w.r.t. the nuisance para\-meter \( \nuiv \).
It appears that local quadratic approximation of the function \( \fs \) in a vicinity of the extreme point
\( \prmtvs \) yields a nearly linear dependence of \( \targv_{\nuiv} \) on \( \nuiv \).
We illustrate this fact on the case of a quadratic function \( \fs(\cdot) \).
Consider the negative Hessian \( \IFT = - \nabla^{2} \fs(\prmtvs) \) in the block form:
\begin{EQA}
	\IFT
	& \eqdef &
	- \nabla^{2} \fs(\prmtvs)
	=
	\begin{pmatrix}
	\IFT_{\targv\targv} & \IFT_{\targv\nuiv}
	\\
	\IFT_{\nuiv\targv} & \IFT_{\nuiv\nuiv}
	\end{pmatrix} 
\label{hwe78yf2diwe76tfw67etfwtbso}
\end{EQA}
with \( \IFT_{\nuiv\targv} = \IFT_{\targv\nuiv}^{\T} \).
If \( \fs(\prmtv) \) is quadratic then \( \IFT \) and its blocks do not depend on \( \prmtv \).

\begin{lemma}
\label{Lpartmaxq}
%To see this, suppose for a moment that 
Let \( \fs(\prmtv) \) be {quadratic}, {strongly concave}, and \( \nabla \fs(\prmtvs) = 0 \).
Then
\begin{EQA}
	\targv_{\nuiv} - \targvs 
	&=& 
	- \IFT_{\targv\targv}^{-1} \, \IFT_{\targv\nuiv} \, (\nuiv - \nuivs) .
\label{0fje7fhihy84efiewkw}
\end{EQA}
\end{lemma}

\begin{proof}
The condition \( \nabla \fs(\prmtvs) = 0 \) implies 
\( \fs(\prmtv) = \fs(\prmtvs) - (\prmtv - \prmtvs)^{\T} \IFT \, (\prmtv - \prmtvs)/2 \) 
with \( \IFT = - \nabla^{2} \fs(\prmtvs) \).
For \( \nuiv \) fixed, the point \( \targv_{\nuiv} \) maximizes 
\( - (\targv - \targvs)^{\T} \IFT_{\targv\targv} \, (\targv - \targvs) /2 - (\targv - \targvs)^{\T} \IFT_{\targv\nuiv} \, (\nuiv - \nuivs) \)
and thus, \( \targv_{\nuiv} - \targvs = - \IFT_{\targv\targv}^{-1} \, \IFT_{\targv\nuiv} \, (\nuiv - \nuivs) \).
\end{proof} 

This observation \eqref{0fje7fhihy84efiewkw} is in fact discouraging 
because the bias \( \targv_{\nuiv} - \targvs \) has the same magnitude as the nuisance parameter \( \nuiv - \nuivs \).
However, the condition \( \IFT_{\targv\nuiv} = 0 \) yields \( \targv_{\nuiv} \equiv \targvs \) 
and the bias vanishes.
If \( \fs(\prmtv) \) is not quadratic, the \emph{orthogonality} condition \( \nabla_{\nuiv} \nabla_{\targv} \, \fs(\targv,\nuiv) \equiv 0 \)
for all \( (\targv,\nuiv) \in \WV \) still ensures a vanishing bias.


\begin{lemma}
\label{Lpartmax}
Let \( \fs(\targv,\nuiv) \) be continuously differentiable and 
\( \nabla_{\nuiv} \nabla_{\targv} \, \fs(\targv,\nuiv) \equiv 0 \).
Then the point 
\( \targv_{\nuiv} = \argmax_{\targv} f(\targv,\nuiv) \) does not depend on \( \nuiv \).
\end{lemma}

\begin{proof}
The condition \( \nabla_{\nuiv} \nabla_{\targv} \, \fs(\targv,\nuiv) \equiv 0 \) implies the decomposition 
\( \fs(\targv,\nuiv) = \fs_{1}(\targv) + \fs_{2}(\nuiv) \) for some functions 
\( \fs_{1} \) and \( \fs_{2} \).
This in turn yields \( \targv_{\nuiv} \equiv \targvs \).
%Moreover, without loss of generality, one may assume \( \fs_{1}(\targvs) = \max_{\targv} \fs_{1}(\targv) = 0 \) and 
%\( \fs_{2}(\nuivs) = \max_{\nuiv} \fs_{2}(\nuiv) = 0 \).  
\end{proof}

In some cases, one can check \emph{semi-orthogonality} condition 
\begin{EQA}
	\nabla_{\nuiv} \nabla_{\targv} \, \fs(\targvs,\nuiv)  
	&=&
	0,
	\qquad
	\forall \nuiv \in \Nui \, .
\label{jdgyefe74erjscgygfydhwse}
\end{EQA}
\ifapp{A typical example is given by nonlinear regression; see Section~\ref{SnonlinLA}.}{}

\begin{lemma}
\label{Lsemiorto}
Assume \eqref{jdgyefe74erjscgygfydhwse}.
Then 
\begin{EQA}[rcccl]
	\nabla_{\targv} \, \fs(\targvs,\nuiv)
	& \equiv &
	0,
	\qquad
%	\IFN_{\nuiv}
%	& \equiv &
%	\IFN_{\nuivs}
%	= 
	\nabla_{\targv\targv}^{2} \fs(\targvs,\nuiv) 
	& \equiv &
	\nabla_{\targv\targv}^{2} \fs(\targvs,\nuivs),
	\qquad
	\nuiv \in \Nui .
\label{0xyc5ftr4j43vefvuruendt}
\end{EQA}
Moreover, if \( \fs(\targv,\nuiv) \) is concave in \( \targv \) given \( \nuiv \) then
\begin{EQA}
	\targv_{\nuiv} 
	& \eqdef & 
	\argmax_{\targv} \fs(\targv,\nuiv) \equiv \targvs ,
	\qquad
	\forall \nuiv \in \Nui \,.
\label{irdtyrnjjutu45r7gjhr}
\end{EQA}
%\( \IFN_{\nuiv} \eqdef - \nabla_{\targv\targv}^{2} \fs(\targvs,\nuiv) \) satisfies
\end{lemma}

\begin{proof}
Consider the vector \( \Av_{\nuiv} = \nabla_{\targv} \, \fs(\targvs,\nuiv) \).
%\begin{EQA}
%	\Av_{\nuiv} 
%	& \eqdef & 
%	\nabla_{\targv} \, \fs(\targvs,\nuiv) \, .
%\label{02h874shki7rwhuyfv}
%\end{EQA}
Obviously \( \Av_{\nuivs} = 0 \).
Moreover, \eqref{jdgyefe74erjscgygfydhwse} implies that \( \Av_{\nuiv} \) 
does not depend on \( \nuiv \) and thus, vanishes everywhere.
As \( \fs \) is concave in \( \targv \), 
this implies \( \fs(\targvs,\nuiv) = \max_{\targv} \fs(\targv,\nuiv) \)
and \( \targv_{\nuiv} = \argmax_{\targv} \fs(\targv,\nuiv) \equiv \targvs \).
Similarly, by \eqref{jdgyefe74erjscgygfydhwse}, it holds
\( \nabla_{\nuiv} \nabla_{\targv\targv} \, \fs(\targvs,\nuiv) \equiv 0 \) 
and \eqref{0xyc5ftr4j43vefvuruendt} follows.
Concavity of \( \fs(\targv,\nuiv) \) in \( \targv \) for \( \nuiv \) fixed and \eqref{0xyc5ftr4j43vefvuruendt} 
imply \eqref{irdtyrnjjutu45r7gjhr}.
\end{proof}

Orthogonality or semi-orthogonality \eqref{jdgyefe74erjscgygfydhwse} conditions are rather 
restrictive and fulfilled only in special situations.
% like nonlinear regression in Section~\ref{SnonlinLA}.
A weaker condition of 
%
\emph{one-point orthogonality} means \( \nabla_{\nuiv} \nabla_{\targv} \, \fs(\targvs,\nuivs) = 0 \).
This condition is not restrictive and can always be enforced by a linear transform of the nuisance variable \( \nuiv \).
%see Section~\ref{Sonepointtrans}.


\Subsection{Semiparametric bias}
\label{Sonepoint}


%\Subsection{A bound on \( \targv_{\nuiv} \)}

This section explains how one can bound variability of 
\( \IFN_{\nuiv} = - \nabla_{\targv\targv}^{2} \fs(\targvs,\nuiv) \)
and of the norm of \( \targv_{\nuiv} - \targvs \) under  
conditions on the cross-derivatives of \( \fs(\targv,\nuiv) \) for \( \nuiv = \nuivs \)
or \( \targv = \targvs \).
Suppose that the nuisance variable \( \nuiv \) is already localized to a small vicinity \( \Nui \) of \( \nuivs \).
A typical example is given by the level set \( \Nui \) of the form
\begin{EQA}
	\Nui
	&=&
	\bigl\{ \nuiv \colon \| \HFN (\nuiv - \nuivs) \|_{\nano} \leq \rru \bigr\} ,
\label{6chbdtw2hydfuguye4223w23}
\end{EQA}
where \( \HFN \) is a metric tensor in \( \R^{\dimq} \), 
\( \| \cdot \|_{\nano} \) is a norm in \( \R^{\dimq} \), and \( \rru > 0 \).
Often \( \| \cdot \|_{\nano} \) is the usual \( \ell_{2} \)-norm.
However, in some situations, it is beneficial to use different topology for the target parameter \( \targv \)
and the nuisance parameter \( \nuiv \).
One example is given by estimation in \( \sup \)-norm with \( \| \cdot \|_{\nano} = \| \cdot \|_{\infty} \).

Assume the following condition.

\begin{description}

%    \item[\label{LLpT2ref} \( \bb{(\mathcal{T}_{2,\Nui}^{*})} \)]
%      \emph{
%      It holds with some \( \dltwbns \)
%}
%\begin{EQA}
%	\sup_{\nuiv \in \Nui} \,\, 
%	\sup_{\zv \in \R^{\dimp}, \wv \in \R^{\dimq}} \,
%	\frac{| \langle \nabla_{\targv\nuiv}^{2} \fs(\targvs,\nuiv), \zv \otimes \wv \rangle |}
%		 {\| \DFN \zv \| \, \| \HFN \wv \|_{\nano}}
%	& \leq &
%	\dltwbns \, ;
%	\qquad
%\label{c6ceyecc5e5etcT1}
%\end{EQA}

    \item[\label{LLpT3ref} \( \bb{(\mathcal{T}_{3,\Nui}^{*})} \)]
      \emph{%The function \( \fs(\targvs,\nuiv) \) is strongly convex in \( \nuiv \).
%      With \( \DFN^{2} \leq - \nabla_{\targv\targv}^{2} \fs(\prmtvs) \) and
%      \( \HFN^{2} \leq - \nabla_{\nuiv\nuiv}^{2} \fs(\prmtvs) \), 
      It holds with some \( \dltwun, \dltwunn \)
}
\begin{EQA}[rccl]
	\sup_{\nuiv \in \Nui} \,\, 
	\sup_{\zv \in \R^{\dimp}, \wv \in \R^{\dimq}} \,
	&
	\frac{| \langle \nabla_{\targv\nuiv\nuiv}^{3} \fs(\targvs,\nuiv), \zv \otimes \wv^{\otimes 2} \rangle |}
		 {\| \DFN \zv \| \, \| \HFN \wv \|_{\nano}^{2}}
	& \leq &
	\dltwun \, ,
	\qquad
\label{c6ceyecc5e5etcT2}
	\\
	\sup_{\nuiv \in \Nui} \,\, 
	\sup_{\zv \in \R^{\dimp}, \wv \in \R^{\dimq}} \,
	&
	\frac{| \langle \nabla_{\targv\targv\nuiv}^{3} \fs(\targvs,\nuiv), \zv^{\otimes 2} \otimes \wv \rangle |}
		 {\| \DFN \zv \|^{2} \, \| \HFN \wv \|_{\nano}}
	& \leq &
	\dltwunn \, .
\label{c6ceyecc5e5etctwhcyegwc}
\end{EQA}
\end{description}



\begin{remark}
Later we establish some bounds on the semiparametric bias assuming %\( \dltwu_{3} \, \rr \ll 1 \) from \nameref{LLsoT3ref} and 
\( (\dltwun + \dltwunn) \, \rru \ll 1 \). % from \nameref{LLpT3ref}. 
\end{remark}

\begin{remark}
Condition \nameref{LLpT3ref} only involves mixed derivatives 
%\( \nabla_{\targv\nuiv}^{2} \fs(\targvs,\nuiv) \), 
\( \nabla_{\targv\nuiv\nuiv}^{3} \fs(\targvs,\nuiv) \) and \( \nabla_{\targv\targv\nuiv}^{3} \fs(\targvs,\nuiv) \) 
of \( \fs(\targvs,\nuiv) \) for the fixed value \( \targv = \targvs \),
while condition \nameref{LLsoT3ref} only concerns smoothness of \( \fs(\targv,\nuiv) \) w.r.t. \( \targv \) for \( \nuiv \) fixed.
Therefore, the combination of \nameref{LLsoT3ref} and \nameref{LLpT3ref} is much weaker than the full dimensional 
condition \nameref{LLsT3ref}.
\end{remark}


The next result provides an expansion of the semiparametric bias \( \targv_{\nuiv} - \targvs \). 
For the norm \( \| \cdot \|_{\nano} \), 
let \( \| \BBH \|_{\dual} \) be the corresponding dual norm of an operator
\( \BBH \colon \R^{\dimq} \to \R^{\dimp} \):
\begin{EQA}
	\| \BBH \|_{\dual}
	&=&
	\sup_{\zv \colon \| \zv \|_{\nano} \leq 1} \| \BBH \zv \| .
\label{ygtuesdfhiwdsoif9ruta}
\end{EQA}
If \( p=1 \) and \( \| \cdot \|_{\nano} \) is the sup-norm \( \| \cdot \|_{\infty} \) then 
\( \| \BBH \|_{\dual} = \| \BBH \|_{1} \).
Define
\begin{EQA}
\label{f8vuehery6gv65ftehwee}
	\crossnorm
	& \eqdef &
	\| \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1} \|_{\dual} \, ,
	\\
	\crossgrad
	& \eqdef &
	\| \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1} \|_{\dual} + \dltwun \, \rru /2 \, .
\label{f8vuehery6gv65ftehwee1}
\end{EQA}
%
Proposition~\ref{PbiassemiN} evaluates the semiparametric bias \( \targvs - \targv_{\nuiv} \) in terms of 
the matrix 
%Later we need an upper bound on variability of the matrix 
\( \IFN_{\nuiv} = - \nabla_{\targv\targv}^{2} \fs(\targvs,\nuiv) \) and the vector 
\( \Av_{\nuiv} = \nabla \fs_{\nuiv}(\targvs) \).
The next result explains how these quantities can be controlled under \nameref{LLpT3ref}.
To simplify the formulation, we assume that \( \DFN^{2} \leq \IFN \); see Remark~\ref{Rdmax2} for an extension.

\begin{proposition}
\label{PsemiAvex}
Assume \nameref{LLpT3ref} with \( \DFN^{2} \leq \IFN \).
%\( \Nui \) from \eqref{6chbdtw2hydfuguye4223w23}, and
%\( \DFN, \dltwun, \dltwunn , \rru \) satisfying 
Fix \( \nuiv \in \Nui \), set \( \dltwbun \eqdef \dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} \), 
and assume \nameref{LLsoT3ref} with \( \DFN_{\nuiv} \equiv \DFN \), \( \rrn_{\nuiv} \equiv \rrn \), 
and \( \dltwu_{3} \),
such that %with \( \dltwbun \eqdef \dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} \), it holds
\begin{EQA}[c]
	\dltwbun < 1 \, ,
	\quad
	\rr 
	\geq 
	\frac{3 \crossgrad}{2(1 - \dltwbun)} \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, ,
	\quad
	\frac{\crossgrad \, \dltwu_{3}}{1 - \dltwbun} \, \| \HFN (\nuiv - \nuivs) \|_{\nano}
	\leq 
	\frac{4}{9} \, ,
	\qquad
\label{6cuydjd5eg3jfggu8eyt4h}
\end{EQA}
for \( \crossgrad \) from \eqref{f8vuehery6gv65ftehwee1}.
Then the partial solution \( \targv_{\nuiv} \) obeys 
\begin{EQA}
	\| \DFN (\targv_{\nuiv} - \targvs) \|
	& \leq &
	\frac{3 \crossgrad}{2(1 - \dltwbun)} \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \,. 
\label{rhDGtuGmusGU0a2spt}
\end{EQA}
%If \( \IFT_{\targv\nuiv} = \nabla_{\targv} \nabla_{\nuiv} \, \fs(\targvs,\nuivs) = 0 \), then
%for any linear mapping \( \QP \colon \R^{\dimp} \to \R^{\dimq} \)
%\begin{EQA}
%\label{36gfijh94ejdvtwekoi}
%	\| \QP (\targv_{\nuiv} - \targvs) \|
%	& \leq &
%	\| \QP \, \IFN^{-1} \DFN \| \, \frac{1}{1 - \dltwbun}
%	\Bigl( \frac{\dltwun}{2} 
%		+ \frac{3\dltwu_{3} \, \dltwun^{2} \, \rru^{2}}{4(1-\dltwbund)^{2}} 
%	\Bigr) 
%	\| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
%%	(1 + \dltwbun) \, \frac{\dltwun}{2} \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} 
% 	\, .
%\end{EQA}
Moreover, with \( \crossnorm \) from \eqref{f8vuehery6gv65ftehwee}, it holds
\begin{EQA}[c]
\label{36gfijh94ejdvtwekoise}
	\| \QP \{ \targv_{\nuiv} - \targvs + \IFN^{-1} \IFT_{\targv\nuiv} (\nuiv - \nuivs) \} \|
	\leq 
	\| \QP \, \IFN^{-1} \DFN \| \, \dltwuns
	\, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
	\, ,
	\qquad
	\\
	\dltwuns
	\eqdef 
	\frac{1}{1 - \dltwbun} \, 
	\biggl( \crossnorm \, \dltwunn + \frac{\dltwun}{2}
		+ \frac{3\crossgrad^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} 
%		+ \frac{3\dltwu_{3}\, \dltwun^{2} \, \rru^{2}}{4(1 - \dltwbund)^{2}} 
	\biggr) \, .
\label{36gfijh94ejdvtwekoised}
\end{EQA}
\end{proposition}

\begin{proof}
First we bound the variability of \( \IFN_{\nuiv} \) over \( \Nui \). 
%For \( \Nui \) of the form \eqref{6chbdtw2hydfuguye4223w23}, such a bound can be obtained from \nameref{LLpT3ref}.
Let \( \IFN = \IFN_{\nuivs} \).

\begin{lemma}
\label{L3IFNNui}
Assume \nameref{LLpT3ref}.
% and let \( \dltwunn \, \rru < 1 \).
Then for any \( \nuiv \in \Nui \)
\begin{EQA}
	\| \DFN^{-1} \, (\IFN_{\nuiv} - \IFN) \, \DFN^{-1} \|
	& \leq &
	\dltwunn \, \| \HFN (\nuiv - \nuivs) \|_{\nano} 
	\, .
\label{8c7c67cc6c63kdldlvvudw}
\end{EQA}
\end{lemma}

\begin{proof}
Let \( \nuiv \in \Nui \).
By \eqref{c6ceyecc5e5etctwhcyegwc}, for any \( \zv \in \R^{\dimp} \), it holds
\begin{EQA}
	&& \!\!\!\!
	\bigl| \bigl\langle \DFN^{-1} \, (\IFN_{\nuiv} - \IFN) \, \DFN^{-1}, \zv^{\otimes 2} \bigr\rangle \bigr|
	=
	\bigl| \bigl\langle \IFN_{\nuiv} - \IFN, (\DFN^{-1} \zv)^{\otimes 2} \bigr\rangle \bigr|
	\\
	& \leq &
	\sup_{t \in [0,1]}
	\bigl| \langle \nabla_{\targv\targv\nuiv}^{3} \fs(\targvs,\nuivs + t (\nuiv - \nuivs)), (\DFN^{-1} \zv)^{\otimes 2} \otimes (\nuiv - \nuivs) \rangle \bigr|
	\leq 
	\dltwunn \, \| \zv \|^{2}  \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, .
\label{9487654r5tghasdfgsup}
\end{EQA}
This yields \eqref{8c7c67cc6c63kdldlvvudw}.
\end{proof}


The next result describes some corollaries of \eqref{8c7c67cc6c63kdldlvvudw}. 

\begin{lemma}
\label{LIFvari}
Assume \( \DFN^{2} \leq \dmax^{2} \IFN \) and let some other matrix \( \IFN_{1} \in \Matr_{\dimp} \) satisfy
\begin{EQA}
	\| \DFN^{-1} \, (\IFN_{1} - \IFN) \, \DFN^{-1} \|
	& \leq &
	\dmax^{-2} \dltwbun 
\label{icfuifcu7dy7e3gw3ft6e}
\end{EQA}
with \( \dltwbun < 1 \).
Then
%Moreover, if \( \dltwbun \eqdef \dmax^{2} \, \dltwuud \| \HFN (\nuiv - \nuivs) \|_{\nano} < 1 \), then
\begin{EQA}[ccc]
\label{8c7c67cc6c63kdldlvvudw2}
	\| \IFN^{-1/2} \, (\IFN_{1} - \IFN) \, \IFN^{-1/2} \|
	& \leq &
	\dltwbun 
%	=
%	\dmax^{2} \, \dltwuud \| \HFN (\nuiv - \nuivs) \|_{\nano} 
	\, ,
	\\
	\| \IFN^{1/2} \, (\IFN_{1}^{-1} - \IFN^{-1}) \, \IFN^{1/2} \|
	& \leq &
	\frac{\dltwbun}{1 - \dltwbun} 
	\, ,
\label{g98g75re3gf76r4egu4e}
\end{EQA}
and
\begin{EQA}
	\frac{1}{1 + \dltwbun} \, \| \DFN \, \IFN^{-1} \, \DFN \|
	\leq 
	\| \DFN \, \IFN_{1}^{-1} \DFN \|
	& \leq &
	\frac{1}{1 - \dltwbun} \, \| \DFN \, \IFN^{-1} \, \DFN \|
	\, .
\label{g98g75re3gf76r4egu4ee}
\end{EQA}
Furthermore, for any vector \( \uv \)
\begin{EQA}[rcccl]
\label{uciuvcdiu3eoooodffcy}
	(1 - \dltwbun) \| \DFN^{-1} \IFN \uv \|
	& \leq &
	\| \DFN^{-1} \IFN_{1} \uv \|
	& \leq &
	(1 + \dltwbun) \| \DFN^{-1} \IFN \uv \| \, ,
	\qquad
	\\
	\frac{1 - 2 \dltwbun}{1 - \dltwbun} \| \DFN \, \IFN^{-1} \uv \|
	& \leq &
	\| \DFN \, \IFN_{1}^{-1} \uv \|
	& \leq &
	\frac{1}{1 - \dltwbun} \| \DFN \, \IFN^{-1} \uv \| \, .
	\qquad
\label{uciuvcdiu3eoooodffcym}
\end{EQA}
\end{lemma}

\begin{proof}
Statement \eqref{8c7c67cc6c63kdldlvvudw2} follows from \eqref{icfuifcu7dy7e3gw3ft6e}
because of \( \IFN^{-1} \leq \dmax^{2} \, \DFN^{-2} \).
Define now \( \Uv \eqdef \IFN^{-1/2} \, (\IFN_{1} - \IFN) \, \IFN^{-1/2} \). 
Then \( \| \Uv \| \leq \dltwbun \) and
\begin{EQA}
	\| \IFN^{1/2} \, (\IFN_{1}^{-1} - \IFN^{-1}) \, \IFN^{1/2} \|
	&=&
	\| (\Id + \Uv)^{-1} - \Id \|
	\leq 
	\frac{1}{1 - \dltwbun} \| \Uv \|
\label{uefu83yr83y38frkfbg7e}
\end{EQA}
yielding \eqref{g98g75re3gf76r4egu4e}.
Further,
\begin{EQA}
	\| \DFN \, (\IFN_{1}^{-1} - \IFN^{-1}) \, \DFN \|
	&=&
	\| \DFN \, \IFN_{1}^{-1} \IFN_{1} (\IFN_{1}^{-1} - \IFN^{-1}) \, \IFN \, \IFN^{-1} \DFN \|
	\\
	&=&
	\| \DFN \, \IFN_{1}^{-1} \DFN \, \DFN^{-1} (\IFN_{1} - \IFN) \DFN^{-1} \, \DFN \, \IFN^{-1} \DFN \|
	\\
	& \leq &
	\| \DFN \, \IFN_{1}^{-1} \DFN \| \, \| \DFN \, \IFN^{-1} \DFN \| \, \| \DFN^{-1} (\IFN_{1} - \IFN) \DFN^{-1} \| 
	\leq 
	\dltwbun \| \DFN \, \IFN_{1}^{-1} \DFN \| \, .
\label{odfu7eujgvy55r44rf}
\end{EQA}
This implies \eqref{g98g75re3gf76r4egu4ee}.
Also, by \( \DFN^{2} \leq \dmax^{2} \IFN \)
\begin{EQA}
	\| \DFN^{-1} \IFN_{1} \uv \|
	& \leq &
	\| \DFN^{-1} \IFN \uv \| + \| \DFN^{-1} (\IFN_{1} - \IFN) \DFN^{-1} \DFN \uv \|
	\leq 
	\| \DFN^{-1} \IFN \uv \| + \dltwbun \, \| \DFN \uv \|
	\\
	& \leq & 
	\| \DFN^{-1} \IFN \uv \| + \dltwbun \| \DFN^{-1} \IFN \uv \| 
	\leq 
	(1 + \dltwbun) \| \DFN^{-1} \IFN \uv \| \, ,
	\qquad
\label{uciuvcdiu3ery7httrwbgfcy}
\end{EQA}
and \eqref{uciuvcdiu3eoooodffcy} follows.
Similarly
\begin{EQA}
	\| \DFN \, (\IFN_{1}^{-1} - \IFN^{-1}) \uv \| 
	& = &
	\| \DFN \, \IFN_{1}^{-1} (\IFN_{1} - \IFN) \IFN^{-1} \uv \|
	=
	\| \DFN \, \IFN_{1}^{-1} \DFN \,\, \DFN^{-1} (\IFN_{1} - \IFN) \DFN^{-1} \, \DFN \, \IFN^{-1} \uv \|
	\\
	& \leq &
	\| \DFN^{-1} \, (\IFN_{1} - \IFN) \, \DFN^{-1} \| \,\,
	\| \DFN \, \IFN_{1}^{-1} \, \DFN \| \,\, \| \DFN \, \IFN^{-1} \uv \|
	\leq 
	\frac{\dltwbun}{1 - \dltwbun} \| \DFN \, \IFN^{-1} \uv \|
\label{rtiuru8bttg3hfy7vrgf}
\end{EQA}
and \eqref{uciuvcdiu3eoooodffcym} follows as well.
\end{proof}



Definition \eqref{ygtuesdfhiwdsoif9ruta} implies the following bound.
\begin{lemma}
\label{Lsemidual}
For any \( \nuiv \in \Nui \) and any linear mapping \( \QP \), it holds
\begin{EQA}
	\| \QP \IFT_{\targv\nuiv} (\nuiv - \nuivs) \|
	& \leq &
	\| \QP \IFT_{\targv\nuiv} \, \HFN^{-1} \|_{\dual} \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, .
\label{difkjv78frhjrjhfh6wekd}
\end{EQA}
\end{lemma}

The next lemma shows that \( \Av_{\nuiv} = \nabla \fs_{\nuiv}(\targvs) \) is nearly linear in \( \nuiv \).

\begin{lemma}
\label{LvarDVa}
Assume \eqref{c6ceyecc5e5etcT2}.
Then
\begin{EQA}
	\| \DFN^{-1} \{ \Av_{\nuiv} + \IFT_{\targv\nuiv} (\nuiv - \nuivs) \} \|
	& \leq &
	\frac{\dltwun}{2} \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} \, .
\label{4cbijjm09j9hhrjfifkrs3}
\end{EQA}
and with \( \crossgrad \) from \eqref{f8vuehery6gv65ftehwee1}, it holds
\begin{EQA}
	\| \DFN^{-1} \Av_{\nuiv} \|
	& \leq &
	\Bigl( \| \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1} \|_{\dual} 
	+ \frac{\dltwun}{2} \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \Bigr) \, \| \HFN (\nuiv - \nuivs) \|_{\nano}
	\\
	& \leq &
	\crossgrad \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, .
\label{4cbijjm09j9hhrjfifkrs}
\end{EQA}
\end{lemma}

\begin{proof}
Fix \( \nuiv \in \Nui \) and define \( \av_{\nuiv}(t) \eqdef \Av_{\nuivs + t (\nuiv - \nuivs)} \).
Then \( \av_{\nuiv}(0) = \Av_{\nuivs} = 0 \), \( \av_{\nuiv}(1) = \Av_{\nuiv} \), 
and
\begin{EQA}
	\av_{\nuiv}(1) - \av_{\nuiv}(0) 
	&=&
	\int_{0}^{1} \av'_{\nuiv}(t) \, dt \, ,
\label{dsf7hgduw3heiuwed53ww3}
\end{EQA}
where \( \av'_{\nuiv}(t) = \frac{d}{dt} \av_{\nuiv}(t) \) for \( t \in [0,1] \).
%Condition \eqref{c6ceyecc5e5etcT1} ensures
%\begin{EQA}
%	\bigl| \langle \av'_{\nuiv}(t), \zv \rangle \bigr|
%	&=&
%	\bigl| \bigl\langle \nabla_{\targv\nuiv}^{2} \fs(\targvs,\nuivs + t (\nuiv - \nuivs)), \zv \otimes (\nuiv - \nuivs) \bigr\rangle \bigr|
%	\leq 
%	\crossgrad \, \| \DFN \zv \| \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, .
%\label{5cbgcfyt6webhwefuy62}
%\end{EQA}
%This implies 
%%by \( \DFN^{2} \leq \, \IFN \) 
%\begin{EQA}
%	\| \DFN^{-1} \av'_{\nuiv}(t) \|
%	&=&
%	\sup_{\zv \colon \| \zv \| \leq 1} \bigl| \langle \DFN^{-1} \av'_{\nuiv}(t), \zv \rangle \bigr|
%	=
%	\sup_{\zv \colon \| \zv \| \leq 1}  
%		\bigl| \langle \av'_{\nuiv}(t), \DFN^{-1} \zv \rangle \bigr|
%	\\
%	& \leq &
%	\crossgrad \sup_{\zv \colon \| \zv \| \leq 1}
%	\| \zv \| \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, 
%	=
%	\crossgrad \| \HFN (\nuiv - \nuivs) \|_{\nano} \,
%\label{bje4f7hj4g8mnw3furtf}
%\end{EQA}
%yielding \eqref{4cbijjm09j9hhrjfifkrs}.
Similarly, by \( \av'_{\nuiv}(0) = - \IFT_{\targv\nuiv} (\nuiv - \nuivs) \), we derive 
\begin{EQA}
	\av_{\nuiv}(1) - \av_{\nuiv}(0) - \av'_{\nuiv}(0)
	&=&
	\int_{0}^{1} (\av'_{\nuiv}(t) - \av'_{\nuiv}(0)) \, dt
	=
	\int_{0}^{1} (1 - t) \, \av''_{\nuiv}(t) \, dt \, ,
\label{g8eh35fgtg7t76868jdy}
\end{EQA}
where 
\( \av''_{\nuiv}(t) = \frac{d^{2}}{dt^{2}} \av_{\nuiv}(t) \).
By condition \nameref{LLpT3ref} 
\begin{EQA}
	\bigl| \langle \av''_{\nuiv}(t), \zv \rangle \bigr|
	&=&
	\bigl| \bigl\langle \nabla_{\targv\nuiv\nuiv}^{3} \fs(\targvs,\nuivs + t (\nuiv - \nuivs)), \zv \otimes (\nuiv - \nuivs)^{\otimes 2} \bigr\rangle \bigr|
	\leq 
	\dltwun \, \| \DFN \zv \| \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} \, 
\label{5cbgcfyt6webhwefuy6}
\end{EQA}
and hence,
%by \( \DFN^{2} \leq \, \IFN \) 
\begin{EQA}
	\| \DFN^{-1} \av''_{\nuiv}(t) \|
	&=&
	\sup_{\zv \colon \| \zv \| \leq 1} \bigl| \langle \DFN^{-1} \av''_{\nuiv}(t), \zv \rangle \bigr|
	=
	\sup_{\zv \colon \| \zv \| \leq 1}  
		\bigl| \langle \av''_{\nuiv}(t), \DFN^{-1} \zv \rangle \bigr|
	\\
	& \leq &
	\dltwun \sup_{\zv \colon \| \zv \| \leq 1}
	\| \zv \| \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} \, 
	=
	\dltwun  \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} \, .
\label{hgvytew3hw36fdfnhrg}
\end{EQA}
This yields
\begin{EQA}
	\| \DFN^{-1} \{ \Av_{\nuiv} + \IFT_{\targv\nuiv} (\nuiv - \nuivs) \} \|
	& \leq &
	\dltwun \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} \, \int_{0}^{1} (1 - t) \, dt
	\leq 
	\frac{\dltwun \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}}{2} \, 
\label{4cbijjm09j9hhrjfifkr}
\end{EQA}
as claimed in \eqref{4cbijjm09j9hhrjfifkrs3}. 
Lemma~\ref{Lsemidual} implies \eqref{4cbijjm09j9hhrjfifkrs}.
\end{proof}

\noindent
Now Proposition~\ref{PbiassemiN} helps to show \eqref{rhDGtuGmusGU0a2spt} and to bound
\( \targv_{\nuiv} - \targvs + \IFN_{\nuiv}^{-1} \Av_{\nuiv} \).

\begin{lemma}
If \( \dltwbun = \dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} < 1 \) then
\begin{EQA}
	\| \DFN (\targv_{\nuiv} - \targvs) \|
	& \leq &
	\frac{3}{2} \| \DFN \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \| 
	\leq 
	\frac{3 \crossgrad}{2(1 - \dltwbun)} \, \| \HFN (\nuiv - \nuivs) \|_{\nano}\,. 
\label{rhDGtuGmusGU0a2sp}
\end{EQA}
Moreover, 
\begin{EQA}
	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs + \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
	& \leq &
	\frac{3 \crossgrad^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} \, 
	\| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
	\, .
	\qquad
\label{d73jejg7tre3fdy3fujell}
\end{EQA}
\end{lemma}

\begin{proof}
%First rescale \( \DFN \) to reduce the proof to the case \( \dmax = 1 \).
By \( \DFN^{2} \leq \IFN \), \eqref{8c7c67cc6c63kdldlvvudw},
\eqref{uciuvcdiu3eoooodffcym} of Lemma~\ref{LIFvari}, and \eqref{4cbijjm09j9hhrjfifkrs} 
\begin{EQA}
	\| \DFN \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|
	& \leq &
	\| \DFN \, \IFN_{\nuiv}^{-1} \DFN \| \,\, \| \DFN^{-1} \Av_{\nuiv} \|
	\leq 
	\frac{1}{1 - \dltwbun} \, \| \DFN^{-1} \Av_{\nuiv} \|
	\leq 
	\frac{\crossgrad}{1 - \dltwbun} \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, .
\label{6dvgycuw76yeficf7wnfo}
\end{EQA}
This and the conditions of the proposition enable us to apply Proposition~\ref{PbiassemiN} which implies \eqref{rhDGtuGmusGU0a2sp} and
\begin{EQA}
	&& \nquad
	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs + \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
	\leq 
	\frac{3 \dltwu_{3}}{4} \, \| \DFN \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{2}
	\leq 
	\frac{3 \crossgrad^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} \, \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
	\, .
\label{suhyd78wyedw378yedh2}
\end{EQA}
This completes the proof.
\end{proof}


%
%
%\begin{lemma}
%It holds with \( \varrho = \| \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1} \|_{\dual} \)
%and \( \dltwbun = \, \dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} < 1 \)
%\begin{EQA}
%	&& \nquad
%	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs - \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
%	\leq
%	\frac{\dltwu_{3}}{(1 - \dltwbun)^{2}} \, 
%	\Bigl( \varrho^{2} \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} 
%		+ \frac{3 \dltwun^{2}}{4} \| \HFN (\nuiv - \nuivs) \|_{\nano}^{4} 
%	\Bigr)
%	\\
%	& \leq &
%	\frac{\dltwu_{3}}{(1 - \dltwbun)^{2}} \, 
%	\Bigl( \varrho^{2} + \frac{3 \dltwun^{2} \, \rru^{2}}{4} \Bigr) \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
%	\, .
%	\qquad
%\label{d73jejg7tre3fdy3fujelld}
%\end{EQA}
%\end{lemma}
%
%\begin{proof}
%First rescale \( \DFN \) to reduce the proof to the case \( \dmax = 1 \).
%Then \( \DFN^{2} \leq \IFN \) and by \eqref{8c7c67cc6c63kdldlvvudw}, \eqref{uciuvcdiu3eoooodffcym},
%and \eqref{usucxy88u7vjwdodx} 
%\begin{EQA}
%	\| \DFN \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|
%	& \leq &
%	\frac{1}{1 - \dltwbun} \, \| \DFN \, \IFN^{-1} \Av_{\nuiv} \|
%	\leq 
%	\frac{1}{1 - \dltwbun} \, \| \DFN^{-1} \Av_{\nuiv} \|
%	\leq 
%	\frac{1}{1 - \dltwbun} \, \Bigl( \varrho \, \rru + \frac{\dltwun}{2} \rru^{2} \Bigr) \, .
%\label{6dvgycuw76yeficf7wnfo}
%\end{EQA}
%This and the conditions of the proposition enable us to apply Proposition~\ref{PbiassemiN}.
%The use of \( \frac{3}{4} (a+b)^{2} \leq a^{2} + 3 b^{2} \) for any \( a,b \), 
%and of the bound \eqref{jhcvu7ejdytur39e9frtfw} yields with \( \AUv_{\nuiv} \eqdef \IFT_{\targv\nuiv} (\nuiv - \nuivs) \)
%\begin{EQA}
%	&& \nquad
%	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs - \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
%	\leq 
%	\frac{3 \dltwu_{3}}{4} \, \| \DFN \, \IFN_{\nuiv}^{-1} \Av_{\nuiv} \|^{2}
%	\leq 
%	\frac{3 \dltwu_{3}}{4} \, \| \DFN \, \IFN_{\nuiv}^{-1} \DFN \|^{2} \, \| \DFN^{-1} \Av_{\nuiv} \|^{2}
%	\\
%	& \leq &
%	\dltwu_{3} \, \| \DFN \, \IFN_{\nuiv}^{-1} \DFN \|^{2} \, 
%	\Bigl( \| \DFN^{-1} \AUv_{\nuiv} \|^{2} + 3 \| \DFN^{-1} (\Av_{\nuiv} - \AUv_{\nuiv}) \|^{2} \Bigr)
%	\, ,
%\label{suhyd78wyedw378yedh}
%\end{EQA}
%where by \eqref{s8dfy8weiu3re5gdh36b} 
%\( \| \DFN^{-1} \AUv_{\nuiv} \| \leq \varrho \| \HFN (\nuiv - \nuivs) \|_{\nano} \).
%The obtained bounds together with \eqref{4cbijjm09j9hhrjfifkrs} and \eqref{g98g75re3gf76r4egu4ee} imply 
%\begin{EQA}[c]
%	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs - \IFN_{\nuiv}^{-1} \Av_{\nuiv}) \|
%	\leq 
%	\frac{\dltwu_{3}}{(1 - \dltwbun)^{2}} \, 
%	\Bigl( \varrho^{2} \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2} 
%		+ \frac{3 \, \dltwun^{2}}{4} \| \HFN (\nuiv - \nuivs) \|_{\nano}^{4} 
%	\Bigr)
%	\, ,
%\label{suhyd78wyedw378yedhh}
%\end{EQA}
%and \eqref{d73jejg7tre3fdy3fujell} follows.
%\end{proof}


Now we can finalize the proof of the proposition.
With \( \AUv_{\nuiv} \eqdef - \IFT_{\targv\nuiv} (\nuiv - \nuivs) \), it holds
\begin{EQA}
	&& \nquad
	\targv_{\nuiv} - \targvs + \IFN^{-1} \AUv_{\nuiv}
	=
	\targv_{\nuiv} - \targvs + \IFN_{\nuiv}^{-1} \Av_{\nuiv}
	- \IFN_{\nuiv}^{-1} \Av_{\nuiv}
	+ \IFN^{-1} \AUv_{\nuiv} 
	\\
	& = &
	\targv_{\nuiv} - \targvs + \IFN_{\nuiv}^{-1} \Av_{\nuiv}
	- \IFN_{\nuiv}^{-1} (\Av_{\nuiv} - \AUv_{\nuiv}) 
	- (\IFN_{\nuiv}^{-1} - \IFN^{-1}) \AUv_{\nuiv}
	\, .
\label{36gfijh94ejdvtwekoDg}
\end{EQA}
The use of \eqref{8c7c67cc6c63kdldlvvudw} and \eqref{f8vuehery6gv65ftehwee} yields
\begin{EQA}
	&& \! \! \! \! \! \! \! \! 
	\| \DFN^{-1} \IFN_{\nuiv} (\IFN^{-1} - \IFN_{\nuiv}^{-1}) \AUv_{\nuiv} \|
	= 
	\| \DFN^{-1} (\IFN - \IFN_{\nuiv}) \IFN^{-1} \AUv_{\nuiv} \|
	\\
	& \leq &
	\| \DFN^{-1} (\IFN - \IFN_{\nuiv}) \DFN^{-1} \| \,\, 
	\| \DFN \, \IFN^{-1} \DFN \| \,\, \| \DFN^{-1} \IFT_{\targv\nuiv} \HFN^{-1} \|_{\dual} \,\, \| \HFN (\nuiv - \nuivs) \|_{\nano}
	\\
	& \leq &
	\dltwunn \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \, \,
	\crossnorm \, \| \HFN (\nuiv - \nuivs) \|_{\nano}.
	\qquad
\label{jufuf7yfy7tg643yrh}
\end{EQA}
This together with \eqref{4cbijjm09j9hhrjfifkrs} and \eqref{d73jejg7tre3fdy3fujell} implies
\begin{EQA}[c]
	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs + \IFN^{-1} \AUv_{\nuiv}) \|
	\leq 
	\Bigl\{ \frac{3 \crossgrad^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} \, 
	+ \crossnorm \, \dltwunn + \frac{\dltwun}{2}
	\Bigr\} \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
	\, .
\label{7tfce7sdfy7w7y73wrytk3f7}
\end{EQA}
The use of \eqref{uciuvcdiu3eoooodffcy} allows to bound
\begin{EQA}[c]
	\| \DFN^{-1} \IFN (\targv_{\nuiv} - \targvs + \IFN^{-1} \AUv_{\nuiv}) \|
	\leq
	\frac{1}{1 - \dltwbun} \, 
	\| \DFN^{-1} \IFN_{\nuiv} (\targv_{\nuiv} - \targvs + \IFN^{-1} \AUv_{\nuiv}) \| 
	\, ,
\label{9jjjjh3d4dd32x32sg3thj}
\end{EQA}
and \eqref{36gfijh94ejdvtwekoise} follows.
% by \( \dltwbun \leq \dltwbund \).
\end{proof}


\begin{remark}
\label{Rdmax2}
An extension to the case \( \DFN^{2} \leq \dmax^{2} \IFN \) can be done by replacing everywhere
\( \dltwu_{3} \),
\( \dltwun \),
\( \dltwunn \),
\( \dltwuns \),
\( \crossnorm \),
\( \crossgrad \) with \( \dmax^{3} \dltwu_{3} \), \( \dmax \, \dltwun \), 
\( \dmax^{2} \dltwunn \), 
\( \dmax \, \dltwuns \), 
\( \dmax^{-1} \crossnorm \), 
\( \dmax^{-1} \crossgrad \)
respectively.
\end{remark}

\Subsection{A linear perturbation}
Let \( \fn(\targv,\nuiv) \) be a linear perturbation of \( \fs(\targv,\nuiv) \):
\begin{EQA}
	\fn(\targv,\nuiv) - \fn(\targvs,\nuivs)
	&=&
	\fs(\targv,\nuiv) - \fn(\targvs,\nuivs) + \langle \AAv,\targv - \targvs \rangle + \langle \CCv,\nuiv - \nuivs \rangle ;
\label{s6cdt76ws6656ysjwsdftc6}
\end{EQA}
cf. \eqref{4hbh8njoelvt6jwgf09}.
Let also \( \Nui \) be given by \eqref{6chbdtw2hydfuguye4223w23} and \( \nuiv \in \Nui \).
We are interested in quantifying the distance between \( \targvs \) and \( \targvn_{\nuiv} \), where 
\begin{EQA}
	\targvn_{\nuiv}
	& \eqdef &
	\argmax_{\targv} \fn(\targv,\nuiv) .
\label{8dcudxjd5t6t5mkwsyddf}
\end{EQA}
The linear perturbation \( \langle \CCv,\nuiv - \nuivs \rangle \) does not depend on \( \targv \) and it can be ignored.



\begin{proposition}
\label{Pconcsupp}
For \( \nuiv \in \Nui \),
assume the conditions of Proposition~\ref{PsemiAvex} and let 
\begin{EQA}[c]
	\dltwbun \eqdef \dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} \leq 1/4 \, .
\end{EQA}
Then 
\begin{EQA}
	\| \DFN (\targvn_{\nuiv} - \targvs) \|
	& \leq &
	\frac{3 }{2(1 - \dltwbun)} \, 
	\bigl( \crossgrad \, \| \HFN (\nuiv - \nuivs) \|_{\nano} + \| \DFN^{-1} \AAv \| \bigr) 
\label{ysd7euwejfg653wthf873k}
\end{EQA}
and for any linear mapping \( \QP \), it holds with 
\( \dltwuns \) from \eqref{36gfijh94ejdvtwekoised} 
%and \( \| \HFN (\nuiv - \nuivs) \|_{\nano} = \| \HFN (\nuiv - \nuivs) \|_{\nano} \)
\begin{EQA}[l]
	\!\!\!
	\| \QP \{ \targvn_{\nuiv} - \targvs + \IFN^{-1} \IFT_{\targv\nuiv} (\nuiv - \nuivs) - \IFN^{-1} \AAv \} \|
	\\
	\leq 
	\| \QP \, \IFN^{-1} \DFN \| \, \Bigl( \dltwuns \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
		+ 2 \dltwu_{3} \, \| \DFN \, \IFN^{-1} \AAv \|^{2}
		+ \frac{4\dltwunn}{3} \, \| \DFN \, \IFN^{-1} \AAv \| \, \| \HFN (\nuiv - \nuivs) \|_{\nano}
	\Bigr)	
	\\
	\leq 
	\| \QP \, \IFN^{-1} \DFN \| \, \Bigl\{ (\dltwuns + \dltwunn) \, \| \HFN (\nuiv - \nuivs) \|_{\nano}^{2}
		+ (2 \dltwu_{3} + \dltwunn/2) \, \| \DFN \, \IFN^{-1} \AAv \|^{2}
	\Bigr\}	
	\, .
	\qquad 
\label{usdhyw6hikhurnetr256}
\end{EQA}
\end{proposition}

\begin{proof}
%Let us fix any \( \nuiv \in \Nui \).
Proposition~\ref{PbiassemiN} applied to \( \fs_{\nuiv}(\targv) \) and 
\( \fn_{\nuiv}(\targv) = \fs_{\nuiv}(\targv) - \langle \AAv, \targv \rangle \) implies  by \eqref{uciuvcdiu3eoooodffcym}
\begin{EQA}
	\| \DFN (\targvn_{\nuiv} - \targv_{\nuiv}) \|
	& \leq &
	\frac{3}{2} \| \DFN \, \IFN_{\nuiv}^{-1} \AAv \|
	\leq 
	\frac{3}{2(1 - \dltwbun)} \| \DFN^{-1} \AAv \| 
	\, .
\label{djvhehfief6yh3jfgiu2}
\end{EQA}
This and \eqref{rhDGtuGmusGU0a2spt} imply \eqref{ysd7euwejfg653wthf873k}.
Next we check \eqref{usdhyw6hikhurnetr256} using the decomposition
\begin{EQA}
	&& \nquad
	\targvn_{\nuiv} - \targvs + \IFN^{-1} \IFT_{\targv\nuiv} (\nuiv - \nuivs) - \IFN^{-1} \AAv
	\\
	&=&
	(\targvn_{\nuiv} - \targv_{\nuiv} - \IFN_{\nuiv}^{-1} \AAv) 
	+ (\IFN_{\nuiv}^{-1} \AAv - \IFN^{-1} \AAv)
	+ \{ \targv_{\nuiv} - \targvs + \IFN^{-1} \IFT_{\targv\nuiv} (\nuiv - \nuivs) \} 
	\, .
\label{yhdt56swhew454erjhfgi}
\end{EQA}
Proposition~\ref{PsemiAvex} evaluates the last term.
Lemma~\ref{L3IFNNui} helps to bound
\begin{EQA}
	\| \DFN^{-1} \IFN (\IFN_{\nuiv}^{-1} - \IFN^{-1}) \IFN_{\nuiv} \, \DFN^{-1} \|
	& = &
	\| \DFN^{-1} (\IFN_{\nuiv} - \IFN) \DFN^{-1} \|
	\leq 
	\dltwunn \| \HFN (\nuiv - \nuivs) \|_{\nano} 
	\, .
\label{cuyedgfcuedgtfbvj}
\end{EQA}
This yields 
\begin{EQA}
	\| \QP (\IFN_{\nuiv}^{-1} - \IFN^{-1}) \AAv \|
	& \leq &
	\| \QP \, \IFN^{-1} \DFN \| 
	\, \| \DFN^{-1} \IFN_{\nuiv} (\IFN_{\nuiv}^{-1} - \IFN^{-1}) \IFN \, \DFN^{-1} \|
	\, \| \DFN \, \IFN_{\nuiv}^{-1} \AAv \|
	\\
	& \leq &
	\| \QP \, \IFN^{-1} \DFN \| 
	\, \dltwunn \, \| \HFN (\nuiv - \nuivs) \|_{\nano} \,
	\, \frac{1}{1 - \dltwbun} \| \DFN \, \IFN^{-1} \AAv \|
	\, .
\label{7duewjf87he4fyjwucyfne}
\end{EQA}
Moreover, 
for \( \epsv_{\nuiv} \eqdef \targvn_{\nuiv} - \targv_{\nuiv} - \IFN_{\nuiv}^{-1} \AAv \), it holds
\begin{EQA}
	\| \DFN^{-1} \IFN_{\nuiv} \, \epsv_{\nuiv} \|
	& \leq &
	\frac{3 \dltwu_{3}}{4} \| \DFN \, \IFN_{\nuiv}^{-1} \AAv \|^{2}  
	\leq 
	\frac{3 \dltwu_{3}}{4(1 - \dltwbun)^{2}} \| \DFN \, \IFN^{-1} \AAv \|^{2}
	\, ,
\label{ud82uegkftryyde6ewhde}
\end{EQA} 
and by \eqref{uciuvcdiu3eoooodffcym} and \( \dltwbun \leq 1/4 \)
\begin{EQA}
	\| \QP \, \epsv_{\nuiv} \|
	& \leq &
	\| \QP \, \IFN^{-1} \DFN \| \,\, \| \DFN^{-1} \IFN \, \epsv_{\nuiv} \|
	\leq 
	\| \QP \, \IFN^{-1} \DFN \| \, \frac{1 - \dltwbun}{1 - 2 \dltwbun} \, \| \DFN^{-1} \IFN_{\nuiv} \, \epsv_{\nuiv} \|
	\\
	& \leq &
	\| \QP \, \IFN^{-1} \DFN \| \,\, 
	\frac{3 \dltwu_{3}}{4(1 - \dltwbun) (1 - 2 \dltwbun)} \| \DFN \, \IFN^{-1} \AAv \|^{2} 
	\leq 
	\| \QP \, \IFN^{-1} \DFN \| \, 2 \dltwu_{3} \, \| \DFN \, \IFN^{-1} \AAv \|^{2}
	\, .
\label{ysdudhwuw8ey87wejue4bf}
\end{EQA}
The obtained bounds imply \eqref{usdhyw6hikhurnetr256} in view of
\( (4/3)ab \leq a^{2} + b^{2}/2 \) for any \( a,b \).
\end{proof}

\begin{comment}
\Subsection{One-point orthogonality by a linear transform}
\label{Sonepointtrans}
\emph{One-point orthogonality} condition means \( \nabla_{\nuiv} \nabla_{\targv} \, \fs(\prmtvs) = 0 \).
This section explains how
this condition can be enforced for a general function \( \fs \) by 
a linear transform of the nuisance parameter.
We only need a mild \emph{separability condition} which 
assumes that the full-dimensional information matrix
\( \IFT(\prmtv) = - \nabla^{2} \fs(\prmtv) \) is well posed
%can be bounded from below by the block-diagonal matrix 
%\( \blk\{ - \nabla_{\targv\targv}^{2} \fs(\prmtv), - \nabla_{\nuiv\nuiv}^{2} \fs(\prmtv) \} \)
for \( \prmtv = \prmtvs \).

\begin{description}
	\item[\label{IFLref} \( \bb{(\IFT)} \)]
	\emph{%The function \( \fs(\prmtv) \) is strongly concave. 
	The matrix \( \IFT = \IFT(\prmtvs) \) is positive definite 
	and for some constant \( \rhoIF = \rhoIF(\IFT) < 1 \)} % and \( \prmtv = \prmtvs \), it holds}
\begin{EQA}
	\| 
	\IFT_{\targv\targv}^{-1/2} \IFT_{\targv\nuiv} \, \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} \, \IFT_{\targv\targv}^{-1/2} 
	\|
	& \leq &
	\rhoIF^{2}
	< 
	1 .
\label{vcjcfvedt7wdwhesqgghwqLco}
\end{EQA}
\end{description}


\begin{lemma}
\label{Lidentsemi}
Suppose \nameref{IFLref}. 
Then with \( \IFTN \eqdef \blk\{ \IFT_{\targv\targv},\IFT_{\nuiv\nuiv} \} \)
\begin{EQA}
	(1 - \rhoIF) \IFTN
	\leq 
	\IFT
	& \leq &
	(1 + \rhoIF) \IFTN
\label{f6eh3ewfd6ehev65r43tre}
\end{EQA}
and the matrices
\begin{EQA}
	\IFTb_{\targv\targv} 
	& \eqdef &
	\IFT_{\targv\targv} - \IFT_{\targv\nuiv} \, \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} \, ,
	\qquad
	\IFTb_{\nuiv\nuiv}
	\eqdef 
	\IFT_{\nuiv\nuiv} - \IFT_{\nuiv\targv} \, \IFT_{\targv\targv}^{-1} \, \IFT_{\targv\nuiv} \, ,
	\qquad
\label{ljhy6furf4rfeder8jfu8rd}
\end{EQA}
satisfy
\begin{EQA}
	(1 - \rhoIF^{2}) \, \IFT_{\targv\targv}
	\leq 
	\IFTb_{\targv\targv}
	& \leq &
	\IFT_{\targv\targv} \, ,
	\qquad
	(1 - \rhoIF^{2}) \, \IFT_{\nuiv\nuiv}
	\leq 
	\IFTb_{\nuiv\nuiv}
	\leq 
	\IFT_{\nuiv\nuiv} \, .
\label{yg3w5dffctvyry4r7er7dgfe}
\end{EQA}
\end{lemma}

\begin{proof}
Define \( \DFN^{2} = \IFT_{\targv\targv} \), \( \HFN^{2} = \IFT_{\nuiv\nuiv} \),
\( \IFTN = \blk\{ \DFN^{2},\HFN^{2} \} \), \( \AFN = \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1} \), and consider the matrix 
\begin{EQA}
	\IFTN^{-1/2} \IFT \, \IFTN^{-1/2} - \Id_{\dimttl}
	&=&
	\begin{pmatrix}
		0 & \DFN^{-1} \IFT_{\targv\nuiv} \, \HFN^{-1}
		\\
		\HFN^{-1} \IFT_{\nuiv\targv} \, \DFN^{-1} & 0
	\end{pmatrix}
	=
	\begin{pmatrix}
		0 & \AFN
		\\
		\AFN^{\T} & 0
	\end{pmatrix} .
\label{gswrew35e35e35e5txzgtqw}
\end{EQA}
Condition \eqref{vcjcfvedt7wdwhesqgghwqLco} implies \( \| \AFN \AFN^{\T} \| \leq \rhoIF^{2} \) and hence,
\begin{EQA}
	- \rhoIF \, \Id_{\dimttl} 
	& \leq &
	\IFTN^{-1/2} \IFT \, \IFTN^{-1/2} - \Id_{\dimttl} 
	\leq 
	\rhoIF \, \Id_{\dimttl} \, .
\label{ye376evhgder52wedsytg}
\end{EQA}
Moreover,
\begin{EQA}
	\IFTb_{\targv\targv} 
	& = &
	\IFT_{\targv\targv} - \IFT_{\targv\nuiv} \, \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} 
	=
	\DFN (\Id_{\dimp} - \AFN \AFN^{\T}) \DFN 
	\geq 
	(1 - \rhoIF^{2}) \DFN^{2} \, ,
\label{ljhy6furf4jfu8rdfcweerdd}
\end{EQA}
and similarly for \( \IFTb_{\nuiv\nuiv} \).
\end{proof}

\noindent
Note that \( \DFN^{2} = \IFT_{\targv\targv} \) is the \( \targv\targv \)-block of \( \IFT = - \nabla^{2} \fs(\prmtvs) \), while 
\( \DFNb^{-2} \eqdef \IFTb_{\targv\targv}^{-1} \) from \eqref{ljhy6furf4rfeder8jfu8rd} 
is the \( \targv\targv \)-block of \( \IFT^{-1} \)
by the formula of block-inversion.
The matrices \( \DFN^{2} \) and \( \DFNb^{2} \) only coincide if the matrix \( \IFT \) is of block-diagonal structure.

\begin{lemma}
\label{Onepointorto}
%
With block representation \eqref{hwe78yf2diwe76tfw67etfwtbso},
define \( \CFT = \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} \) and
\begin{EQ}[rcl]
	\nuov 
	&=& 
	\nuiv + \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} \, (\targv - \targvs) 
	=
	\nuiv + \CFT \, (\targv - \targvs) ,
	\\
	\fsb(\targv,\nuov)
	&=&
	\fs(\targv,\nuiv) 
	=
	\fs(\targv,\nuov - \CFT \, (\targv - \targvs)) .
\label{0vcucvf653nhftdreyenwe}
\end{EQ}
Then 
\begin{EQA}
	\nabla_{\nuov} \nabla_{\targv} \, \fsb(\targv,\nuov) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}}
	&=&
	0 \, ,
	\quad
%\label{jdgyefe74erjscgygfydhw}
	\nabla_{\targv\targv}^{2} \, \fsb(\targv,\nuov) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}} 
	=
	\DFNb^{2} \, ,
	\quad
	\nabla_{\nuov\nuov}^{2} \, \fsb(\targv,\nuov) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}} 
	=
	\HFN^{2} 
	 \, .
	 \qquad
\label{n6d2fgujrt6fgfrjrd}
\end{EQA}
\end{lemma}

\begin{proof}
By definition \( \fs(\targv,\nuiv) = \fs(\targv,\nuov - \CFT \, \targv) \), and it is straightforward to check that
\begin{EQA}
	\nabla_{\nuov} \nabla_{\targv} \, \fsb(\targv,\nuov) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}}
%	_{\targv=\targvs,\nuov=\nuivs}
	=
	\nabla_{\nuov} \nabla_{\targv} \, \fs(\targv,\nuov 
	- \CFT \, (\targv - \targvs)) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}} 
	&=&
	0 .
	\qquad
\label{jdgyefe74erjscgygfydhwp}
\end{EQA}
Similarly
\begin{EQA}
	\nabla_{\targv\targv}^{2} \, \fsb(\prmtvs) 
	=
	\nabla_{\targv\targv}^{2} \, \fs(\targv,\nuov - \CFT \, (\targv - \targvs)) \Big|_{\binomb{\targv=\targvs}{\nuov=\nuivs}}
	&=&
	\IFT_{\targv\targv} - \IFT_{\targv\nuiv} \, \IFT_{\nuiv\nuiv}^{-1} \, \IFT_{\nuiv\targv} 
	=
	\DFNb^{2} \, 
\label{d3gr7hyrfygieshfdhfjk}
\end{EQA}
and \( \nabla_{\nuov\nuov}^{2} \, \fsb(\prmtvs) = \nabla_{\nuiv\nuiv}^{2} \, \fs(\prmtvs) = \HFN^{2} \)
as required.
\end{proof}


%Note that \( \DFNb^{-2} \) is the \( \targv\targv \)-block of \( \IFT^{-1} \) by the formula of block-inversion.
We can summarize that the linear transform \eqref{0vcucvf653nhftdreyenwe} ensures the one-point orthogonality
condition \( \nabla_{\nuov} \nabla_{\targv} \, \fsb(\prmtvs) = 0 \) for the function 
\( \fsb(\targv,\nuov) = \fs(\targv,\nuov - \cc{C} \, (\targv - \targvs)) \) with 
\( - \nabla_{\targv\targv}^{2} \fsb(\prmtvs) = \DFNb^{2} \).
For this function, one can redefine all the characteristics including
\begin{EQA}
	\breve{\feta}_{\nuov}
	& \eqdef &
	\max_{\targv} \fsb(\targv,\nuov),
	\\
	\targvb_{\nuov}
	& \eqdef &
	\argmax_{\targv} \fsb(\targv,\nuov),
	\\
	\DFNb_{\nuov}^{2}
	& \eqdef &
	- \nabla_{\targv\targv}^{2} \fsb(\targvb_{\nuov},\nuov). 
\label{nfyehendcghegwdgqgqngd}
\end{EQA}
If \( \fs(\targv,\nuiv) \) is quadratic, then orthogonality can be achieved by a linear transform of the nuisance parameter \( \nuiv \).
In particular, for \( \fs(\prmtv) = \fs(\prmtvs) - (\prmtv - \prmtvs)^{\T} \IFT \, (\prmtv - \prmtvs)/2 \) quadratic, it holds with 
\( \HFN^{2} = \IFT_{\nuiv\nuiv} \)
\begin{EQA}
	\fsb(\targv,\nuov)
	&=&
	\fs(\prmtvs) - \frac{\| \DFNb (\targv - \targvs) \|^{2}}{2}  - \frac{\| \HFN (\nuov - \nuivs) \|^{2}}{2}  \, ,
\label{ovjv8734mfdgdytwndbgg}
\end{EQA}
and hence
\begin{EQA}
	\targvb_{\nuov}
	& \equiv &
	\targvs,
	\qquad
	\DFNb_{\nuov}^{2}
	\equiv 
	\DFNb^{2} ,
	\qquad
	\breve{\feta}_{\nuov}
	=
	- \frac{\| \HFN (\nuov - \nuivs) \|^{2}}{2} \, .
\label{lfibubgue5t335r6tt7ehw}
\end{EQA}

%\Subsection{Semiorthogonality}

For a general smooth function \( \fs(\prmtv) = \fs(\targv,\nuiv) \) satisfying \nameref{LLsT3ref}, 
we expect that these identities are fulfilled
in a local vicinity of \( \prmtvs \) up to the error of quadratic approximation.
The next result quantifies this guess.

\begin{proposition}
\label{PonepptLL}
Let \( \fs(\prmtv) \) satisfy \nameref{IFLref}, \nameref{LLsT3ref}, and
\begin{EQA}[c]
	(1 - \rhoIF)^{-1} \, \dltwu_{3} \, \rr
	\leq 
	1/3 .
\label{8uiiihkkcrdrdteggcjcjdan}
\end{EQA} 
Then for any \( \nuov \) with \( \| \HFN (\nuov - \nuovs) \| \leq \rr \) and any linear mapping 
\( \QP \colon \R^{\dimp} \to \R^{\dimq} \), the bias \( \targvb_{\nuov} - \targvs \) satisfies
with \( \DFNb^{2} = \IFTb_{\targv\targv} \) from \eqref{ljhy6furf4rfeder8jfu8rd} 
\begin{EQA}
	\| \QP (\targvb_{\nuov} - \targvs) \|
	& \leq &
	\| \QP \, \DFNb^{-1} \| \, \frac{(1 + \dltwu_{3} \, \rr/2)}{2(1 - \dltwu_{3} \, \rr)} \, \dltwu_{3} \, \| \HFN (\nuov - \nuovs) \|^{2} \, .
\label{36gfijh94ejdvtwekoib}
\end{EQA}
In particular, with \( \QP = \DFNb \)
\begin{EQA}
	\| \DFNb (\targvb_{\nuov} - \targvs) \|
	& \leq &
	\frac{(1 + \dltwu_{3} \, \rr/2)}{2(1 - \dltwu_{3} \, \rr)} \, \dltwu_{3} \, \| \HFN (\nuov - \nuovs) \|^{2} \, .
\label{36gfijh94ejdvtwekoDL}
\end{EQA}
\end{proposition}

\begin{proof}
Linear transform \eqref{0vcucvf653nhftdreyenwe} reduces the proof 
to the case with one-point orthogonality. 
Condition \nameref{LLsT3ref} still applies with the same constant \( \dltwu_{3} \).
Condition \eqref{8uiiihkkcrdrdteggcjcjdan} ensures \nameref{LLsoT3ref}, \nameref{LLpT3ref} after
this transform, and the result follows from Proposition~\ref{PsemiAv}.
\end{proof}
\end{comment}


%\Subsection{Semiorthogonality}
%
%This section discusses a special case when the mixed derivative of 
%\( \fs(\targv,\nuiv) \) only depends on \( \targv \):
%\begin{EQA}
%	\nabla_{\nuiv} \nabla_{\targv} \fs(\targv,\nuiv)
%	& \equiv &
%	- \dCross(\targv) ,
%	\qquad
%	\nabla_{\nuiv\nuiv}^{2} \fs(\targv,\nuiv)
%	\equiv 
%	- \dPartial^{2}(\targv),
%\label{0hy533rycirudle}
%\end{EQA}
%for a \( \dimq \times \dimp \)-matrix function \( \dCross(\targv) \) and a positive \( \dimq \times \dimq \)-matrix function 
%\( \dPartial^{2}(\targv) \).
%We also write \( \dCross \) and \( \dPartial^{2} \) in place of \( \dCross(\targvs) \) and \( \dPartial^{2}(\targvs) \).
%Due to the next result, this condition yields a semi-orthogonality of the transformed function \( \fsb(\cdot) \).
%
%\begin{lemma}
%\label{LCrossdervs}
%Assume \eqref{0hy533rycirudle}.
%Then the function \( \fsb(\targv,\nuov) \) from \eqref{0vcucvf653nhftdreyenwe} satisfies the semi-orthogonality condition 
%\begin{EQA}
%	\nabla_{\nuov} \nabla_{\targv} \fsb(\targvs,\nuov)
%	& \equiv &
%	0.
%\label{juifue36fhg65e3yeh}
%\end{EQA}
%Moreover, %with \( \DFNb^{2} = - \nabla_{\targv\targv}^{2} \fsb(\targvs,\nuivs) =  \)
%for any \( \nuov \) with \( (\targvs,\nuov) \in \Upsb \), it holds
%\begin{EQA}[rcccl]
%	\nabla_{\targv} \fsb(\targvs,\nuov)
%	& \equiv &
%	0,
%	\qquad
%	\nabla_{\targv\targv}^{2} \fsb(\targvs,\nuov)
%	& \equiv &
%	\nabla_{\targv\targv}^{2} \fsb(\targvs,\nuivs) .
%\label{klfu87fjhr57765645r}
%\end{EQA}
%If \( \fs(\prmtv) \) is concave in \( \prmtv \) then 
%\begin{EQA}
%	\targvb_{\nuov}
%	& \eqdef &
%	\argmax_{\targv} \fsb(\targv,\nuov)
%	\equiv 
%	\targvs \, .	
%\label{juifue36fhg65e3yehop}
%\end{EQA}
%%and
%%\begin{EQA}
%%	\targv_{\nuiv}
%%	\eqdef
%%	\argmax_{\targv} \fs(\targv,\nuiv)
%%	& \equiv &
%%	\targvs \, .
%%\label{juifue36fhg65e3yehopb}
%%\end{EQA}
%\end{lemma}
%
%\begin{proof}
%Let \( \fsb(\targv,\nuov) \) be defined by \eqref{0vcucvf653nhftdreyenwe}.
%Lemma~\ref{Onepointorto} ensures one-point orthogonality 
%\( \nabla_{\nuov} \nabla_{\targv} \fsb(\prmtvs) = \nabla_{\nuov} \nabla_{\targv} \fsb(\targvs,\nuivs) = 0 \).
%Moreover, \eqref{0hy533rycirudle} yields \( \CFT = \dPartial^{-2} \, \dCross \).
%Now consider \( \nabla_{\nuov} \nabla_{\targv} \fsb(\targvs,\nuov) \).
%It holds by \eqref{0hy533rycirudle} and definition \eqref{0vcucvf653nhftdreyenwe}
%\begin{EQA}
%	\nabla_{\nuov} \nabla_{\targv} \fsb(\targvs,\nuov) 
%	&=&
%	\nabla_{\nuov} \nabla_{\targv} \fs(\targv,\nuov - \CFT \, (\targv - \targvs)) \bigg|_{\targv = \targvs}
%	\\
%	&=&
%	\nabla_{\nuov} \nabla_{\targv} \fs(\targvs,\nuov) - \nabla_{\nuov}^{2} \fs(\targvs,\nuov) \CFT
%	=
%	- \dCross + \dPartial^{2} \CFT
%	=
%	0
%\label{ucieruier3dchedndm}
%\end{EQA}
%yielding semi-orthogonality of \( \fsb \).
%Lemma~\ref{Lsemiorto} implies \eqref{klfu87fjhr57765645r} and \eqref{juifue36fhg65e3yehop}.
%\end{proof}
%
%


\Section{Sup-norm expansions for linearly perturbed optimization}
\label{Ssupnormco}
Let \( \fs(\upsv) \) be a concave function and \( \upsvs = \argmax_{\upsv} \fs(\upsv) \).
Define \( \IFT = - \nabla^{2} \fs(\upsvs) = (\IFT_{jm}) \).
Let also \( \fn(\upsv) \) be obtained by a linear perturbation of \( \fs(\upsv) \) as in \eqref{4hbh8njoelvt6jwgf09}
and let \( \upsvn = \argmax_{\upsv} \fn(\upsv) \).
We intend to bound the corresponding change \( \upsvn - \upsvs \) in a sup-norm.
The strategy of the study is to fix one component \( \ups_{j} \) of \( \upsv \) and treat the remaining entries as the nuisance 
parameter.
Fix a metric tensor \( \DFN \) in diagonal form:
\begin{EQA}[c]
	\DFN \eqdef \diag(\DFN_{1}, \ldots, \DFN_{\dimp}).
\label{7dycf8mwdy6ey43hf98yh}
\end{EQA}
Later we assume \( \DFN_{j}^{2} = \IFT_{jj} \).
For each \( j \leq \dimp \), we will use the representation \( \upsv = (\ups_{j},\nuiv_{j}) \), where 
\( \nuiv_{j} \in \R^{\dimp-1} \) collects all the remaining entries of \( \upsv \).
Similarly, define \( \DFN = (\DFN_{j},\HFN_{j}) \) with \( \HFN_{j} = \diag(\DFN_{m}) \) for \( m \neq j \).
%
Define also for some radius \( \rrinf \)
\begin{EQA}[c]
	\Upsd = \{ \upsv \colon \| \DFN (\upsv - \upsvs) \|_{\infty} \leq \rrinf \} 
	=
	\Bigl\{ \upsv \colon \max_{j \leq \dimp} \bigl| \DFN_{j} (\ups_{j} - \upss_{j}) \bigr| 
	\leq \rrinf \Bigr\}.
\label{du7duydy7cy6fc6df3}
\end{EQA}
%Also, for each \( j \leq \dimp \), define
%\begin{EQA}
%	\Nuid_{j}
%	& \eqdef &
%	\bigl\{ \nuiv_{j} \colon \| \HFN_{j}(\nuiv_{j} - \nuivs_{j}) \|_{\infty} \leq \rrinf \bigr\} \, .
%\label{6xdycyvtv544e4seg3df}
%\end{EQA}
Assume the following condition.

\begin{description}
    \item[\label{LLpsupref} \( \bb{(\mathcal{T}_{\infty}^{*})} \)]
      \emph{For each \( j \leq \dimp \), 
     the function \( \fs(\ups_{j},\nuiv_{j}) \) fulfills}
%   \item[\label{LLpsup3ref} \( \bb{(\mathcal{T}_{3,\infty}^{*})} \)]
%      \emph{For each \( j \leq \dimp \), 
%      }
\begin{EQA}[rcl]
	\sup_{\nuiv_{j} \colon \| \HFN_{j} (\nuiv_{j} - \nuivs_{j}) \|_{\infty} \leq \rrinfi} \,\, 
	\sup_{\ups \colon \DFN_{j} |\ups - \upss_{j}| \leq 2\rrinfi} \,
	\frac{\bigl| \nabla_{\ups_{j}\ups_{j} \ups_{j}}^{(3)} \fs(\ups_{j},\nuiv_{j}) \bigr|}
		 {\DFN_{j}^{3}}
	& \leq &
	\dltwu_{3} \, ,
\label{d6f53ye5vry4fddfgsup}
\end{EQA}
\emph{and}
\begin{EQA}[lccl]
	\sup_{\upsv = (\upss_{j},\nuiv_{j}) \in \Upsd} \,
	\sup_{\zv_{j} \in \R^{\dimp-1}} \,
	&
	\frac{| \langle \nabla_{\ups_{j}\ups_{j}\nuiv_{j}}^{(3)} \fs(\upss_{j},\nuiv_{j}), \zv_{j} \rangle |}
		 {\DFN_{j}^{2} \, \| \HFN_{j} \zv_{j} \|_{\infty}}
	& \leq &
	\dltwunn 
	\, ,
\label{c6hyi8ietctwhcsup}
	\\
	\sup_{\upsv = (\upss_{j},\nuiv_{j}) \in \Upsd}  \,
	\sup_{\zv_{j} \in \R_{j}^{\dimp}} \,
	&
	\frac{| \langle \nabla_{\ups_{j}\nuiv_{j}\nuiv_{j}}^{3} \fs(\upss_{j},\nuiv_{j}), \zv_{j}^{\otimes 2} \rangle |}
		 {\DFN_{j} \, \| \HFN_{j} \zv_{j} \|_{\infty}^{2}}
	& \leq &
	\dltwun 
	\, .
	\qquad
\label{c6ceyecc5e5etcT2sup}
\end{EQA}
\end{description}

For the dual norm \( \| \cdot \|_{\dual} \) from \eqref{ygtuesdfhiwdsoif9ruta}, define
\begin{EQA}
	\crosssup
	& \eqdef &
	\max_{j = 1,\ldots,\dimp} \| \DFN_{j}^{-1} \IFT_{\ups_{j},\nuiv_{j}} \, \HFN_{j}^{-1} \|_{\dual} 
	=
	\max_{j = 1,\ldots,\dimp} \,\, \sup_{\| \zv \|_{\infty} \leq 1}
	\| \DFN_{j}^{-1} \IFT_{\ups_{j},\nuiv_{j}} \, \HFN_{j}^{-1} \zv \|
	\, .
	\qquad
\label{7tdsyf8iuwopkrtg4576}
\end{EQA}

\begin{lemma}
\label{Lcrosssup}
It holds
\begin{EQA}[c]
	\crosssup^{2}
	\leq 
	\max_{j = 1,\ldots,\dimp} \frac{1}{\DFN_{j}^{2}}
	\sum_{m \neq j} \frac{\IFT_{jm}^{2}}{\DFN_{m}^{2}} \, .
\end{EQA}
\end{lemma}

\begin{proof}
By definition,
\begin{EQA}[rcl]
	\crosssup^{2}
	& \leq &
	\max_{j = 1,\ldots,\dimp} \,\, \sup_{\| \zv \|_{\infty} \leq 1}
	\sum_{m \neq j} \frac{1}{\DFN_{j}^{2} \, \DFN_{m}^{2}} \, \IFT_{jm}^{2} z_{m}^{2} 
	\leq 
	\max_{j = 1,\ldots,\dimp} \frac{1}{\DFN_{j}^{2}}
	\sum_{m \neq j} \frac{\IFT_{jm}^{2}}{\DFN_{m}^{2}} \,  
\end{EQA}
as claimed.
\end{proof}
%
It is mandatory for the proposed approach that \( \crosssup < 1 \).
% and \( \dltwbun = \dltwunn \, \rrinf < 1 \).
%Moreover, some of results including the final expansion \eqref{usdhyw6hikhurnetrspp2} assume that \( \crosssup \) is small.
%The value \( \dltwuns \) from \eqref{36gfijh94ejdvtwekoised} can be specified as
The next result provides an upper bound on \( \| \upsvd - \upsvs \|_{\infty} \).


\begin{proposition}
\label{Psemibiassup}
Let \( \fs(\upsv) \) be concave function and 
\( \fn(\upsv) \) be a linear perturbation of \( \fs(\upsv) \) with a vector \( \AAv \). 
For a diagonal metric tensor \( \DFN \), assume \( \crosssup < 1 \); see \eqref{7tdsyf8iuwopkrtg4576}. 
Fix 
\begin{EQA}
	\rrinf 
	&=& 
	\frac{\sqrt{2}}{1 - \crosssup} \| \DFN^{-1} \AAv \|_{\infty} 
	\, .
\label{8drywjwuycrt5sdeteyhfuwk}
\end{EQA}
Let \nameref{LLpsupref} hold with this \( \rrinf \) and
\( \dltwun, \dltwunn, \dltwu_{3} \) satisfying  
\begin{EQA}[c]
	\dltwbun = \dltwunn \, \rrinf \leq 1/4 ,
	\qquad
	\dltwun \, \rrinf \leq 1/4 \, ,
	\qquad	
	\dltwunss \| \DFN^{-1} \AAv \|_{\infty} 
	\leq 
	\sqrt{2} - 1
	\, ,
\label{dhfiejfowelocuyehbrf}
\end{EQA}
where
\begin{EQA}[rcl]
	\dltwuns
	& \eqdef &
	\frac{1}{1 - \dltwbun} \, 
	\biggl( \crosssup \, \dltwunn + \frac{\dltwun}{2}
		+ \frac{3(\crosssup + \dltwbun/2)^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} 
%		+ \frac{3\dltwu_{3}\, \dltwun^{2} \, \rru^{2}}{4(1 - \dltwbund)^{2}} 
	\biggr) 
	\, ,
\label{36gfijh94ejdvtwekoisedi}
	\\
	\dltwunss
	& \eqdef &
	2 \dltwu_{3} + \frac{\dltwunn}{2}  + \frac{2(\dltwuns + \dltwunn)}{(1 - \crosssup)^{2}} 
	\, .
\end{EQA}
Then \( \upsvd = \argmax_{\upsv} \fn(\upsv) \) satisfies
\begin{EQA}
	\| \DFN (\upsvd - \upsvs) \|_{\infty}
	\eqdef
	\max_{j \leq \dimp} | \DFN_{j} (\upsd_{j} - \upss_{j}) |
	& \leq &
	\rrinf \, .
\label{7ytdufchskmls7rghnk}
\end{EQA} 
Furthermore, 
\begin{EQA}
\label{usdhyw6hikhurnetrspp}
	\bigl\| \DFN^{-1} \bigl\{ \IFT (\upsvd - \upsvs) - \AAv \bigr\} \bigr\|_{\infty}
	& \leq &
	\dltwunss \, \| \DFN^{-1} \AAv \|_{\infty}^{2} 
	\, ,
	\\
	\bigl\| \DFN (\upsvd - \upsvs - \IFT^{-1} \AAv) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}^{2} 
	\, ,
	\qquad
\label{usdhyw6hikhurnetrspp1}
\end{EQA}
and with \( \Delta \eqdef \Id_{\dimp} - \DFN^{-1} \IFT \, \DFN^{-1} \)
\begin{EQ}[rcl]
	\bigl\| \DFN (\upsvd - \upsvs) - \DFN^{-1} \AAv) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}^{2} + \frac{\crosssup}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}
	\, ,
	\\
	\bigl\| \DFN (\upsvd - \upsvs) - (\Id_{\dimp} + \Delta) \DFN^{-1} \AAv) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}^{2} + \frac{\crosssup^{2}}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}
	\, .
	\qquad
\label{usdhyw6hikhurnetrspp2}
\end{EQ}
\end{proposition}


\begin{remark}
To gain an intuition about the result of the proposition, consider a typical situation with 
\( \dltwun \leq \dltwu_{3} \),
\( \dltwunn \leq \dltwu_{3} \),
\( \dltwbun \leq 1/4 \),
\( 1 - \crosssup \leq 1/\sqrt{2} \).
Then \( \dltwuns \) from \eqref{36gfijh94ejdvtwekoisedi} fulfills \( \dltwuns \leq 1.37 \), and it holds
\( \dltwunss \leq 12 \dltwu_{3} \).
\end{remark}



\begin{proof}
Let us fix any \( j \leq \dimp \), e.g. \( j=1 \).
Represent any \( \upsv \in \Upsd \) as \( \upsv = (\ups_{1},\nuiv_{1}) \), where \( \nuiv_{1} = (\ups_{2},\ldots,\ups_{\dimp})^{\T} \). 
%Define \( \Nuid_{1} = \{ \nuiv_{1} \colon  \max_{j\geq 2} \| \DFN_{j} \ups_{j} \| \leq \rrinf \} \).
By \eqref{7tdsyf8iuwopkrtg4576}
\begin{EQA}
	&& \nquad
	\bigl| \DFN_{1} \IFT_{11}^{-1} \IFT_{\ups_{1}\nuiv_{1}}(\nuiv_{1} - \nuivs_{1}) \bigr|
	\leq 
	\bigl| \DFN_{1}^{-1} \IFT_{\ups_{1}\nuiv_{1}}(\nuiv_{1} - \nuivs_{1}) \bigr|
	\leq 
	\crosssup \, \| \HFN_{1} (\nuiv_{1} - \nuivs_{1}) \|_{\infty}
%	\\
%	& \leq &
%	\sum_{m=2}^{\dimp} \frac{|\IFT_{1m}|}{\DFN_{1} \DFN_{m}} \bigl| \DFN_{m} (\ups_{m} - \upss_{m}) \bigr|
%	\leq 
%	\crosssup \, \max_{m=2,\ldots,\dimp} \bigl| \DFN_{m} (\ups_{m} - \upss_{m}) \bigr|
	\, .
\label{dekweivytre34wfgbc}
\end{EQA}
For any \( \nupv_{1} \), define
\begin{EQA}
	\upsd_{1}(\nupv_{1})
	& \eqdef &
	\argmax_{\ups_{1}} \fn(\ups_{1},\nupv_{1}) .
\label{fifwi9jhrio3jiofcwgyt7we}
\end{EQA}
Now we apply Proposition~\ref{Pconcsupp} 
with \( \QP = \DFN_{1} \), \( \IFN = \IFT_{11} \), \( \HFN = \HFN_{1} = \diag(\DFN_{2},\ldots,\DFN_{\dimp}) \),
and \( \| \HFN_{1} (\nuiv_{1} - \nuivs_{1}) \|_{\infty} \leq \rrinf \).
%using 
%\( \IFT_{\targv\nuiv} (\nuiv - \nuivs) = \Delta_{1} \) and 
%\( \| \HFN (\nuiv - \nuivs) \|_{\nano} \leq \| \DFN (\upsv - \upsvs) \|_{\infty} \leq \rrinf \).
As \( \DFN_{1} \IFT_{11}^{-1} \leq \DFN_{1}^{-1} \), bound \eqref{usdhyw6hikhurnetr256} yields
\begin{EQA}
	&& \nquad
	\bigl| \DFN_{1} \{ \upsd_{1}(\nuiv_{1}) - \upss_{1} - \IFT_{11}^{-1} \AAv_{1} + \IFT_{11}^{-1} \IFT_{\ups_{1}\nuiv_{1}}(\nuiv_{1} - \nuivs_{1}) \} \bigr|
	\\
	& \leq &
	(\dltwuns + \dltwunn) \, \| \HFN_{1} (\nuiv_{1} - \nuivs_{1}) \|_{\nano}^{2}
		+ \bigl(2 \dltwu_{3} + \frac{\dltwunn}{2} \bigr) \, \DFN_{1}^{-2} \AAv_{1}^{2}
	\\
	& \leq &
	(\dltwuns + \dltwunn) \rrinf^{2} + \bigl(2 \dltwu_{3} + \frac{\dltwunn}{2} \bigr) \, \| \DFN^{-1} \AAv \|_{\infty}^{2} 
	=
	\dltwunss \, \| \DFN^{-1} \AAv \|_{\infty}^{2} 
	\, .
	\qquad
\label{usdhyw6hikhurnetr256sup}
\end{EQA}
This, \eqref{dekweivytre34wfgbc}, and \eqref{dhfiejfowelocuyehbrf} imply by \( \rrinf = \cmax \| \DFN^{-1} \AAv \|_{\infty} \)
and \( \cmax = \sqrt{2}/(1 - \crosssup) \)
\begin{EQA}
	\bigl| \DFN_{1} \{ \upsd_{1}(\nupv) - \upss_{1} \} \bigr|
	& \leq &
	\| \DFN^{-1} \AAv \|_{\infty} + \crosssup \, \rrinf
	+ \dltwunss \, \| \DFN^{-1} \AAv \|_{\infty}^{2}
	\\
	& \leq &
	\bigl( 1 + \cmax \, \crosssup + \sqrt{2} - 1 \bigr) \| \DFN^{-1} \AAv \|_{\infty}
	=
	\cmax \| \DFN^{-1} \AAv \|_{\infty}
	= 
	\rrinf \, .
\label{7deje8vg7g76gvgv5f43w}
\end{EQA}
The same bounds apply to each \( j \leq \dimp \).
Therefore, when started from any point \( \upsv \in \Upsd \), the sequential optimization procedure 
which maximizes the objective function w.r.t. one coordinate while keeping all the remaining coordinates
has its solution within \( \Upsd \).
As the function \( \fs \) is strongly concave, and its value improves at every step, the procedure converges to a unique solution \( \upsvd \in \Upsd \).
This implies \eqref{7ytdufchskmls7rghnk}.
Further, with \( \upsv = \upsvd \), 
\begin{EQA}
	\IFT_{11} \{ \ups_{1}(\nuiv_{1}) - \upss_{1} \} + \IFT_{\ups_{1}\nuiv_{1}}(\nuiv_{1} - \nuivs_{1})
	&=&
	\IFT (\upsvd - \upsvs) 
	\, .
\label{tdtdtd6tf78gf98ggt}
\end{EQA}
This yields \eqref{usdhyw6hikhurnetrspp}.
Moreover, with \( \uv \eqdef \DFN (\upsvd - \upsvs) \) and \( B \eqdef \DFN^{-1} \IFT \, \DFN^{-1} \), it holds
\begin{EQA}
	\DFN^{-1} \bigl\{ \IFT (\upsvd - \upsvs) - \AAv \bigr\} 
	&=&
	B (\uv - \DFN \, \IFT^{-1} \AAv) \, ,
\label{fi8fu7v7y6vyv44v3eged}
\end{EQA}
and by \eqref{usdhyw6hikhurnetrspp} and Lemma~\ref{LinvGersh} 
\begin{EQA}
	&& \nquad
	\bigl\| \DFN (\upsvd - \upsvs - \IFT^{-1} \AAv) \bigr\|_{\infty}
	=
	\bigl\| \uv - \DFN \, \IFT^{-1} \AAv \bigr\|_{\infty}
	\\
	&=&
	\bigl\| B^{-1} \DFN^{-1} \{ \IFT (\upsvd - \upsvs) - \AAv \} \bigr\|_{\infty}
	\leq 
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \AAv \|_{\infty}^{2} 
	\, .
\label{6f6f67vfg3we5dgwytquw}
\end{EQA}
Finally, by \eqref{Thd7w3jhdujrrfrrfgdyw3} of Lemma~\ref{LinvGersh} and by \( \DFN \, \IFT^{-1} \AAv = \BBN^{-1} \DFN^{-1} \AAv  \)
\begin{EQA}[rcccl]
	\| \DFN \, \IFT^{-1} \AAv - \DFN^{-1} \AAv \|_{\infty}
	& = &
	\bigl\| (\BBN^{-1} - \Id_{\dimp}) \DFN^{-1} \AAv \bigr\|_{\infty}
	& \leq &
	\frac{\crosssup}{1 - \crosssup} \| \DFN^{-1} \AAv \bigr\|_{\infty} \, ,
	\\
	\| \DFN \, \IFT^{-1} \AAv - (\Id_{\dimp} + \Delta) \DFN^{-1} \AAv \|_{\infty}
	& = &
	\bigl\| (\BBN^{-1} - \Id_{\dimp} - \Delta) \DFN^{-1} \AAv \bigr\|_{\infty}
	& \leq &
	\frac{\crosssup^{2}}{1 - \crosssup} \| \DFN^{-1} \AAv \bigr\|_{\infty} \, .
\label{6c6tyc6c6cf6de5tw5}
\end{EQA}
This and \eqref{6f6f67vfg3we5dgwytquw} imply the final inequalities of the proposition.
\end{proof}

\begin{lemma}
\label{LinvGersh}
Let \( \BBN = (\BBN_{ij}) \in \Matr_{\dimp} \) with \( \BBN_{ii} = 1 \) and 
\begin{EQA}[c]
	\sup_{\uv \colon \| \uv \|_{\infty} \leq 1} \, \| (\BBN - \Id_{\dimp}) \uv \|_{\infty} \leq \crosssup < 1 .
\label{8f98dej237yt656543n}
\end{EQA}
Then \( \| \BBN \uv \|_{\infty} \leq (1 - \crosssup)^{-1} \| \uv \|_{\infty} \) for any \( \uv \in \R^{\dimp} \).
Similarly,
\begin{EQA}[c]
	\| (\BBN^{-1} - \Id_{\dimp}) \uv \|_{\infty} \leq \frac{\crosssup}{1 - \crosssup} \, \| \uv \|_{\infty}
	\, ,
	\quad
	\| (\BBN^{-1} - 2 \Id_{\dimp} + \BBN) \uv \|_{\infty} \leq \frac{\crosssup^{2}}{1 - \crosssup} \, \| \uv \|_{\infty}
	\, .
	\qquad
\label{Thd7w3jhdujrrfrrfgdyw3}
\end{EQA}
\end{lemma}

\begin{proof}
Represent \( \BBN = \Id_{\dimp} - \Delta \).
Then \eqref{8f98dej237yt656543n} implies \( \| \Delta \uv \|_{\infty} \leq \crosssup \| \uv \|_{\infty} \).
The use of \( \BBN^{-1} = \Id_{\dimp} + \Delta + \Delta^{2} + \ldots \) yields for any \( \uv \in \R^{\dimp} \)
\begin{EQA}[c]
	\| \BBN^{-1} \uv \|_{\infty}
	\leq 
	\sum_{m=0}^{\infty} \| \Delta^{m} \uv \|_{\infty} \, .
\end{EQA}
Further, with \( \uv_{m} \eqdef \Delta^{m} \uv \), it holds
\begin{EQA}
	\| \Delta^{m+1} \uv \|_{\infty}
	&=&
	\| \Delta \uv_{m} \|_{\infty}
	\leq 
	\crosssup \| \uv_{m} \|_{\infty} \, .
\label{cd7dysrtd4ftgewhged4r}
\end{EQA}
By induction, this yields \( \| \Delta^{m} \uv \|_{\infty} \leq \crosssup^{m} \| \uv \|_{\infty} \) and thus,
\begin{EQA}[c]
	\| \BBN^{-1} \uv \|_{\infty}
	\leq 
	\sum_{m=0}^{\infty} \crosssup^{m} \| \uv \|_{\infty}
	= 
	\frac{1}{1 - \crosssup} \, \| \uv \|_{\infty}
\end{EQA}
as claimed. 
The proof of \eqref{Thd7w3jhdujrrfrrfgdyw3} is similar in view of \( \Id_{\dimp} + \Delta = 2 \Id_{\dimp} - \BBN \).
\end{proof}

\Section{Sup-norm expansions for a separable perturbation}
A linear perturbation is a special case of a separable perturbation of the form 
\( \pert(\upsv) = \sum_{j} \pert_{j}(\ups_{j}) \).
Another popular example is a Tikhonov regularization with \( \pert_{j}(\ups_{j}) = \lambda \ups_{j}^{2} \) or, 
more generally, a Sobolev-type penalty \( \pert_{j}(\ups_{j}) = \gp_{j}^{2} \ups_{j}^{2} \) for a given sequence 
\( \gp_{j}^{2} \).
Later we assume each component \( \pert_{j}(\ups_{j}) \) to be sufficiently smooth.
This does not allow to incorporate a sparse penalty \( \pert_{j}(\ups_{j}) = \lambda |\ups_{j}| \) or
complexity penalty \( \pert_{j}(\ups_{j}) = \lambda \Ind(\ups_{j} \neq 0) \).

Let \( \fs(\upsv) \) be concave, \( \upsvs = \argmax_{\upsv} \fs(\upsv) \), and
\( \IFT = - \nabla^{2} \fs(\upsvs) = (\IFT_{jm}) \).
Define a separable perturbation \( \fn(\upsv) = \fs(\upsv) - \pert(\upsv) \) of \( \fs(\upsv) \) by smooth functions \( \pert_{j}(\ups_{j}) \):
\begin{EQA}
	\fn(\upsv)
	&=&
	\fs(\upsv) - \pert(\upsv)
	=
	\fs(\upsv) - \sum_{j} \pert_{j}(\ups_{j}), 
\label{c7c7ctefwct5enfvyewsd}
\end{EQA} 
and let \( \upsvn = \argmax_{\upsv} \fn(\upsv) \).
We intend to bound the corresponding change \( \upsvn - \upsvs \) in a sup-norm.
Separability of the penalty is very useful, the cross derivatives of \( \fn \) are the same as for \( \fs \).
We only update the tensor \( \DFN(\upsv) \) assuming concavity of each \( \pert_{j}(\cdot) \):
\begin{EQA}
	\DFN(\upsv)
	& \eqdef &
	\diag\{ \DFN_{1}(\upsv),\ldots,\DFN_{\dimp}(\upsv) \},
	\qquad
	\DFN_{j}^{2}(\upsv)
	\eqdef
	\IF_{jj}(\upsv) - \pert''_{j}(\ups_{j}) \, .
\label{7fyc5wgdf7vrewgdhfywh}
\end{EQA}

\begin{proposition}
\label{Psemibiassupp}
Let \( \fs(\upsv) \) be concave function and 
\( \fn(\upsv) \) be a separable perturbation of \( \fs(\upsv) \); see \eqref{c7c7ctefwct5enfvyewsd}. 
For \( \upsvn = \argmax_{\upsv} \fn(\upsv) \), define the diagonal metric tensor \( \DFN = \DFN(\upsvn) \); 
see \eqref{7fyc5wgdf7vrewgdhfywh}.
Let \( \crosssup \) from \eqref{7tdsyf8iuwopkrtg4576} fulfill \( \crosssup < 1 \). 
Fix \( \Avm \eqdef \nabla \pert(\upsvs) = (\pert'_{j}(\upss_{j})) \) and 
\begin{EQA}
	\rrinf 
	&=& 
	\frac{\sqrt{2}}{1 - \crosssup} \| \DFN^{-1} \Avm \|_{\infty} 
	\, .
\label{8drywjwuycrt5sdeteyhfuwkp}
\end{EQA}
Let \nameref{LLpsupref} hold for \( \fn \) with this \( \rrinf \) and
\( \dltwun, \dltwunn, \dltwu_{3} \) satisfying  
\begin{EQA}[c]
	\dltwbun = \dltwunn \, \rrinf \leq 1/4 ,
	\qquad
	\dltwun \, \rrinf \leq 1/4 \, ,
	\qquad	
	\dltwunss \| \DFN^{-1} \Avm \|_{\infty} 
	\leq 
	\sqrt{2} - 1
	\, ,
\label{dhfiejfowelocuyehbrfp}
\end{EQA}
where
\begin{EQA}[rcl]
	\dltwuns
	& \eqdef &
	\frac{1}{1 - \dltwbun} \, 
	\biggl( \crosssup \, \dltwunn + \frac{\dltwun}{2}
		+ \frac{3(\crosssup + \dltwbun/2)^{2} \, \dltwu_{3}}{4(1 - \dltwbun)^{2}} 
%		+ \frac{3\dltwu_{3}\, \dltwun^{2} \, \rru^{2}}{4(1 - \dltwbund)^{2}} 
	\biggr) 
	\, ,
\label{36gfijh94ejdvtwekoisedip}
	\\
	\dltwunss
	& \eqdef &
	2 \dltwu_{3} + \frac{\dltwunn}{2}  + \frac{2(\dltwuns + \dltwunn)}{(1 - \crosssup)^{2}} 
	\, .
\end{EQA}
Then \( \upsvd = \argmax_{\upsv} \fn(\upsv) \) satisfies
\begin{EQA}
	\| \DFN (\upsvd - \upsvs) \|_{\infty}
	\eqdef
	\max_{j \leq \dimp} | \DFN_{j} (\upsd_{j} - \upss_{j}) |
	& \leq &
	\rrinf \, .
\label{7ytdufchskmls7rghnkp}
\end{EQA} 
Furthermore, 
\begin{EQA}
\label{usdhyw6hikhurnetrsppp}
	\bigl\| \DFN^{-1} \bigl\{ \IFT (\upsvd - \upsvs) - \Avm \bigr\} \bigr\|_{\infty}
	& \leq &
	\dltwunss \, \| \DFN^{-1} \Avm \|_{\infty}^{2} 
	\, ,
	\\
	\bigl\| \DFN (\upsvd - \upsvs - \IFT^{-1} \Avm) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \Avm \|_{\infty}^{2} 
	\, ,
	\qquad
\label{usdhyw6hikhurnetrspp1p}
\end{EQA}
and with \( \Delta \eqdef \Id_{\dimp} - \DFN^{-1} \IFT \, \DFN^{-1} \)
\begin{EQ}[rcl]
	\bigl\| \DFN (\upsvd - \upsvs) - \DFN^{-1} \Avm) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \Avm \|_{\infty}^{2} + \frac{\crosssup}{1 - \crosssup} \, \| \DFN^{-1} \Avm \|_{\infty}
	\, ,
	\\
	\bigl\| \DFN (\upsvd - \upsvs) - (\Id_{\dimp} + \Delta) \DFN^{-1} \Avm) \bigr\|_{\infty}
	& \leq &
	\frac{\dltwunss}{1 - \crosssup} \, \| \DFN^{-1} \Avm \|_{\infty}^{2} + \frac{\crosssup^{2}}{1 - \crosssup} \, \| \DFN^{-1} \Avm \|_{\infty}
	\, .
	\qquad
\label{usdhyw6hikhurnetrspp2p}
\end{EQ}
\end{proposition}

\begin{remark}
\label{RLLsup}
If each \( \pert_{j}(\ups_{j}) \) is quadratic, then condition \nameref{LLpsupref} for \( \fn(\upsv) \) follows from 
the same condition for \( \fs(\upsv) \) as the third derivatives of these two functions coincide.
For general smooth perturbations \( \pert_{j} \), \eqref{d6f53ye5vry4fddfgsup} should be checked
for \( \nabla^{3}_{\ups_{j}\ups_{j} \ups_{j}} \fn(\upsv) = \nabla^{3}_{\ups_{j}\ups_{j} \ups_{j}} \fs(\upsv) + \pert'''_{j}(\ups_{j}) \).
The other conditions in \nameref{LLpsupref} can be checked for \( \fs \).
\end{remark}



